Unchecked or Falsely Accused? Evaluating AI-Generated Text Detectors on Kazakh

AI-text detectors are already applied to Kazakh writing, yet no study reports how often publicly available detectors flag Kazakh text whose human authorship is dated before ChatGPT. We present AINA-KK: 3,811 human passages from encyclopedic, news, web and educational pages that provably existed before ChatGPT, and 5,597 machine and gray-zone passages from 9 generators, including the Kazakh-built KazLLM and Sherkala, with script and length stress tests. Five English-trained detectors from the Hugging Face Hub flag up to 81.4% of human passages and 79.6% of published student essays; recalibrated, they catch at most 1.3% of machine text. Calibrated zero-shot detectors catch at most 50.3% of machine text from in-distribution generators. Fine-tuned encoders rank text almost perfectly, but mDeBERTa at its default threshold flags 24.4% of 50-word human excerpts, partly because machine outputs are shorter than human text; calibrated, it catches only 47.1% of KazLLM and 62.7% of Sherkala passages. Without script handling, machine-transliterated Latin-2021 text defeats every detector. Fixes that need no new data (calibration, script canonicalization, script-augmented and length-matched training, and an OR with a zero-shot scorer) form AINA-KK-Det. On test it flags 0.9% of human passages (95% CI 0.4-2.7; 1.5% on development data) and catches 85.2% of machine text from known generators, 92.9% from two unseen Gemini-family Gemma-4 models and 61.3% from the Kazakh-built ones; its configuration was chosen with test results in view. We release the data, code and detector at https://github.com/ozxmn/aina-kk.

==> results.tex <==
\makeatletter
\newcommand{\res}[1]{\@ifundefined{res@#1}{\textbf{??#1??}}{\@nameuse{res@#1}}}
\@namedef{res@aud/human-valid-h}{75.0}
\@namedef{res@aud/human-valid-m}{66.7}
\@namedef{res@aud/kappa}{0.38}
\@namedef{res@aud/llm-valid-h}{88.7}
\@namedef{res@aud/llm-valid-m}{92.7}
\@namedef{res@aud/mt/g31fl/n}{1}
\@namedef{res@aud/mt/g31fl/of}{8}
\@namedef{res@aud/mt/gemma31/n}{5}
\@namedef{res@aud/mt/gemma31/of}{15}
\@namedef{res@aud/mt/gptoss/n}{2}
\@namedef{res@aud/mt/gptoss/of}{10}
\@namedef{res@aud/mt/qwen/n}{1}
\@namedef{res@aud/mt/qwen/of}{3}
\@namedef{res@aud/n-both}{100}
\@namedef{res@aud/n-disagree}{21}
\@namedef{res@aud/n-disagree-mt}{9}
\@namedef{res@aud/n-human-judged}{100}
\@namedef{res@aud/n-llm}{273}
\@namedef{res@aud/post/fakespot-roberta/invalid}{2}
\@namedef{res@aud/post/fakespot-roberta/valid}{9}
\@namedef{res@aud/post/h-broken}{12}
\@namedef{res@aud/post/h-mt}{5}
\@namedef{res@aud/post/h-other}{2}
\@namedef{res@aud/post/h-valid}{33}
\@namedef{res@aud/post/h-valid-w}{66}
\@namedef{res@aud/post/h-valid-w-ci/hi}{79}
\@namedef{res@aud/post/h-valid-w-ci/lo}{52}
\@namedef{res@aud/post/m-broken}{two}
\@namedef{res@aud/post/m-mt}{7}
\@namedef{res@aud/post/n}{100}
\@namedef{res@aud/post/n-h}{52}
\@namedef{res@aud/post/n-h-per-domain}{13}
\@namedef{res@aud/post/n-invalid}{19}
\@namedef{res@aud/post/n-m}{48}
\@namedef{res@aud/post/n-m-per-gen}{6}
\@namedef{res@aud/post/n-valid}{33}
\@namedef{res@aud/post/overlap-first}{0}
\@namedef{res@aud/post/tmr-roberta/invalid}{15}
\@namedef{res@aud/post/tmr-roberta/valid}{28}
\@namedef{res@aud/raw}{79.0}
\@namedef{res@canon/charsim}{99.1}
\@namedef{res@canon/n}{901}
\@namedef{res@canon/n-aligned}{901}
\@namedef{res@canon/word-exact}{96.1}
\@namedef{res@compute/ft-run-minutes}{ten}
\@namedef{res@compute/gpu-hours}{25}
\@namedef{res@const/accum}{2}
\@namedef{res@const/aug-hg}{0.20}
\@namedef{res@const/aug-hg-rates}{5, 10 or 20}
\@namedef{res@const/aug-hg-words}{a fifth}
\@namedef{res@const/aug-latin}{0.25}
\@namedef{res@const/aug-latin-words}{a quarter}
\@namedef{res@const/batch}{16}
\@namedef{res@const/boot-auc-B}{300}
\@namedef{res@const/boot-rate-B}{400}
\@namedef{res@const/c2-prefix}{50}
\@namedef{res@const/ci-level}{95}
\@namedef{res@const/clip}{1.0}
\@namedef{res@const/cutoff-date}{30 Nov 2022}
\@namedef{res@const/default-thr}{0.5}
\@namedef{res@const/epochs}{2}
\@namedef{res@const/excerpt-hi}{120}
\@namedef{res@const/excerpt-lo}{40}
\@namedef{res@const/glotlid-p}{0.9}
\@namedef{res@const/gpu-gb}{16}
\@namedef{res@const/hg-attack}{10}
\@namedef{res@const/id-digits}{12}
\@namedef{res@const/jaccard}{0.8}
\@namedef{res@const/lenctrl-hi}{220}
\@namedef{res@const/lenctrl-lo}{120}
\@namedef{res@const/lenmatch-ex}{15}
\@namedef{res@const/lenmatch-h}{half}
\@namedef{res@const/lr}{$2\times10^{-5}$}
\@namedef{res@const/max-tokens}{512}
\@namedef{res@const/max-words}{320}
\@namedef{res@const/microbatch}{8}
\@namedef{res@const/min-words}{60}
\@namedef{res@const/ngram}{6}
\@namedef{res@const/per-n}{1,000}
\@namedef{res@const/prevalence}{5}
\@namedef{res@const/req-words}{150, 200 or 250}
\@namedef{res@const/seeds}{three}
\@namedef{res@const/seeds-digit}{3}
\@namedef{res@const/span-max}{320}
\@namedef{res@const/span-min}{120}
\@namedef{res@const/target-fpr}{1}
\@namedef{res@const/trunc-long}{100}
\@namedef{res@const/trunc-short}{50}
\@namedef{res@const/trunc-short-word}{Fifty}
\@namedef{res@const/warmup}{6}
\@namedef{res@const/wd}{0.01}
\@namedef{res@const/xsplit-jaccard}{0.3}
\@namedef{res@corpus/gen/g31fl/HP}{127}
\@namedef{res@corpus/gen/g31fl/M}{758}
\@namedef{res@corpus/gen/g31fl/MH}{0}
\@namedef{res@corpus/gen/g31fl/MIX}{351}
\@namedef{res@corpus/gen/g31fl/MT}{86}
\@namedef{res@corpus/gen/g35fl/HP}{0}
\@namedef{res@corpus/gen/g35fl/M}{831}
\@namedef{res@corpus/gen/g35fl/MH}{147}
\@namedef{res@corpus/gen/g35fl/MIX}{388}
\@namedef{res@corpus/gen/g35fl/MT}{0}
\@namedef{res@corpus/gen/gemma26/HP}{0}
\@namedef{res@corpus/gen/gemma26/M}{310}
\@namedef{res@corpus/gen/gemma26/MH}{0}
\@namedef{res@corpus/gen/gemma26/MIX}{137}
\@namedef{res@corpus/gen/gemma26/MT}{0}
\@namedef{res@corpus/gen/gemma31/HP}{0}
\@namedef{res@corpus/gen/gemma31/M}{404}
\@namedef{res@corpus/gen/gemma31/MH}{0}
\@namedef{res@corpus/gen/gemma31/MIX}{185}
\@namedef{res@corpus/gen/gemma31/MT}{0}
\@namedef{res@corpus/gen/gptoss/HP}{60}
\@namedef{res@corpus/gen/gptoss/M}{316}
\@namedef{res@corpus/gen/gptoss/MH}{0}
\@namedef{res@corpus/gen/gptoss/MIX}{149}
\@namedef{res@corpus/gen/gptoss/MT}{0}
\@namedef{res@corpus/gen/kazllm/HP}{0}
\@namedef{res@corpus/gen/kazllm/M}{215}
\@namedef{res@corpus/gen/kazllm/MH}{0}
\@namedef{res@corpus/gen/kazllm/MIX}{101}
\@namedef{res@corpus/gen/kazllm/MT}{0}
\@namedef{res@corpus/gen/nllb/HP}{0}
\@namedef{res@corpus/gen/nllb/M}{0}
\@namedef{res@corpus/gen/nllb/MH}{0}
\@namedef{res@corpus/gen/nllb/MIX}{0}
\@namedef{res@corpus/gen/nllb/MT}{198}
\@namedef{res@corpus/gen/qwen/HP}{0}
\@namedef{res@corpus/gen/qwen/M}{313}
\@namedef{res@corpus/gen/qwen/MH}{0}
\@namedef{res@corpus/gen/qwen/MIX}{146}
\@namedef{res@corpus/gen/qwen/MT}{58}
\@namedef{res@corpus/gen/sherkala/HP}{0}
\@namedef{res@corpus/gen/sherkala/M}{216}
\@namedef{res@corpus/gen/sherkala/MH}{0}
\@namedef{res@corpus/gen/sherkala/MIX}{101}
\@namedef{res@corpus/gen/sherkala/MT}{0}
\@namedef{res@corpus/heldout-names}{KazLLM-1.0-8B, Sherkala-8B-Chat, Gemma 4 26B-A4B, Gemma 4 31B}
\@namedef{res@corpus/n-domains}{four}
\@namedef{res@corpus/n-domains-n}{4}
\@namedef{res@corpus/n-edu-hosts}{68}
\@namedef{res@corpus/n-gen}{9}
\@namedef{res@corpus/n-heldout-gemma}{two}
\@namedef{res@corpus/n-heldout-gens}{four}
\@namedef{res@corpus/n-heldout-m}{1,145}
\@namedef{res@corpus/n-heldout-mix}{524}
\@namedef{res@corpus/n-heldout-rows}{1,669}
\@namedef{res@corpus/n-human}{3,811}
\@namedef{res@corpus/n-label/H}{3,811}
\@namedef{res@corpus/n-label/HP}{187}
\@namedef{res@corpus/n-label/M}{3,363}
\@namedef{res@corpus/n-label/MH}{147}
\@namedef{res@corpus/n-label/MIX}{1,558}
\@namedef{res@corpus/n-label/MT}{342}
\@namedef{res@corpus/n-nonhuman}{5,597}
\@namedef{res@corpus/n-outlets}{27}
\@namedef{res@corpus/n-train-gens}{four}
\@namedef{res@corpus/n-zs-families}{four}
\@namedef{res@corpus/variant/H/devtrunc100}{391}
\@namedef{res@corpus/variant/H/devtrunc50}{391}
\@namedef{res@corpus/variant/H/folded}{197}
\@namedef{res@corpus/variant/H/latin2021}{503}
\@namedef{res@corpus/variant/H/latin2021canon}{503}
\@namedef{res@corpus/variant/H/trunc100}{394}
\@namedef{res@corpus/variant/H/trunc50}{394}
\@namedef{res@corpus/variant/M/homoglyph10}{409}
\@namedef{res@corpus/variant/M/homoglyph10fold}{409}
\@namedef{res@corpus/variant/M/latin2021}{398}
\@namedef{res@corpus/variant/M/latin2021canon}{398}
\@namedef{res@corpus/variant/M/trunc100}{394}
\@namedef{res@corpus/variant/M/trunc50}{394}
\@namedef{res@cue/bold_markup/g31fl}{2.6}
\@namedef{res@cue/bold_markup/g35fl}{1.3}
\@namedef{res@cue/bold_markup/gemma26}{10.2}
\@namedef{res@cue/bold_markup/gemma31}{10.2}
\@namedef{res@cue/bold_markup/gptoss}{7.5}
\@namedef{res@cue/bold_markup/h}{0.0}
\@namedef{res@cue/bold_markup/kazllm}{0.0}
\@namedef{res@cue/bold_markup/m}{3.9}
\@namedef{res@cue/bold_markup/qwen}{1.3}
\@namedef{res@cue/bold_markup/sherkala}{1.3}
\@namedef{res@cue/ellipsis_char/g31fl}{0.0}
\@namedef{res@cue/ellipsis_char/g35fl}{0.5}
\@namedef{res@cue/ellipsis_char/gemma26}{0.6}
\@namedef{res@cue/ellipsis_char/gemma31}{0.2}
\@namedef{res@cue/ellipsis_char/gptoss}{1.3}
\@namedef{res@cue/ellipsis_char/h}{2.2}
\@namedef{res@cue/ellipsis_char/kazllm}{0.0}
\@namedef{res@cue/ellipsis_char/m}{0.3}
\@namedef{res@cue/ellipsis_char/qwen}{0.0}
\@namedef{res@cue/ellipsis_char/sherkala}{0.0}
\@namedef{res@cue/latin_homoglyph/g31fl}{0.0}
\@namedef{res@cue/latin_homoglyph/g35fl}{4.0}
\@namedef{res@cue/latin_homoglyph/gemma26}{0.6}
\@namedef{res@cue/latin_homoglyph/gemma31}{1.0}
\@namedef{res@cue/latin_homoglyph/gptoss}{2.8}
\@namedef{res@cue/latin_homoglyph/h}{5.1}
\@namedef{res@cue/latin_homoglyph/kazllm}{0.0}
\@namedef{res@cue/latin_homoglyph/m}{1.7}
\@namedef{res@cue/latin_homoglyph/qwen}{1.6}
\@namedef{res@cue/latin_homoglyph/sherkala}{2.1}
\@namedef{res@cue/markdown_header/g31fl}{0.0}
\@namedef{res@cue/markdown_header/g35fl}{0.0}
\@namedef{res@cue/markdown_header/gemma26}{0.0}
\@namedef{res@cue/markdown_header/gemma31}{0.0}
\@namedef{res@cue/markdown_header/gptoss}{0.9}
\@namedef{res@cue/markdown_header/h}{0.0}
\@namedef{res@cue/markdown_header/kazllm}{0.0}
\@namedef{res@cue/markdown_header/m}{0.1}
\@namedef{res@cue/markdown_header/qwen}{0.0}
\@namedef{res@cue/markdown_header/sherkala}{0.0}
\@namedef{res@cue/mixed_script_token/g31fl}{0.0}
\@namedef{res@cue/mixed_script_token/g35fl}{4.0}
\@namedef{res@cue/mixed_script_token/gemma26}{1.0}
\@namedef{res@cue/mixed_script_token/gemma31}{2.1}
\@namedef{res@cue/mixed_script_token/gptoss}{0.0}
\@namedef{res@cue/mixed_script_token/h}{0.0}
\@namedef{res@cue/mixed_script_token/kazllm}{0.0}
\@namedef{res@cue/mixed_script_token/m}{1.6}
\@namedef{res@cue/mixed_script_token/qwen}{2.2}
\@namedef{res@cue/mixed_script_token/sherkala}{0.8}
\@namedef{res@cue/n-human}{3,299}
\@namedef{res@cue/n-machine}{3,483}
\@namedef{res@cue/narrow_nbsp_U+202F/g31fl}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/g35fl}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/gemma26}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/gemma31}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/gptoss}{7.8}
\@namedef{res@cue/narrow_nbsp_U+202F/h}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/kazllm}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/m}{0.7}
\@namedef{res@cue/narrow_nbsp_U+202F/qwen}{0.0}
\@namedef{res@cue/narrow_nbsp_U+202F/sherkala}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/g31fl}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/g35fl}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/gemma26}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/gemma31}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/gptoss}{41.7}
\@namedef{res@cue/nb_hyphen_U+2011/h}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/kazllm}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/m}{3.8}
\@namedef{res@cue/nb_hyphen_U+2011/qwen}{0.0}
\@namedef{res@cue/nb_hyphen_U+2011/sherkala}{0.0}
\@namedef{res@cue/soft_hyphen_U+00AD/g31fl}{0.0}
\@namedef{res@cue/soft_hyphen_U+00AD/g35fl}{0.1}
\@namedef{res@cue/soft_hyphen_U+00AD/gemma26}{0.0}
\@namedef{res@cue/soft_hyphen_U+00AD/gemma31}{0.0}
\@namedef{res@cue/soft_hyphen_U+00AD/gptoss}{0.3}
\@namedef{res@cue/soft_hyphen_U+00AD/h}{1.6}
\@namedef{res@cue/soft_hyphen_U+00AD/kazllm}{0.0}
\@namedef{res@cue/soft_hyphen_U+00AD/m}{0.1}
\@namedef{res@cue/soft_hyphen_U+00AD/qwen}{0.3}
\@namedef{res@cue/soft_hyphen_U+00AD/sherkala}{0.0}
\@namedef{res@cue/title_line/g31fl}{1.2}
\@namedef{res@cue/title_line/g35fl}{0.8}
\@namedef{res@cue/title_line/gemma26}{6.7}
\@namedef{res@cue/title_line/gemma31}{5.5}
\@namedef{res@cue/title_line/gptoss}{1.9}
\@namedef{res@cue/title_line/h}{0.9}
\@namedef{res@cue/title_line/kazllm}{3.7}
\@namedef{res@cue/title_line/m}{2.4}
\@namedef{res@cue/title_line/qwen}{1.3}
\@namedef{res@cue/title_line/sherkala}{2.1}
\@namedef{res@cue/trailing_fragment/g31fl}{0.0}
\@namedef{res@cue/trailing_fragment/g35fl}{0.0}
\@namedef{res@cue/trailing_fragment/gemma26}{0.3}
\@namedef{res@cue/trailing_fragment/gemma31}{0.0}
\@namedef{res@cue/trailing_fragment/gptoss}{0.3}
\@namedef{res@cue/trailing_fragment/h}{3.6}
\@namedef{res@cue/trailing_fragment/kazllm}{5.8}
\@namedef{res@cue/trailing_fragment/m}{1.6}
\@namedef{res@cue/trailing_fragment/qwen}{1.9}
\@namedef{res@cue/trailing_fragment/sherkala}{14.6}
\@namedef{res@det/all/auroc}{0.997}
\@namedef{res@det/all/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/all/auroc-by-gen/g35fl}{0.997}
\@namedef{res@det/all/auroc-by-gen/gemma26}{0.997}
\@namedef{res@det/all/auroc-by-gen/gemma31}{0.997}
\@namedef{res@det/all/auroc-by-gen/gptoss}{0.995}
\@namedef{res@det/all/auroc-by-gen/kazllm}{0.968}
\@namedef{res@det/all/auroc-by-gen/qwen}{0.995}
\@namedef{res@det/all/auroc-by-gen/sherkala}{0.967}
\@namedef{res@det/all/auroc-ci/hi}{0.999}
\@namedef{res@det/all/auroc-ci/lo}{0.995}
\@namedef{res@det/all/auroc-heldout}{0.986}
\@namedef{res@det/all/auroc-len120-220}{0.998}
\@namedef{res@det/all/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/kazllm}{95.3}
\@namedef{res@det/all/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/all/flag-by-gen-at-0.5/sherkala}{92.0}
\@namedef{res@det/all/flag-by-gen-at-dev/g31fl}{99.6}
\@namedef{res@det/all/flag-by-gen-at-dev/g35fl}{94.1}
\@namedef{res@det/all/flag-by-gen-at-dev/gemma26}{98.2}
\@namedef{res@det/all/flag-by-gen-at-dev/gemma31}{97.6}
\@namedef{res@det/all/flag-by-gen-at-dev/gptoss}{88.7}
\@namedef{res@det/all/flag-by-gen-at-dev/kazllm}{29.4}
\@namedef{res@det/all/flag-by-gen-at-dev/qwen}{85.6}
\@namedef{res@det/all/flag-by-gen-at-dev/sherkala}{42.7}
\@namedef{res@det/all/flag-gray-at-0.5/HP}{65.4}
\@namedef{res@det/all/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/all/flag-gray-at-0.5/MIX}{96.3}
\@namedef{res@det/all/flag-gray-at-0.5/MT}{56.4}
\@namedef{res@det/all/flag-gray-at-dev/HP}{10.3}
\@namedef{res@det/all/flag-gray-at-dev/MH}{92.2}
\@namedef{res@det/all/flag-gray-at-dev/MIX}{51.4}
\@namedef{res@det/all/flag-gray-at-dev/MT}{4.1}
\@namedef{res@det/all/fpr-at-0.5}{12.6}
\@namedef{res@det/all/fpr-at-dev}{1.1}
\@namedef{res@det/all/fpr-at-dev-ci-thr/hi}{2.2}
\@namedef{res@det/all/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/all/fpr-at-dev-ci/hi}{1.6}
\@namedef{res@det/all/fpr-at-dev-ci/lo}{0.7}
\@namedef{res@det/all/fpr-at-lenaware}{0.8}
\@namedef{res@det/all/fpr-by-domain-at-0.5/encyclopedic}{8.4}
\@namedef{res@det/all/fpr-by-domain-at-0.5/essay}{6.5}
\@namedef{res@det/all/fpr-by-domain-at-0.5/news}{13.4}
\@namedef{res@det/all/fpr-by-domain-at-0.5/web}{18.1}
\@namedef{res@det/all/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/all/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/all/fpr-by-domain-at-dev/news}{0.6}
\@namedef{res@det/all/fpr-by-domain-at-dev/web}{3.0}
\@namedef{res@det/all/fpr-by-len-at-0.5/120-160}{21.2}
\@namedef{res@det/all/fpr-by-len-at-0.5/160-220}{11.3}
\@namedef{res@det/all/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/all/fpr-by-len-at-dev/120-160}{2.6}
\@namedef{res@det/all/fpr-by-len-at-dev/160-220}{0.8}
\@namedef{res@det/all/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/all/fpr-by-len-at-lenaware/120-160}{0.6}
\@namedef{res@det/all/fpr-by-len-at-lenaware/160-220}{0.8}
\@namedef{res@det/all/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/all/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/all/script/canon-tpr-at-dev}{94.0}
\@namedef{res@det/all/script/hg-tpr-at-dev}{96.8}
\@namedef{res@det/all/script/hg-tpr-orig-at-dev}{96.3}
\@namedef{res@det/all/script/hgfold-tpr-at-dev}{96.6}
\@namedef{res@det/all/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/all/script/hghum-n}{103}
\@namedef{res@det/all/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/all/script/latin-fpr-at-dev}{0.4}
\@namedef{res@det/all/script/latin-tpr-at-dev}{77.1}
\@namedef{res@det/all/script/latin2021}{0.997}
\@namedef{res@det/all/script/latin2021canon}{0.998}
\@namedef{res@det/all/script/trunc100}{0.987}
\@namedef{res@det/all/script/trunc50}{0.925}
\@namedef{res@det/all/seed-range/fpr-at-dev/hi}{0.7}
\@namedef{res@det/all/seed-range/fpr-at-dev/lo}{0.6}
\@namedef{res@det/all/seed-range/fpr50-at-dev/hi}{0.8}
\@namedef{res@det/all/seed-range/fpr50-at-dev/lo}{0.0}
\@namedef{res@det/all/seed-range/gen/g31fl/hi}{96.8}
\@namedef{res@det/all/seed-range/gen/g31fl/lo}{40.0}
\@namedef{res@det/all/seed-range/gen/g35fl/hi}{91.2}
\@namedef{res@det/all/seed-range/gen/g35fl/lo}{55.2}
\@namedef{res@det/all/seed-range/gen/gemma26/hi}{93.0}
\@namedef{res@det/all/seed-range/gen/gemma26/lo}{42.1}
\@namedef{res@det/all/seed-range/gen/gemma31/hi}{89.9}
\@namedef{res@det/all/seed-range/gen/gemma31/lo}{33.9}
\@namedef{res@det/all/seed-range/gen/gptoss/hi}{87.1}
\@namedef{res@det/all/seed-range/gen/gptoss/lo}{33.9}
\@namedef{res@det/all/seed-range/gen/kazllm/hi}{45.9}
\@namedef{res@det/all/seed-range/gen/kazllm/lo}{4.7}
\@namedef{res@det/all/seed-range/gen/qwen/hi}{79.2}
\@namedef{res@det/all/seed-range/gen/qwen/lo}{32.0}
\@namedef{res@det/all/seed-range/gen/sherkala/hi}{65.3}
\@namedef{res@det/all/seed-range/gen/sherkala/lo}{14.7}
\@namedef{res@det/all/seed-range/tpr-at-dev/hi}{90.3}
\@namedef{res@det/all/seed-range/tpr-at-dev/lo}{44.8}
\@namedef{res@det/all/seed-range/tpr-heldout-at-dev/hi}{78.1}
\@namedef{res@det/all/seed-range/tpr-heldout-at-dev/lo}{31.9}
\@namedef{res@det/all/short/100/auroc}{0.987}
\@namedef{res@det/all/short/100/fpr-at-0.5}{41.9}
\@namedef{res@det/all/short/100/fpr-at-dev}{2.3}
\@namedef{res@det/all/short/100/fpr-at-devlen}{1.3}
\@namedef{res@det/all/short/100/fpr-at-devlen-ci-thr/hi}{3.8}
\@namedef{res@det/all/short/100/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/all/short/100/fpr-at-devlen-ci/hi}{2.5}
\@namedef{res@det/all/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/all/short/100/thr-devlen}{0.9987}
\@namedef{res@det/all/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/all/short/100/tpr-at-dev}{88.6}
\@namedef{res@det/all/short/100/tpr-at-devlen}{66.0}
\@namedef{res@det/all/short/50/auroc}{0.925}
\@namedef{res@det/all/short/50/fpr-at-0.5}{76.9}
\@namedef{res@det/all/short/50/fpr-at-dev}{0.3}
\@namedef{res@det/all/short/50/fpr-at-devlen}{1.5}
\@namedef{res@det/all/short/50/fpr-at-devlen-ci-thr/hi}{3.3}
\@namedef{res@det/all/short/50/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/all/short/50/fpr-at-devlen-ci/hi}{2.5}
\@namedef{res@det/all/short/50/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/all/short/50/thr-devlen}{0.9984}
\@namedef{res@det/all/short/50/tpr-at-0.5}{100.0}
\@namedef{res@det/all/short/50/tpr-at-dev}{14.5}
\@namedef{res@det/all/short/50/tpr-at-devlen}{32.2}
\@namedef{res@det/all/thr-dev}{0.9986}
\@namedef{res@det/all/thr-lenaware/120-160}{0.9988}
\@namedef{res@det/all/thr-lenaware/160-220}{0.9985}
\@namedef{res@det/all/thr-lenaware/220-320}{0.4716}
\@namedef{res@det/all/tpr-at-0.5}{100.0}
\@namedef{res@det/all/tpr-at-dev}{94.9}
\@namedef{res@det/all/tpr-at-lenaware}{81.8}
\@namedef{res@det/all/tpr-heldout-at-0.5}{97.7}
\@namedef{res@det/all/tpr-heldout-at-dev}{75.3}
\@namedef{res@det/alllen/auroc}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/g31fl}{0.999}
\@namedef{res@det/alllen/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/kazllm}{0.977}
\@namedef{res@det/alllen/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/alllen/auroc-by-gen/sherkala}{0.959}
\@namedef{res@det/alllen/auroc-ci/hi}{1.000}
\@namedef{res@det/alllen/auroc-ci/lo}{0.997}
\@namedef{res@det/alllen/auroc-heldout}{0.988}
\@namedef{res@det/alllen/auroc-len120-220}{0.998}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/kazllm}{89.4}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/alllen/flag-by-gen-at-0.5/sherkala}{88.0}
\@namedef{res@det/alllen/flag-by-gen-at-dev/g31fl}{98.8}
\@namedef{res@det/alllen/flag-by-gen-at-dev/g35fl}{97.1}
\@namedef{res@det/alllen/flag-by-gen-at-dev/gemma26}{98.2}
\@namedef{res@det/alllen/flag-by-gen-at-dev/gemma31}{99.4}
\@namedef{res@det/alllen/flag-by-gen-at-dev/gptoss}{91.1}
\@namedef{res@det/alllen/flag-by-gen-at-dev/kazllm}{60.0}
\@namedef{res@det/alllen/flag-by-gen-at-dev/qwen}{96.8}
\@namedef{res@det/alllen/flag-by-gen-at-dev/sherkala}{64.0}
\@namedef{res@det/alllen/flag-gray-at-0.5/HP}{46.2}
\@namedef{res@det/alllen/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/alllen/flag-gray-at-0.5/MIX}{96.4}
\@namedef{res@det/alllen/flag-gray-at-0.5/MT}{39.5}
\@namedef{res@det/alllen/flag-gray-at-dev/HP}{5.1}
\@namedef{res@det/alllen/flag-gray-at-dev/MH}{96.9}
\@namedef{res@det/alllen/flag-gray-at-dev/MIX}{57.0}
\@namedef{res@det/alllen/flag-gray-at-dev/MT}{7.0}
\@namedef{res@det/alllen/fpr-at-0.5}{8.6}
\@namedef{res@det/alllen/fpr-at-dev}{0.5}
\@namedef{res@det/alllen/fpr-at-dev-ci-thr/hi}{2.8}
\@namedef{res@det/alllen/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/alllen/fpr-at-dev-ci/hi}{0.8}
\@namedef{res@det/alllen/fpr-at-dev-ci/lo}{0.1}
\@namedef{res@det/alllen/fpr-at-lenaware}{1.1}
\@namedef{res@det/alllen/fpr-by-domain-at-0.5/encyclopedic}{5.5}
\@namedef{res@det/alllen/fpr-by-domain-at-0.5/essay}{2.8}
\@namedef{res@det/alllen/fpr-by-domain-at-0.5/news}{9.1}
\@namedef{res@det/alllen/fpr-by-domain-at-0.5/web}{13.1}
\@namedef{res@det/alllen/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/alllen/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/alllen/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/alllen/fpr-by-domain-at-dev/web}{1.1}
\@namedef{res@det/alllen/fpr-by-len-at-0.5/120-160}{13.2}
\@namedef{res@det/alllen/fpr-by-len-at-0.5/160-220}{8.0}
\@namedef{res@det/alllen/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/alllen/fpr-by-len-at-dev/120-160}{1.1}
\@namedef{res@det/alllen/fpr-by-len-at-dev/160-220}{0.3}
\@namedef{res@det/alllen/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/alllen/fpr-by-len-at-lenaware/120-160}{3.4}
\@namedef{res@det/alllen/fpr-by-len-at-lenaware/160-220}{0.3}
\@namedef{res@det/alllen/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/alllen/script/canon-fpr-at-dev}{0.8}
\@namedef{res@det/alllen/script/canon-tpr-at-dev}{95.7}
\@namedef{res@det/alllen/script/hg-tpr-at-dev}{98.3}
\@namedef{res@det/alllen/script/hg-tpr-orig-at-dev}{98.8}
\@namedef{res@det/alllen/script/hgfold-tpr-at-dev}{98.8}
\@namedef{res@det/alllen/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/alllen/script/hghum-n}{103}
\@namedef{res@det/alllen/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/alllen/script/latin-fpr-at-dev}{0.4}
\@namedef{res@det/alllen/script/latin-tpr-at-dev}{87.9}
\@namedef{res@det/alllen/script/latin2021}{0.999}
\@namedef{res@det/alllen/script/latin2021canon}{0.998}
\@namedef{res@det/alllen/script/trunc100}{0.991}
\@namedef{res@det/alllen/script/trunc50}{0.985}
\@namedef{res@det/alllen/seed-range/fpr-at-dev/hi}{1.0}
\@namedef{res@det/alllen/seed-range/fpr-at-dev/lo}{0.5}
\@namedef{res@det/alllen/seed-range/fpr50-at-dev/hi}{1.5}
\@namedef{res@det/alllen/seed-range/fpr50-at-dev/lo}{0.8}
\@namedef{res@det/alllen/seed-range/gen/g31fl/hi}{99.4}
\@namedef{res@det/alllen/seed-range/gen/g31fl/lo}{94.0}
\@namedef{res@det/alllen/seed-range/gen/g35fl/hi}{99.0}
\@namedef{res@det/alllen/seed-range/gen/g35fl/lo}{92.3}
\@namedef{res@det/alllen/seed-range/gen/gemma26/hi}{99.1}
\@namedef{res@det/alllen/seed-range/gen/gemma26/lo}{94.7}
\@namedef{res@det/alllen/seed-range/gen/gemma31/hi}{98.8}
\@namedef{res@det/alllen/seed-range/gen/gemma31/lo}{97.0}
\@namedef{res@det/alllen/seed-range/gen/gptoss/hi}{92.7}
\@namedef{res@det/alllen/seed-range/gen/gptoss/lo}{85.5}
\@namedef{res@det/alllen/seed-range/gen/kazllm/hi}{60.0}
\@namedef{res@det/alllen/seed-range/gen/kazllm/lo}{57.6}
\@namedef{res@det/alllen/seed-range/gen/qwen/hi}{94.4}
\@namedef{res@det/alllen/seed-range/gen/qwen/lo}{91.2}
\@namedef{res@det/alllen/seed-range/gen/sherkala/hi}{70.7}
\@namedef{res@det/alllen/seed-range/gen/sherkala/lo}{56.0}
\@namedef{res@det/alllen/seed-range/tpr-at-dev/hi}{98.0}
\@namedef{res@det/alllen/seed-range/tpr-at-dev/lo}{92.2}
\@namedef{res@det/alllen/seed-range/tpr-heldout-at-dev/hi}{86.2}
\@namedef{res@det/alllen/seed-range/tpr-heldout-at-dev/lo}{82.4}
\@namedef{res@det/alllen/short/100/auroc}{0.991}
\@namedef{res@det/alllen/short/100/fpr-at-0.5}{12.4}
\@namedef{res@det/alllen/short/100/fpr-at-dev}{1.3}
\@namedef{res@det/alllen/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/alllen/short/100/fpr-at-devlen-ci-thr/hi}{3.6}
\@namedef{res@det/alllen/short/100/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/alllen/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/alllen/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/alllen/short/100/thr-devlen}{0.9952}
\@namedef{res@det/alllen/short/100/tpr-at-0.5}{99.7}
\@namedef{res@det/alllen/short/100/tpr-at-dev}{89.6}
\@namedef{res@det/alllen/short/100/tpr-at-devlen}{97.5}
\@namedef{res@det/alllen/short/50/auroc}{0.985}
\@namedef{res@det/alllen/short/50/fpr-at-0.5}{25.1}
\@namedef{res@det/alllen/short/50/fpr-at-dev}{1.0}
\@namedef{res@det/alllen/short/50/fpr-at-devlen}{1.8}
\@namedef{res@det/alllen/short/50/fpr-at-devlen-ci-thr/hi}{3.6}
\@namedef{res@det/alllen/short/50/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/alllen/short/50/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/alllen/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/alllen/short/50/thr-devlen}{0.9960}
\@namedef{res@det/alllen/short/50/tpr-at-0.5}{99.2}
\@namedef{res@det/alllen/short/50/tpr-at-dev}{63.2}
\@namedef{res@det/alllen/short/50/tpr-at-devlen}{78.9}
\@namedef{res@det/alllen/thr-dev}{0.9964}
\@namedef{res@det/alllen/thr-lenaware/120-160}{0.9916}
\@namedef{res@det/alllen/thr-lenaware/160-220}{0.9965}
\@namedef{res@det/alllen/thr-lenaware/220-320}{0.6069}
\@namedef{res@det/alllen/tpr-at-0.5}{100.0}
\@namedef{res@det/alllen/tpr-at-dev}{97.2}
\@namedef{res@det/alllen/tpr-at-lenaware}{98.8}
\@namedef{res@det/alllen/tpr-heldout-at-0.5}{95.9}
\@namedef{res@det/alllen/tpr-heldout-at-dev}{85.5}
\@namedef{res@det/allnoaug/auroc}{0.998}
\@namedef{res@det/allnoaug/auroc-by-gen/g31fl}{0.999}
\@namedef{res@det/allnoaug/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/allnoaug/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/allnoaug/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/allnoaug/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/allnoaug/auroc-by-gen/kazllm}{0.978}
\@namedef{res@det/allnoaug/auroc-by-gen/qwen}{0.997}
\@namedef{res@det/allnoaug/auroc-by-gen/sherkala}{0.967}
\@namedef{res@det/allnoaug/auroc-ci/hi}{0.999}
\@namedef{res@det/allnoaug/auroc-ci/lo}{0.996}
\@namedef{res@det/allnoaug/auroc-heldout}{0.989}
\@namedef{res@det/allnoaug/auroc-len120-220}{0.998}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/kazllm}{96.5}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-0.5/sherkala}{92.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/g35fl}{99.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/kazllm}{75.3}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/allnoaug/flag-by-gen-at-dev/sherkala}{73.3}
\@namedef{res@det/allnoaug/flag-gray-at-0.5/HP}{65.4}
\@namedef{res@det/allnoaug/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/allnoaug/flag-gray-at-0.5/MIX}{97.4}
\@namedef{res@det/allnoaug/flag-gray-at-0.5/MT}{55.3}
\@namedef{res@det/allnoaug/flag-gray-at-dev/HP}{14.1}
\@namedef{res@det/allnoaug/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/allnoaug/flag-gray-at-dev/MIX}{75.8}
\@namedef{res@det/allnoaug/flag-gray-at-dev/MT}{14.0}
\@namedef{res@det/allnoaug/fpr-at-0.5}{12.4}
\@namedef{res@det/allnoaug/fpr-at-dev}{1.3}
\@namedef{res@det/allnoaug/fpr-at-dev-ci-thr/hi}{3.7}
\@namedef{res@det/allnoaug/fpr-at-dev-ci-thr/lo}{0.3}
\@namedef{res@det/allnoaug/fpr-at-dev-ci/hi}{1.8}
\@namedef{res@det/allnoaug/fpr-at-dev-ci/lo}{0.8}
\@namedef{res@det/allnoaug/fpr-at-lenaware}{1.3}
\@namedef{res@det/allnoaug/fpr-by-domain-at-0.5/encyclopedic}{8.4}
\@namedef{res@det/allnoaug/fpr-by-domain-at-0.5/essay}{10.6}
\@namedef{res@det/allnoaug/fpr-by-domain-at-0.5/news}{11.7}
\@namedef{res@det/allnoaug/fpr-by-domain-at-0.5/web}{17.2}
\@namedef{res@det/allnoaug/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/allnoaug/fpr-by-domain-at-dev/essay}{0.5}
\@namedef{res@det/allnoaug/fpr-by-domain-at-dev/news}{1.1}
\@namedef{res@det/allnoaug/fpr-by-domain-at-dev/web}{2.8}
\@namedef{res@det/allnoaug/fpr-by-len-at-0.5/120-160}{21.2}
\@namedef{res@det/allnoaug/fpr-by-len-at-0.5/160-220}{10.8}
\@namedef{res@det/allnoaug/fpr-by-len-at-0.5/220-320}{2.8}
\@namedef{res@det/allnoaug/fpr-by-len-at-dev/120-160}{3.2}
\@namedef{res@det/allnoaug/fpr-by-len-at-dev/160-220}{0.9}
\@namedef{res@det/allnoaug/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/allnoaug/fpr-by-len-at-lenaware/120-160}{2.9}
\@namedef{res@det/allnoaug/fpr-by-len-at-lenaware/160-220}{0.9}
\@namedef{res@det/allnoaug/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/allnoaug/script/canon-fpr-at-dev}{1.0}
\@namedef{res@det/allnoaug/script/canon-tpr-at-dev}{98.2}
\@namedef{res@det/allnoaug/script/hg-tpr-at-dev}{25.4}
\@namedef{res@det/allnoaug/script/hg-tpr-orig-at-dev}{99.5}
\@namedef{res@det/allnoaug/script/hgfold-tpr-at-dev}{99.5}
\@namedef{res@det/allnoaug/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/allnoaug/script/hghum-n}{103}
\@namedef{res@det/allnoaug/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/allnoaug/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/allnoaug/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/allnoaug/script/latin2021}{0.879}
\@namedef{res@det/allnoaug/script/latin2021canon}{0.998}
\@namedef{res@det/allnoaug/script/trunc100}{0.989}
\@namedef{res@det/allnoaug/script/trunc50}{0.969}
\@namedef{res@det/allnoaug/seed-range/fpr-at-dev/hi}{2.4}
\@namedef{res@det/allnoaug/seed-range/fpr-at-dev/lo}{0.5}
\@namedef{res@det/allnoaug/seed-range/fpr50-at-dev/hi}{23.9}
\@namedef{res@det/allnoaug/seed-range/fpr50-at-dev/lo}{0.0}
\@namedef{res@det/allnoaug/seed-range/gen/g31fl/hi}{100.0}
\@namedef{res@det/allnoaug/seed-range/gen/g31fl/lo}{88.7}
\@namedef{res@det/allnoaug/seed-range/gen/g35fl/hi}{99.6}
\@namedef{res@det/allnoaug/seed-range/gen/g35fl/lo}{67.2}
\@namedef{res@det/allnoaug/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/allnoaug/seed-range/gen/gemma26/lo}{82.5}
\@namedef{res@det/allnoaug/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/allnoaug/seed-range/gen/gemma31/lo}{79.2}
\@namedef{res@det/allnoaug/seed-range/gen/gptoss/hi}{99.2}
\@namedef{res@det/allnoaug/seed-range/gen/gptoss/lo}{75.0}
\@namedef{res@det/allnoaug/seed-range/gen/kazllm/hi}{82.4}
\@namedef{res@det/allnoaug/seed-range/gen/kazllm/lo}{27.1}
\@namedef{res@det/allnoaug/seed-range/gen/qwen/hi}{100.0}
\@namedef{res@det/allnoaug/seed-range/gen/qwen/lo}{82.4}
\@namedef{res@det/allnoaug/seed-range/gen/sherkala/hi}{88.0}
\@namedef{res@det/allnoaug/seed-range/gen/sherkala/lo}{13.3}
\@namedef{res@det/allnoaug/seed-range/tpr-at-dev/hi}{99.8}
\@namedef{res@det/allnoaug/seed-range/tpr-at-dev/lo}{77.9}
\@namedef{res@det/allnoaug/seed-range/tpr-heldout-at-dev/hi}{94.6}
\@namedef{res@det/allnoaug/seed-range/tpr-heldout-at-dev/lo}{58.8}
\@namedef{res@det/allnoaug/short/100/auroc}{0.989}
\@namedef{res@det/allnoaug/short/100/fpr-at-0.5}{37.8}
\@namedef{res@det/allnoaug/short/100/fpr-at-dev}{5.3}
\@namedef{res@det/allnoaug/short/100/fpr-at-devlen}{2.3}
\@namedef{res@det/allnoaug/short/100/fpr-at-devlen-ci-thr/hi}{5.1}
\@namedef{res@det/allnoaug/short/100/fpr-at-devlen-ci-thr/lo}{0.8}
\@namedef{res@det/allnoaug/short/100/fpr-at-devlen-ci/hi}{4.1}
\@namedef{res@det/allnoaug/short/100/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/allnoaug/short/100/thr-devlen}{0.9991}
\@namedef{res@det/allnoaug/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/allnoaug/short/100/tpr-at-dev}{99.2}
\@namedef{res@det/allnoaug/short/100/tpr-at-devlen}{97.7}
\@namedef{res@det/allnoaug/short/50/auroc}{0.969}
\@namedef{res@det/allnoaug/short/50/fpr-at-0.5}{78.7}
\@namedef{res@det/allnoaug/short/50/fpr-at-dev}{2.0}
\@namedef{res@det/allnoaug/short/50/fpr-at-devlen}{2.3}
\@namedef{res@det/allnoaug/short/50/fpr-at-devlen-ci-thr/hi}{5.1}
\@namedef{res@det/allnoaug/short/50/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/allnoaug/short/50/fpr-at-devlen-ci/hi}{3.8}
\@namedef{res@det/allnoaug/short/50/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/allnoaug/short/50/thr-devlen}{0.9989}
\@namedef{res@det/allnoaug/short/50/tpr-at-0.5}{100.0}
\@namedef{res@det/allnoaug/short/50/tpr-at-dev}{52.8}
\@namedef{res@det/allnoaug/short/50/tpr-at-devlen}{60.4}
\@namedef{res@det/allnoaug/thr-dev}{0.9989}
\@namedef{res@det/allnoaug/thr-lenaware/120-160}{0.9990}
\@namedef{res@det/allnoaug/thr-lenaware/160-220}{0.9990}
\@namedef{res@det/allnoaug/thr-lenaware/220-320}{0.6623}
\@namedef{res@det/allnoaug/tpr-at-0.5}{100.0}
\@namedef{res@det/allnoaug/tpr-at-dev}{99.5}
\@namedef{res@det/allnoaug/tpr-at-lenaware}{99.6}
\@namedef{res@det/allnoaug/tpr-heldout-at-0.5}{98.0}
\@namedef{res@det/allnoaug/tpr-heldout-at-dev}{90.7}
\@namedef{res@det/aug/auroc}{0.999}
\@namedef{res@det/aug/auroc-by-gen/g31fl}{0.999}
\@namedef{res@det/aug/auroc-by-gen/g35fl}{0.999}
\@namedef{res@det/aug/auroc-by-gen/gemma26}{0.999}
\@namedef{res@det/aug/auroc-by-gen/gemma31}{0.999}
\@namedef{res@det/aug/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/aug/auroc-by-gen/kazllm}{0.952}
\@namedef{res@det/aug/auroc-by-gen/qwen}{0.999}
\@namedef{res@det/aug/auroc-by-gen/sherkala}{0.950}
\@namedef{res@det/aug/auroc-ci/hi}{1.000}
\@namedef{res@det/aug/auroc-ci/lo}{0.998}
\@namedef{res@det/aug/auroc-heldout}{0.982}
\@namedef{res@det/aug/auroc-len120-220}{0.999}
\@namedef{res@det/aug/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-0.5/gptoss}{99.2}
\@namedef{res@det/aug/flag-by-gen-at-0.5/kazllm}{74.1}
\@namedef{res@det/aug/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-0.5/sherkala}{82.7}
\@namedef{res@det/aug/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-dev/g35fl}{99.6}
\@namedef{res@det/aug/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-dev/gptoss}{98.4}
\@namedef{res@det/aug/flag-by-gen-at-dev/kazllm}{48.2}
\@namedef{res@det/aug/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/aug/flag-by-gen-at-dev/sherkala}{68.0}
\@namedef{res@det/aug/flag-gray-at-0.5/HP}{33.3}
\@namedef{res@det/aug/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/aug/flag-gray-at-0.5/MIX}{94.8}
\@namedef{res@det/aug/flag-gray-at-0.5/MT}{21.3}
\@namedef{res@det/aug/flag-gray-at-dev/HP}{10.3}
\@namedef{res@det/aug/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/aug/flag-gray-at-dev/MIX}{84.9}
\@namedef{res@det/aug/flag-gray-at-dev/MT}{7.9}
\@namedef{res@det/aug/fpr-at-0.5}{4.6}
\@namedef{res@det/aug/fpr-at-dev}{0.8}
\@namedef{res@det/aug/fpr-at-dev-ci-thr/hi}{2.9}
\@namedef{res@det/aug/fpr-at-dev-ci-thr/lo}{0.0}
\@namedef{res@det/aug/fpr-at-dev-ci/hi}{1.3}
\@namedef{res@det/aug/fpr-at-dev-ci/lo}{0.4}
\@namedef{res@det/aug/fpr-at-lenaware}{1.2}
\@namedef{res@det/aug/fpr-by-domain-at-0.5/encyclopedic}{4.0}
\@namedef{res@det/aug/fpr-by-domain-at-0.5/essay}{0.9}
\@namedef{res@det/aug/fpr-by-domain-at-0.5/news}{4.0}
\@namedef{res@det/aug/fpr-by-domain-at-0.5/web}{7.5}
\@namedef{res@det/aug/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/aug/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/aug/fpr-by-domain-at-dev/news}{0.9}
\@namedef{res@det/aug/fpr-by-domain-at-dev/web}{1.7}
\@namedef{res@det/aug/fpr-by-len-at-0.5/120-160}{7.2}
\@namedef{res@det/aug/fpr-by-len-at-0.5/160-220}{4.1}
\@namedef{res@det/aug/fpr-by-len-at-0.5/220-320}{2.1}
\@namedef{res@det/aug/fpr-by-len-at-dev/120-160}{2.0}
\@namedef{res@det/aug/fpr-by-len-at-dev/160-220}{0.6}
\@namedef{res@det/aug/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/aug/fpr-by-len-at-lenaware/120-160}{0.9}
\@namedef{res@det/aug/fpr-by-len-at-lenaware/160-220}{1.2}
\@namedef{res@det/aug/fpr-by-len-at-lenaware/220-320}{2.8}
\@namedef{res@det/aug/script/canon-fpr-at-dev}{0.8}
\@namedef{res@det/aug/script/canon-tpr-at-dev}{99.7}
\@namedef{res@det/aug/script/hg-tpr-at-dev}{99.8}
\@namedef{res@det/aug/script/hg-tpr-orig-at-dev}{99.8}
\@namedef{res@det/aug/script/hgfold-tpr-at-dev}{99.8}
\@namedef{res@det/aug/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/aug/script/hghum-n}{103}
\@namedef{res@det/aug/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/aug/script/latin-fpr-at-dev}{1.0}
\@namedef{res@det/aug/script/latin-tpr-at-dev}{98.2}
\@namedef{res@det/aug/script/latin2021}{0.998}
\@namedef{res@det/aug/script/latin2021canon}{0.999}
\@namedef{res@det/aug/script/trunc100}{0.995}
\@namedef{res@det/aug/script/trunc50}{0.986}
\@namedef{res@det/aug/seed-range/fpr-at-dev/hi}{1.0}
\@namedef{res@det/aug/seed-range/fpr-at-dev/lo}{0.5}
\@namedef{res@det/aug/seed-range/fpr50-at-dev/hi}{6.3}
\@namedef{res@det/aug/seed-range/fpr50-at-dev/lo}{0.0}
\@namedef{res@det/aug/seed-range/gen/g31fl/hi}{100.0}
\@namedef{res@det/aug/seed-range/gen/g31fl/lo}{30.8}
\@namedef{res@det/aug/seed-range/gen/g35fl/hi}{99.6}
\@namedef{res@det/aug/seed-range/gen/g35fl/lo}{37.0}
\@namedef{res@det/aug/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/aug/seed-range/gen/gemma26/lo}{37.7}
\@namedef{res@det/aug/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/aug/seed-range/gen/gemma31/lo}{19.6}
\@namedef{res@det/aug/seed-range/gen/gptoss/hi}{98.4}
\@namedef{res@det/aug/seed-range/gen/gptoss/lo}{23.4}
\@namedef{res@det/aug/seed-range/gen/kazllm/hi}{49.4}
\@namedef{res@det/aug/seed-range/gen/kazllm/lo}{5.9}
\@namedef{res@det/aug/seed-range/gen/qwen/hi}{100.0}
\@namedef{res@det/aug/seed-range/gen/qwen/lo}{28.8}
\@namedef{res@det/aug/seed-range/gen/sherkala/hi}{68.0}
\@namedef{res@det/aug/seed-range/gen/sherkala/lo}{10.7}
\@namedef{res@det/aug/seed-range/tpr-at-dev/hi}{99.7}
\@namedef{res@det/aug/seed-range/tpr-at-dev/lo}{32.4}
\@namedef{res@det/aug/seed-range/tpr-heldout-at-dev/hi}{84.8}
\@namedef{res@det/aug/seed-range/tpr-heldout-at-dev/lo}{20.1}
\@namedef{res@det/aug/short/100/auroc}{0.995}
\@namedef{res@det/aug/short/100/fpr-at-0.5}{9.6}
\@namedef{res@det/aug/short/100/fpr-at-dev}{2.5}
\@namedef{res@det/aug/short/100/fpr-at-devlen}{2.0}
\@namedef{res@det/aug/short/100/fpr-at-devlen-ci-thr/hi}{4.1}
\@namedef{res@det/aug/short/100/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/aug/short/100/fpr-at-devlen-ci/hi}{3.6}
\@namedef{res@det/aug/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/aug/short/100/thr-devlen}{0.9945}
\@namedef{res@det/aug/short/100/tpr-at-0.5}{99.7}
\@namedef{res@det/aug/short/100/tpr-at-dev}{98.7}
\@namedef{res@det/aug/short/100/tpr-at-devlen}{97.7}
\@namedef{res@det/aug/short/50/auroc}{0.986}
\@namedef{res@det/aug/short/50/fpr-at-0.5}{26.9}
\@namedef{res@det/aug/short/50/fpr-at-dev}{5.6}
\@namedef{res@det/aug/short/50/fpr-at-devlen}{1.5}
\@namedef{res@det/aug/short/50/fpr-at-devlen-ci-thr/hi}{4.1}
\@namedef{res@det/aug/short/50/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/aug/short/50/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@det/aug/short/50/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/aug/short/50/thr-devlen}{0.9956}
\@namedef{res@det/aug/short/50/tpr-at-0.5}{99.5}
\@namedef{res@det/aug/short/50/tpr-at-dev}{95.7}
\@namedef{res@det/aug/short/50/tpr-at-devlen}{79.4}
\@namedef{res@det/aug/thr-dev}{0.9798}
\@namedef{res@det/aug/thr-lenaware/120-160}{0.9961}
\@namedef{res@det/aug/thr-lenaware/160-220}{0.8958}
\@namedef{res@det/aug/thr-lenaware/220-320}{0.2929}
\@namedef{res@det/aug/tpr-at-0.5}{99.9}
\@namedef{res@det/aug/tpr-at-dev}{99.7}
\@namedef{res@det/aug/tpr-at-lenaware}{98.6}
\@namedef{res@det/aug/tpr-heldout-at-0.5}{92.1}
\@namedef{res@det/aug/tpr-heldout-at-dev}{84.6}
\@namedef{res@det/auglen/auroc}{0.996}
\@namedef{res@det/auglen/auroc-by-gen/g31fl}{0.996}
\@namedef{res@det/auglen/auroc-by-gen/g35fl}{0.997}
\@namedef{res@det/auglen/auroc-by-gen/gemma26}{0.996}
\@namedef{res@det/auglen/auroc-by-gen/gemma31}{0.995}
\@namedef{res@det/auglen/auroc-by-gen/gptoss}{0.996}
\@namedef{res@det/auglen/auroc-by-gen/kazllm}{0.943}
\@namedef{res@det/auglen/auroc-by-gen/qwen}{0.997}
\@namedef{res@det/auglen/auroc-by-gen/sherkala}{0.945}
\@namedef{res@det/auglen/auroc-ci/hi}{0.998}
\@namedef{res@det/auglen/auroc-ci/lo}{0.994}
\@namedef{res@det/auglen/auroc-heldout}{0.977}
\@namedef{res@det/auglen/auroc-len120-220}{0.996}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/kazllm}{69.4}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-0.5/sherkala}{82.7}
\@namedef{res@det/auglen/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-dev/g35fl}{99.8}
\@namedef{res@det/auglen/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/auglen/flag-by-gen-at-dev/kazllm}{48.2}
\@namedef{res@det/auglen/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/auglen/flag-by-gen-at-dev/sherkala}{69.3}
\@namedef{res@det/auglen/flag-gray-at-0.5/HP}{39.7}
\@namedef{res@det/auglen/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/auglen/flag-gray-at-0.5/MIX}{95.3}
\@namedef{res@det/auglen/flag-gray-at-0.5/MT}{21.1}
\@namedef{res@det/auglen/flag-gray-at-dev/HP}{15.4}
\@namedef{res@det/auglen/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/auglen/flag-gray-at-dev/MIX}{90.3}
\@namedef{res@det/auglen/flag-gray-at-dev/MT}{9.9}
\@namedef{res@det/auglen/fpr-at-0.5}{5.3}
\@namedef{res@det/auglen/fpr-at-dev}{1.9}
\@namedef{res@det/auglen/fpr-at-dev-ci-thr/hi}{3.2}
\@namedef{res@det/auglen/fpr-at-dev-ci-thr/lo}{0.4}
\@namedef{res@det/auglen/fpr-at-dev-ci/hi}{2.5}
\@namedef{res@det/auglen/fpr-at-dev-ci/lo}{1.2}
\@namedef{res@det/auglen/fpr-at-lenaware}{1.8}
\@namedef{res@det/auglen/fpr-by-domain-at-0.5/encyclopedic}{3.4}
\@namedef{res@det/auglen/fpr-by-domain-at-0.5/essay}{1.4}
\@namedef{res@det/auglen/fpr-by-domain-at-0.5/news}{5.5}
\@namedef{res@det/auglen/fpr-by-domain-at-0.5/web}{8.4}
\@namedef{res@det/auglen/fpr-by-domain-at-dev/encyclopedic}{0.5}
\@namedef{res@det/auglen/fpr-by-domain-at-dev/essay}{0.5}
\@namedef{res@det/auglen/fpr-by-domain-at-dev/news}{2.3}
\@namedef{res@det/auglen/fpr-by-domain-at-dev/web}{3.2}
\@namedef{res@det/auglen/fpr-by-len-at-0.5/120-160}{9.2}
\@namedef{res@det/auglen/fpr-by-len-at-0.5/160-220}{4.5}
\@namedef{res@det/auglen/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/auglen/fpr-by-len-at-dev/120-160}{2.9}
\@namedef{res@det/auglen/fpr-by-len-at-dev/160-220}{1.7}
\@namedef{res@det/auglen/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@det/auglen/fpr-by-len-at-lenaware/120-160}{2.9}
\@namedef{res@det/auglen/fpr-by-len-at-lenaware/160-220}{1.4}
\@namedef{res@det/auglen/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/auglen/script/canon-fpr-at-dev}{1.8}
\@namedef{res@det/auglen/script/canon-tpr-at-dev}{99.7}
\@namedef{res@det/auglen/script/hg-tpr-at-dev}{99.8}
\@namedef{res@det/auglen/script/hg-tpr-orig-at-dev}{99.8}
\@namedef{res@det/auglen/script/hgfold-tpr-at-dev}{99.8}
\@namedef{res@det/auglen/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/auglen/script/hghum-n}{103}
\@namedef{res@det/auglen/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/auglen/script/latin-fpr-at-dev}{0.6}
\@namedef{res@det/auglen/script/latin-tpr-at-dev}{97.2}
\@namedef{res@det/auglen/script/latin2021}{0.997}
\@namedef{res@det/auglen/script/latin2021canon}{0.995}
\@namedef{res@det/auglen/script/trunc100}{0.990}
\@namedef{res@det/auglen/script/trunc50}{0.985}
\@namedef{res@det/auglen/seed-range/fpr-at-dev/hi}{2.2}
\@namedef{res@det/auglen/seed-range/fpr-at-dev/lo}{1.5}
\@namedef{res@det/auglen/seed-range/fpr50-at-dev/hi}{4.8}
\@namedef{res@det/auglen/seed-range/fpr50-at-dev/lo}{1.3}
\@namedef{res@det/auglen/seed-range/gen/g31fl/hi}{100.0}
\@namedef{res@det/auglen/seed-range/gen/g31fl/lo}{71.4}
\@namedef{res@det/auglen/seed-range/gen/g35fl/hi}{99.8}
\@namedef{res@det/auglen/seed-range/gen/g35fl/lo}{79.7}
\@namedef{res@det/auglen/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/auglen/seed-range/gen/gemma26/lo}{71.9}
\@namedef{res@det/auglen/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/auglen/seed-range/gen/gemma31/lo}{65.5}
\@namedef{res@det/auglen/seed-range/gen/gptoss/hi}{99.2}
\@namedef{res@det/auglen/seed-range/gen/gptoss/lo}{79.8}
\@namedef{res@det/auglen/seed-range/gen/kazllm/hi}{55.3}
\@namedef{res@det/auglen/seed-range/gen/kazllm/lo}{32.9}
\@namedef{res@det/auglen/seed-range/gen/qwen/hi}{100.0}
\@namedef{res@det/auglen/seed-range/gen/qwen/lo}{87.2}
\@namedef{res@det/auglen/seed-range/gen/sherkala/hi}{69.3}
\@namedef{res@det/auglen/seed-range/gen/sherkala/lo}{49.3}
\@namedef{res@det/auglen/seed-range/tpr-at-dev/hi}{99.8}
\@namedef{res@det/auglen/seed-range/tpr-at-dev/lo}{77.2}
\@namedef{res@det/auglen/seed-range/tpr-heldout-at-dev/hi}{86.2}
\@namedef{res@det/auglen/seed-range/tpr-heldout-at-dev/lo}{58.1}
\@namedef{res@det/auglen/short/100/auroc}{0.990}
\@namedef{res@det/auglen/short/100/fpr-at-0.5}{9.1}
\@namedef{res@det/auglen/short/100/fpr-at-dev}{2.5}
\@namedef{res@det/auglen/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/auglen/short/100/fpr-at-devlen-ci-thr/hi}{3.8}
\@namedef{res@det/auglen/short/100/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/auglen/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/auglen/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/auglen/short/100/thr-devlen}{0.9904}
\@namedef{res@det/auglen/short/100/tpr-at-0.5}{99.7}
\@namedef{res@det/auglen/short/100/tpr-at-dev}{99.0}
\@namedef{res@det/auglen/short/100/tpr-at-devlen}{94.2}
\@namedef{res@det/auglen/short/50/auroc}{0.985}
\@namedef{res@det/auglen/short/50/fpr-at-0.5}{13.2}
\@namedef{res@det/auglen/short/50/fpr-at-dev}{3.6}
\@namedef{res@det/auglen/short/50/fpr-at-devlen}{1.3}
\@namedef{res@det/auglen/short/50/fpr-at-devlen-ci-thr/hi}{3.6}
\@namedef{res@det/auglen/short/50/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/auglen/short/50/fpr-at-devlen-ci/hi}{2.5}
\@namedef{res@det/auglen/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/auglen/short/50/thr-devlen}{0.9913}
\@namedef{res@det/auglen/short/50/tpr-at-0.5}{98.7}
\@namedef{res@det/auglen/short/50/tpr-at-dev}{94.2}
\@namedef{res@det/auglen/short/50/tpr-at-devlen}{67.3}
\@namedef{res@det/auglen/thr-dev}{0.9784}
\@namedef{res@det/auglen/thr-lenaware/120-160}{0.9730}
\@namedef{res@det/auglen/thr-lenaware/160-220}{0.9811}
\@namedef{res@det/auglen/thr-lenaware/220-320}{0.3831}
\@namedef{res@det/auglen/tpr-at-0.5}{100.0}
\@namedef{res@det/auglen/tpr-at-dev}{99.8}
\@namedef{res@det/auglen/tpr-at-lenaware}{99.8}
\@namedef{res@det/auglen/tpr-heldout-at-0.5}{91.2}
\@namedef{res@det/auglen/tpr-heldout-at-dev}{84.8}
\@namedef{res@det/base/auroc}{0.998}
\@namedef{res@det/base/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/base/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/base/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/base/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/base/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/base/auroc-by-gen/kazllm}{0.966}
\@namedef{res@det/base/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/base/auroc-by-gen/sherkala}{0.953}
\@namedef{res@det/base/auroc-ci/hi}{0.999}
\@namedef{res@det/base/auroc-ci/lo}{0.996}
\@namedef{res@det/base/auroc-heldout}{0.984}
\@namedef{res@det/base/auroc-len120-220}{0.998}
\@namedef{res@det/base/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/kazllm}{85.9}
\@namedef{res@det/base/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/base/flag-by-gen-at-0.5/sherkala}{85.3}
\@namedef{res@det/base/flag-by-gen-at-dev/g31fl}{99.0}
\@namedef{res@det/base/flag-by-gen-at-dev/g35fl}{99.4}
\@namedef{res@det/base/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/base/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/base/flag-by-gen-at-dev/gptoss}{97.6}
\@namedef{res@det/base/flag-by-gen-at-dev/kazllm}{47.1}
\@namedef{res@det/base/flag-by-gen-at-dev/qwen}{96.8}
\@namedef{res@det/base/flag-by-gen-at-dev/sherkala}{62.7}
\@namedef{res@det/base/flag-gray-at-0.5/HP}{50.0}
\@namedef{res@det/base/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/base/flag-gray-at-0.5/MIX}{96.8}
\@namedef{res@det/base/flag-gray-at-0.5/MT}{35.7}
\@namedef{res@det/base/flag-gray-at-dev/HP}{7.7}
\@namedef{res@det/base/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/base/flag-gray-at-dev/MIX}{82.5}
\@namedef{res@det/base/flag-gray-at-dev/MT}{7.9}
\@namedef{res@det/base/fpr-at-0.5}{7.6}
\@namedef{res@det/base/fpr-at-dev}{0.8}
\@namedef{res@det/base/fpr-at-dev-ci-thr/hi}{3.7}
\@namedef{res@det/base/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/base/fpr-at-dev-ci/hi}{1.2}
\@namedef{res@det/base/fpr-at-dev-ci/lo}{0.4}
\@namedef{res@det/base/fpr-at-lenaware}{1.6}
\@namedef{res@det/base/fpr-by-domain-at-0.5/encyclopedic}{6.1}
\@namedef{res@det/base/fpr-by-domain-at-0.5/essay}{4.2}
\@namedef{res@det/base/fpr-by-domain-at-0.5/news}{7.9}
\@namedef{res@det/base/fpr-by-domain-at-0.5/web}{10.3}
\@namedef{res@det/base/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/base/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/base/fpr-by-domain-at-dev/news}{0.9}
\@namedef{res@det/base/fpr-by-domain-at-dev/web}{1.7}
\@namedef{res@det/base/fpr-by-len-at-0.5/120-160}{11.2}
\@namedef{res@det/base/fpr-by-len-at-0.5/160-220}{7.4}
\@namedef{res@det/base/fpr-by-len-at-0.5/220-320}{0.7}
\@namedef{res@det/base/fpr-by-len-at-dev/120-160}{2.0}
\@namedef{res@det/base/fpr-by-len-at-dev/160-220}{0.6}
\@namedef{res@det/base/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/base/fpr-by-len-at-lenaware/120-160}{0.6}
\@namedef{res@det/base/fpr-by-len-at-lenaware/160-220}{2.0}
\@namedef{res@det/base/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/base/script/canon-fpr-at-dev}{0.4}
\@namedef{res@det/base/script/canon-tpr-at-dev}{99.0}
\@namedef{res@det/base/script/hg-tpr-at-dev}{63.3}
\@namedef{res@det/base/script/hg-tpr-orig-at-dev}{99.0}
\@namedef{res@det/base/script/hgfold-tpr-at-dev}{99.0}
\@namedef{res@det/base/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/base/script/hghum-n}{103}
\@namedef{res@det/base/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/base/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/base/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/base/script/latin2021}{0.384}
\@namedef{res@det/base/script/latin2021canon}{0.996}
\@namedef{res@det/base/script/trunc100}{0.991}
\@namedef{res@det/base/script/trunc50}{0.987}
\@namedef{res@det/base/seed-range/fpr-at-dev/hi}{1.5}
\@namedef{res@det/base/seed-range/fpr-at-dev/lo}{0.5}
\@namedef{res@det/base/seed-range/fpr50-at-dev/hi}{2.3}
\@namedef{res@det/base/seed-range/fpr50-at-dev/lo}{0.8}
\@namedef{res@det/base/seed-range/gen/g31fl/hi}{100.0}
\@namedef{res@det/base/seed-range/gen/g31fl/lo}{91.3}
\@namedef{res@det/base/seed-range/gen/g35fl/hi}{100.0}
\@namedef{res@det/base/seed-range/gen/g35fl/lo}{87.4}
\@namedef{res@det/base/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/base/seed-range/gen/gemma26/lo}{89.5}
\@namedef{res@det/base/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/base/seed-range/gen/gemma31/lo}{86.9}
\@namedef{res@det/base/seed-range/gen/gptoss/hi}{99.2}
\@namedef{res@det/base/seed-range/gen/gptoss/lo}{88.7}
\@namedef{res@det/base/seed-range/gen/kazllm/hi}{61.2}
\@namedef{res@det/base/seed-range/gen/kazllm/lo}{11.8}
\@namedef{res@det/base/seed-range/gen/qwen/hi}{99.2}
\@namedef{res@det/base/seed-range/gen/qwen/lo}{90.4}
\@namedef{res@det/base/seed-range/gen/sherkala/hi}{66.7}
\@namedef{res@det/base/seed-range/gen/sherkala/lo}{18.7}
\@namedef{res@det/base/seed-range/tpr-at-dev/hi}{99.8}
\@namedef{res@det/base/seed-range/tpr-at-dev/lo}{89.3}
\@namedef{res@det/base/seed-range/tpr-heldout-at-dev/hi}{86.9}
\@namedef{res@det/base/seed-range/tpr-heldout-at-dev/lo}{61.5}
\@namedef{res@det/base/short/100/auroc}{0.991}
\@namedef{res@det/base/short/100/fpr-at-0.5}{15.5}
\@namedef{res@det/base/short/100/fpr-at-dev}{2.0}
\@namedef{res@det/base/short/100/fpr-at-devlen}{1.5}
\@namedef{res@det/base/short/100/fpr-at-devlen-ci-thr/hi}{4.3}
\@namedef{res@det/base/short/100/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/base/short/100/fpr-at-devlen-ci/hi}{2.8}
\@namedef{res@det/base/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/base/short/100/thr-devlen}{0.9985}
\@namedef{res@det/base/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/base/short/100/tpr-at-dev}{98.0}
\@namedef{res@det/base/short/100/tpr-at-devlen}{95.9}
\@namedef{res@det/base/short/50/auroc}{0.987}
\@namedef{res@det/base/short/50/fpr-at-0.5}{24.4}
\@namedef{res@det/base/short/50/fpr-at-dev}{1.0}
\@namedef{res@det/base/short/50/fpr-at-devlen}{2.3}
\@namedef{res@det/base/short/50/fpr-at-devlen-ci-thr/hi}{4.3}
\@namedef{res@det/base/short/50/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/base/short/50/fpr-at-devlen-ci/hi}{3.8}
\@namedef{res@det/base/short/50/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/base/short/50/thr-devlen}{0.9981}
\@namedef{res@det/base/short/50/tpr-at-0.5}{99.5}
\@namedef{res@det/base/short/50/tpr-at-dev}{67.5}
\@namedef{res@det/base/short/50/tpr-at-devlen}{86.5}
\@namedef{res@det/base/thr-dev}{0.9984}
\@namedef{res@det/base/thr-lenaware/120-160}{0.9987}
\@namedef{res@det/base/thr-lenaware/160-220}{0.9968}
\@namedef{res@det/base/thr-lenaware/220-320}{0.5685}
\@namedef{res@det/base/tpr-at-0.5}{100.0}
\@namedef{res@det/base/tpr-at-dev}{98.8}
\@namedef{res@det/base/tpr-at-lenaware}{76.1}
\@namedef{res@det/base/tpr-heldout-at-0.5}{94.8}
\@namedef{res@det/base/tpr-heldout-at-dev}{83.5}
\@namedef{res@det/combo-all+bino/auroc}{0.995}
\@namedef{res@det/combo-all+bino/auroc-by-gen/g31fl}{0.995}
\@namedef{res@det/combo-all+bino/auroc-by-gen/g35fl}{0.994}
\@namedef{res@det/combo-all+bino/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/combo-all+bino/auroc-by-gen/gemma31}{0.997}
\@namedef{res@det/combo-all+bino/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/combo-all+bino/auroc-by-gen/kazllm}{0.971}
\@namedef{res@det/combo-all+bino/auroc-by-gen/qwen}{0.996}
\@namedef{res@det/combo-all+bino/auroc-by-gen/sherkala}{0.979}
\@namedef{res@det/combo-all+bino/auroc-ci/hi}{0.997}
\@namedef{res@det/combo-all+bino/auroc-ci/lo}{0.992}
\@namedef{res@det/combo-all+bino/auroc-heldout}{0.989}
\@namedef{res@det/combo-all+bino/auroc-len120-220}{0.995}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/g31fl}{75.1}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/g35fl}{69.5}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/gemma26}{93.9}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/gemma31}{87.5}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/gptoss}{98.4}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/kazllm}{42.4}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/qwen}{75.2}
\@namedef{res@det/combo-all+bino/flag-by-gen-at-dev/sherkala}{66.7}
\@namedef{res@det/combo-all+bino/flag-gray-at-dev/HP}{3.8}
\@namedef{res@det/combo-all+bino/flag-gray-at-dev/MH}{43.8}
\@namedef{res@det/combo-all+bino/flag-gray-at-dev/MIX}{42.5}
\@namedef{res@det/combo-all+bino/flag-gray-at-dev/MT}{5.3}
\@namedef{res@det/combo-all+bino/fpr-at-dev}{0.5}
\@namedef{res@det/combo-all+bino/fpr-at-dev-ci-thr/hi}{1.8}
\@namedef{res@det/combo-all+bino/fpr-at-dev-ci-thr/lo}{0.2}
\@namedef{res@det/combo-all+bino/fpr-at-dev-ci/hi}{0.9}
\@namedef{res@det/combo-all+bino/fpr-at-dev-ci/lo}{0.2}
\@namedef{res@det/combo-all+bino/fpr-at-lenaware}{0.8}
\@namedef{res@det/combo-all+bino/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/combo-all+bino/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/combo-all+bino/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/combo-all+bino/fpr-by-domain-at-dev/web}{0.9}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-dev/120-160}{0.6}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-dev/160-220}{0.6}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-lenaware/120-160}{1.1}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-lenaware/160-220}{0.6}
\@namedef{res@det/combo-all+bino/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/combo-all+bino/script/canon-fpr-at-dev}{0.4}
\@namedef{res@det/combo-all+bino/script/canon-tpr-at-dev}{78.6}
\@namedef{res@det/combo-all+bino/script/hg-tpr-at-dev}{57.0}
\@namedef{res@det/combo-all+bino/script/hg-tpr-orig-at-dev}{78.0}
\@namedef{res@det/combo-all+bino/script/hgfold-tpr-at-dev}{77.5}
\@namedef{res@det/combo-all+bino/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/combo-all+bino/script/hghum-n}{103}
\@namedef{res@det/combo-all+bino/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/combo-all+bino/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/combo-all+bino/script/latin-tpr-at-dev}{5.0}
\@namedef{res@det/combo-all+bino/script/latin2021}{0.996}
\@namedef{res@det/combo-all+bino/script/latin2021canon}{0.996}
\@namedef{res@det/combo-all+bino/script/trunc100}{0.990}
\@namedef{res@det/combo-all+bino/script/trunc50}{0.939}
\@namedef{res@det/combo-all+bino/short/100/auroc}{0.990}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-dev}{0.8}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-devlen}{1.0}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-devlen-ci-thr/hi}{6.1}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@det/combo-all+bino/short/100/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/combo-all+bino/short/100/thr-devlen}{0.9949}
\@namedef{res@det/combo-all+bino/short/100/tpr-at-dev}{61.9}
\@namedef{res@det/combo-all+bino/short/100/tpr-at-devlen}{68.3}
\@namedef{res@det/combo-all+bino/short/50/auroc}{0.939}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-devlen-ci-thr/hi}{5.1}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/combo-all+bino/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/combo-all+bino/short/50/thr-devlen}{0.9977}
\@namedef{res@det/combo-all+bino/short/50/tpr-at-dev}{40.4}
\@namedef{res@det/combo-all+bino/short/50/tpr-at-devlen}{36.5}
\@namedef{res@det/combo-all+bino/thr-dev}{0.9951}
\@namedef{res@det/combo-all+bino/thr-lenaware/120-160}{0.9938}
\@namedef{res@det/combo-all+bino/thr-lenaware/160-220}{0.9960}
\@namedef{res@det/combo-all+bino/thr-lenaware/220-320}{0.9639}
\@namedef{res@det/combo-all+bino/tpr-at-dev}{75.1}
\@namedef{res@det/combo-all+bino/tpr-at-lenaware}{80.2}
\@namedef{res@det/combo-all+bino/tpr-heldout-at-dev}{76.9}
\@namedef{res@det/combo-alllen+bino/auroc}{0.996}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/g31fl}{0.997}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/g35fl}{0.995}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/kazllm}{0.976}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/qwen}{0.997}
\@namedef{res@det/combo-alllen+bino/auroc-by-gen/sherkala}{0.973}
\@namedef{res@det/combo-alllen+bino/auroc-ci/hi}{0.998}
\@namedef{res@det/combo-alllen+bino/auroc-ci/lo}{0.994}
\@namedef{res@det/combo-alllen+bino/auroc-heldout}{0.989}
\@namedef{res@det/combo-alllen+bino/auroc-len120-220}{0.996}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/g31fl}{92.4}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/g35fl}{87.4}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/gemma26}{96.5}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/gemma31}{96.4}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/kazllm}{58.8}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/qwen}{92.0}
\@namedef{res@det/combo-alllen+bino/flag-by-gen-at-dev/sherkala}{74.7}
\@namedef{res@det/combo-alllen+bino/flag-gray-at-dev/HP}{5.1}
\@namedef{res@det/combo-alllen+bino/flag-gray-at-dev/MH}{90.6}
\@namedef{res@det/combo-alllen+bino/flag-gray-at-dev/MIX}{52.3}
\@namedef{res@det/combo-alllen+bino/flag-gray-at-dev/MT}{8.5}
\@namedef{res@det/combo-alllen+bino/fpr-at-dev}{0.6}
\@namedef{res@det/combo-alllen+bino/fpr-at-dev-ci-thr/hi}{1.7}
\@namedef{res@det/combo-alllen+bino/fpr-at-dev-ci-thr/lo}{0.2}
\@namedef{res@det/combo-alllen+bino/fpr-at-dev-ci/hi}{1.0}
\@namedef{res@det/combo-alllen+bino/fpr-at-dev-ci/lo}{0.3}
\@namedef{res@det/combo-alllen+bino/fpr-at-lenaware}{1.2}
\@namedef{res@det/combo-alllen+bino/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/combo-alllen+bino/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/combo-alllen+bino/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/combo-alllen+bino/fpr-by-domain-at-dev/web}{1.1}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-dev/120-160}{1.1}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-dev/160-220}{0.5}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-lenaware/120-160}{2.9}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-lenaware/160-220}{0.5}
\@namedef{res@det/combo-alllen+bino/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/combo-alllen+bino/script/canon-fpr-at-dev}{0.8}
\@namedef{res@det/combo-alllen+bino/script/canon-tpr-at-dev}{91.7}
\@namedef{res@det/combo-alllen+bino/script/hg-tpr-at-dev}{91.0}
\@namedef{res@det/combo-alllen+bino/script/hg-tpr-orig-at-dev}{91.0}
\@namedef{res@det/combo-alllen+bino/script/hgfold-tpr-at-dev}{91.2}
\@namedef{res@det/combo-alllen+bino/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/combo-alllen+bino/script/hghum-n}{103}
\@namedef{res@det/combo-alllen+bino/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/combo-alllen+bino/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/combo-alllen+bino/script/latin-tpr-at-dev}{79.9}
\@namedef{res@det/combo-alllen+bino/script/latin2021}{0.998}
\@namedef{res@det/combo-alllen+bino/script/latin2021canon}{0.995}
\@namedef{res@det/combo-alllen+bino/script/trunc100}{0.994}
\@namedef{res@det/combo-alllen+bino/script/trunc50}{0.975}
\@namedef{res@det/combo-alllen+bino/short/100/auroc}{0.994}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-dev}{0.8}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-devlen}{1.3}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-devlen-ci-thr/hi}{5.1}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-devlen-ci/hi}{2.5}
\@namedef{res@det/combo-alllen+bino/short/100/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/combo-alllen+bino/short/100/thr-devlen}{0.9949}
\@namedef{res@det/combo-alllen+bino/short/100/tpr-at-dev}{77.9}
\@namedef{res@det/combo-alllen+bino/short/100/tpr-at-devlen}{84.5}
\@namedef{res@det/combo-alllen+bino/short/50/auroc}{0.975}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-devlen-ci-thr/hi}{6.1}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-devlen-ci-thr/lo}{0.2}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/combo-alllen+bino/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/combo-alllen+bino/short/50/thr-devlen}{0.9977}
\@namedef{res@det/combo-alllen+bino/short/50/tpr-at-dev}{51.0}
\@namedef{res@det/combo-alllen+bino/short/50/tpr-at-devlen}{36.5}
\@namedef{res@det/combo-alllen+bino/thr-dev}{0.9951}
\@namedef{res@det/combo-alllen+bino/thr-lenaware/120-160}{0.9868}
\@namedef{res@det/combo-alllen+bino/thr-lenaware/160-220}{0.9974}
\@namedef{res@det/combo-alllen+bino/thr-lenaware/220-320}{0.9639}
\@namedef{res@det/combo-alllen+bino/tpr-at-dev}{91.0}
\@namedef{res@det/combo-alllen+bino/tpr-at-lenaware}{98.6}
\@namedef{res@det/combo-alllen+bino/tpr-heldout-at-dev}{85.5}
\@namedef{res@det/combo-aug+bino/auroc}{0.997}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/g35fl}{0.997}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/kazllm}{0.966}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/combo-aug+bino/auroc-by-gen/sherkala}{0.969}
\@namedef{res@det/combo-aug+bino/auroc-ci/hi}{0.999}
\@namedef{res@det/combo-aug+bino/auroc-ci/lo}{0.996}
\@namedef{res@det/combo-aug+bino/auroc-heldout}{0.987}
\@namedef{res@det/combo-aug+bino/auroc-len120-220}{0.997}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/g31fl}{87.3}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/g35fl}{81.0}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/gemma26}{96.5}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/gemma31}{92.9}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/kazllm}{48.2}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/qwen}{95.2}
\@namedef{res@det/combo-aug+bino/flag-by-gen-at-dev/sherkala}{72.0}
\@namedef{res@det/combo-aug+bino/flag-gray-at-dev/HP}{3.8}
\@namedef{res@det/combo-aug+bino/flag-gray-at-dev/MH}{84.4}
\@namedef{res@det/combo-aug+bino/flag-gray-at-dev/MIX}{63.9}
\@namedef{res@det/combo-aug+bino/flag-gray-at-dev/MT}{5.3}
\@namedef{res@det/combo-aug+bino/fpr-at-dev}{0.4}
\@namedef{res@det/combo-aug+bino/fpr-at-dev-ci-thr/hi}{1.9}
\@namedef{res@det/combo-aug+bino/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/combo-aug+bino/fpr-at-dev-ci/hi}{0.7}
\@namedef{res@det/combo-aug+bino/fpr-at-dev-ci/lo}{0.1}
\@namedef{res@det/combo-aug+bino/fpr-at-lenaware}{1.0}
\@namedef{res@det/combo-aug+bino/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/combo-aug+bino/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/combo-aug+bino/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/combo-aug+bino/fpr-by-domain-at-dev/web}{0.4}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-dev/120-160}{0.3}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-dev/160-220}{0.5}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-lenaware/120-160}{1.1}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-lenaware/160-220}{0.5}
\@namedef{res@det/combo-aug+bino/fpr-by-len-at-lenaware/220-320}{4.2}
\@namedef{res@det/combo-aug+bino/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/combo-aug+bino/script/canon-tpr-at-dev}{82.2}
\@namedef{res@det/combo-aug+bino/script/hg-tpr-at-dev}{94.1}
\@namedef{res@det/combo-aug+bino/script/hg-tpr-orig-at-dev}{85.8}
\@namedef{res@det/combo-aug+bino/script/hgfold-tpr-at-dev}{85.8}
\@namedef{res@det/combo-aug+bino/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/combo-aug+bino/script/hghum-n}{103}
\@namedef{res@det/combo-aug+bino/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/combo-aug+bino/script/latin-fpr-at-dev}{0.2}
\@namedef{res@det/combo-aug+bino/script/latin-tpr-at-dev}{88.7}
\@namedef{res@det/combo-aug+bino/script/latin2021}{0.998}
\@namedef{res@det/combo-aug+bino/script/latin2021canon}{0.996}
\@namedef{res@det/combo-aug+bino/script/trunc100}{0.996}
\@namedef{res@det/combo-aug+bino/script/trunc50}{0.975}
\@namedef{res@det/combo-aug+bino/short/100/auroc}{0.996}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-dev}{0.3}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-devlen}{1.0}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-devlen-ci-thr/hi}{4.6}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-devlen-ci/hi}{2.3}
\@namedef{res@det/combo-aug+bino/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/combo-aug+bino/short/100/thr-devlen}{0.9949}
\@namedef{res@det/combo-aug+bino/short/100/tpr-at-dev}{77.2}
\@namedef{res@det/combo-aug+bino/short/100/tpr-at-devlen}{88.8}
\@namedef{res@det/combo-aug+bino/short/50/auroc}{0.975}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-devlen-ci-thr/hi}{9.4}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/combo-aug+bino/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/combo-aug+bino/short/50/thr-devlen}{0.9977}
\@namedef{res@det/combo-aug+bino/short/50/tpr-at-dev}{46.2}
\@namedef{res@det/combo-aug+bino/short/50/tpr-at-devlen}{39.6}
\@namedef{res@det/combo-aug+bino/thr-dev}{0.9951}
\@namedef{res@det/combo-aug+bino/thr-lenaware/120-160}{0.9938}
\@namedef{res@det/combo-aug+bino/thr-lenaware/160-220}{0.9960}
\@namedef{res@det/combo-aug+bino/thr-lenaware/220-320}{0.9639}
\@namedef{res@det/combo-aug+bino/tpr-at-dev}{86.7}
\@namedef{res@det/combo-aug+bino/tpr-at-lenaware}{95.2}
\@namedef{res@det/combo-aug+bino/tpr-heldout-at-dev}{81.7}
\@namedef{res@det/combo-auglen+bino/auroc}{0.994}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/g31fl}{0.994}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/g35fl}{0.993}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/gemma26}{0.997}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/gemma31}{0.996}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/kazllm}{0.962}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/qwen}{0.996}
\@namedef{res@det/combo-auglen+bino/auroc-by-gen/sherkala}{0.968}
\@namedef{res@det/combo-auglen+bino/auroc-ci/hi}{0.997}
\@namedef{res@det/combo-auglen+bino/auroc-ci/lo}{0.991}
\@namedef{res@det/combo-auglen+bino/auroc-heldout}{0.985}
\@namedef{res@det/combo-auglen+bino/auroc-len120-220}{0.994}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/g31fl}{81.9}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/g35fl}{83.5}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/gemma26}{95.6}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/gemma31}{91.1}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/kazllm}{57.6}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/qwen}{96.0}
\@namedef{res@det/combo-auglen+bino/flag-by-gen-at-dev/sherkala}{76.0}
\@namedef{res@det/combo-auglen+bino/flag-gray-at-dev/HP}{9.0}
\@namedef{res@det/combo-auglen+bino/flag-gray-at-dev/MH}{92.2}
\@namedef{res@det/combo-auglen+bino/flag-gray-at-dev/MIX}{84.1}
\@namedef{res@det/combo-auglen+bino/flag-gray-at-dev/MT}{8.8}
\@namedef{res@det/combo-auglen+bino/fpr-at-dev}{0.9}
\@namedef{res@det/combo-auglen+bino/fpr-at-dev-ci-thr/hi}{2.7}
\@namedef{res@det/combo-auglen+bino/fpr-at-dev-ci-thr/lo}{0.4}
\@namedef{res@det/combo-auglen+bino/fpr-at-dev-ci/hi}{1.4}
\@namedef{res@det/combo-auglen+bino/fpr-at-dev-ci/lo}{0.5}
\@namedef{res@det/combo-auglen+bino/fpr-at-lenaware}{1.6}
\@namedef{res@det/combo-auglen+bino/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/combo-auglen+bino/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/combo-auglen+bino/fpr-by-domain-at-dev/news}{0.9}
\@namedef{res@det/combo-auglen+bino/fpr-by-domain-at-dev/web}{1.5}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-dev/120-160}{1.4}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-dev/160-220}{0.8}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-lenaware/120-160}{3.7}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-lenaware/160-220}{0.8}
\@namedef{res@det/combo-auglen+bino/fpr-by-len-at-lenaware/220-320}{2.8}
\@namedef{res@det/combo-auglen+bino/script/canon-fpr-at-dev}{1.0}
\@namedef{res@det/combo-auglen+bino/script/canon-tpr-at-dev}{85.2}
\@namedef{res@det/combo-auglen+bino/script/hg-tpr-at-dev}{92.9}
\@namedef{res@det/combo-auglen+bino/script/hg-tpr-orig-at-dev}{84.6}
\@namedef{res@det/combo-auglen+bino/script/hgfold-tpr-at-dev}{84.4}
\@namedef{res@det/combo-auglen+bino/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/combo-auglen+bino/script/hghum-n}{103}
\@namedef{res@det/combo-auglen+bino/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/combo-auglen+bino/script/latin-fpr-at-dev}{0.4}
\@namedef{res@det/combo-auglen+bino/script/latin-tpr-at-dev}{92.5}
\@namedef{res@det/combo-auglen+bino/script/latin2021}{0.998}
\@namedef{res@det/combo-auglen+bino/script/latin2021canon}{0.993}
\@namedef{res@det/combo-auglen+bino/script/trunc100}{0.992}
\@namedef{res@det/combo-auglen+bino/script/trunc50}{0.978}
\@namedef{res@det/combo-auglen+bino/short/100/auroc}{0.992}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-dev}{1.8}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-devlen-ci-thr/hi}{3.8}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/combo-auglen+bino/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/combo-auglen+bino/short/100/thr-devlen}{0.9974}
\@namedef{res@det/combo-auglen+bino/short/100/tpr-at-dev}{85.8}
\@namedef{res@det/combo-auglen+bino/short/100/tpr-at-devlen}{85.8}
\@namedef{res@det/combo-auglen+bino/short/50/auroc}{0.978}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-dev}{1.5}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-devlen}{1.0}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-devlen-ci-thr/hi}{6.3}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-devlen-ci/hi}{2.3}
\@namedef{res@det/combo-auglen+bino/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/combo-auglen+bino/short/50/thr-devlen}{1.0000}
\@namedef{res@det/combo-auglen+bino/short/50/tpr-at-dev}{69.5}
\@namedef{res@det/combo-auglen+bino/short/50/tpr-at-devlen}{41.1}
\@namedef{res@det/combo-auglen+bino/thr-dev}{0.9951}
\@namedef{res@det/combo-auglen+bino/thr-lenaware/120-160}{0.9882}
\@namedef{res@det/combo-auglen+bino/thr-lenaware/160-220}{0.9960}
\@namedef{res@det/combo-auglen+bino/thr-lenaware/220-320}{0.9639}
\@namedef{res@det/combo-auglen+bino/tpr-at-dev}{85.6}
\@namedef{res@det/combo-auglen+bino/tpr-at-lenaware}{96.5}
\@namedef{res@det/combo-auglen+bino/tpr-heldout-at-dev}{83.3}
\@namedef{res@det/combo-base+bino/auroc}{0.995}
\@namedef{res@det/combo-base+bino/auroc-by-gen/g31fl}{0.995}
\@namedef{res@det/combo-base+bino/auroc-by-gen/g35fl}{0.995}
\@namedef{res@det/combo-base+bino/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/combo-base+bino/auroc-by-gen/gemma31}{0.997}
\@namedef{res@det/combo-base+bino/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/combo-base+bino/auroc-by-gen/kazllm}{0.969}
\@namedef{res@det/combo-base+bino/auroc-by-gen/qwen}{0.997}
\@namedef{res@det/combo-base+bino/auroc-by-gen/sherkala}{0.968}
\@namedef{res@det/combo-base+bino/auroc-ci/hi}{0.998}
\@namedef{res@det/combo-base+bino/auroc-ci/lo}{0.993}
\@namedef{res@det/combo-base+bino/auroc-heldout}{0.987}
\@namedef{res@det/combo-base+bino/auroc-len120-220}{0.996}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/g31fl}{75.9}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/g35fl}{67.0}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/gemma26}{94.7}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/gemma31}{90.5}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/kazllm}{48.2}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/qwen}{89.6}
\@namedef{res@det/combo-base+bino/flag-by-gen-at-dev/sherkala}{66.7}
\@namedef{res@det/combo-base+bino/flag-gray-at-dev/HP}{6.4}
\@namedef{res@det/combo-base+bino/flag-gray-at-dev/MH}{71.9}
\@namedef{res@det/combo-base+bino/flag-gray-at-dev/MIX}{67.3}
\@namedef{res@det/combo-base+bino/flag-gray-at-dev/MT}{7.0}
\@namedef{res@det/combo-base+bino/fpr-at-dev}{0.5}
\@namedef{res@det/combo-base+bino/fpr-at-dev-ci-thr/hi}{2.9}
\@namedef{res@det/combo-base+bino/fpr-at-dev-ci-thr/lo}{0.2}
\@namedef{res@det/combo-base+bino/fpr-at-dev-ci/hi}{0.8}
\@namedef{res@det/combo-base+bino/fpr-at-dev-ci/lo}{0.2}
\@namedef{res@det/combo-base+bino/fpr-at-lenaware}{0.8}
\@namedef{res@det/combo-base+bino/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/combo-base+bino/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/combo-base+bino/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/combo-base+bino/fpr-by-domain-at-dev/web}{0.9}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-dev/120-160}{0.9}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-dev/160-220}{0.5}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-lenaware/120-160}{0.9}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-lenaware/160-220}{0.5}
\@namedef{res@det/combo-base+bino/fpr-by-len-at-lenaware/220-320}{2.8}
\@namedef{res@det/combo-base+bino/script/canon-fpr-at-dev}{0.8}
\@namedef{res@det/combo-base+bino/script/canon-tpr-at-dev}{73.4}
\@namedef{res@det/combo-base+bino/script/hg-tpr-at-dev}{22.5}
\@namedef{res@det/combo-base+bino/script/hg-tpr-orig-at-dev}{78.7}
\@namedef{res@det/combo-base+bino/script/hgfold-tpr-at-dev}{77.8}
\@namedef{res@det/combo-base+bino/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/combo-base+bino/script/hghum-n}{103}
\@namedef{res@det/combo-base+bino/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/combo-base+bino/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/combo-base+bino/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/combo-base+bino/script/latin2021}{0.359}
\@namedef{res@det/combo-base+bino/script/latin2021canon}{0.994}
\@namedef{res@det/combo-base+bino/script/trunc100}{0.991}
\@namedef{res@det/combo-base+bino/script/trunc50}{0.973}
\@namedef{res@det/combo-base+bino/short/100/auroc}{0.991}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-dev}{1.0}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-devlen}{1.5}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-devlen-ci-thr/hi}{5.1}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-devlen-ci/hi}{2.8}
\@namedef{res@det/combo-base+bino/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/combo-base+bino/short/100/thr-devlen}{0.9949}
\@namedef{res@det/combo-base+bino/short/100/tpr-at-dev}{75.4}
\@namedef{res@det/combo-base+bino/short/100/tpr-at-devlen}{81.2}
\@namedef{res@det/combo-base+bino/short/50/auroc}{0.973}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-devlen-ci-thr/hi}{7.9}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/combo-base+bino/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/combo-base+bino/short/50/thr-devlen}{0.9977}
\@namedef{res@det/combo-base+bino/short/50/tpr-at-dev}{41.4}
\@namedef{res@det/combo-base+bino/short/50/tpr-at-devlen}{36.5}
\@namedef{res@det/combo-base+bino/thr-dev}{0.9951}
\@namedef{res@det/combo-base+bino/thr-lenaware/120-160}{0.9956}
\@namedef{res@det/combo-base+bino/thr-lenaware/160-220}{0.9960}
\@namedef{res@det/combo-base+bino/thr-lenaware/220-320}{0.9669}
\@namedef{res@det/combo-base+bino/tpr-at-dev}{75.9}
\@namedef{res@det/combo-base+bino/tpr-at-lenaware}{76.8}
\@namedef{res@det/combo-base+bino/tpr-heldout-at-dev}{79.4}
\@namedef{res@det/complement/aug/bino-catches}{44.1}
\@namedef{res@det/complement/aug/n-kz}{160}
\@namedef{res@det/complement/aug/n-missed}{68}
\@namedef{res@det/complement/auglen/bino-catches}{44.8}
\@namedef{res@det/complement/auglen/n-kz}{160}
\@namedef{res@det/complement/auglen/n-missed}{67}
\@namedef{res@det/complement/base/bino-catches}{43.8}
\@namedef{res@det/complement/base/n-kz}{160}
\@namedef{res@det/complement/base/n-missed}{73}
\@namedef{res@det/kz/auroc}{0.998}
\@namedef{res@det/kz/auroc-by-gen/g31fl}{0.999}
\@namedef{res@det/kz/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/kz/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/kz/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/kz/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/kz/auroc-by-gen/kazllm}{0.965}
\@namedef{res@det/kz/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/kz/auroc-by-gen/sherkala}{0.973}
\@namedef{res@det/kz/auroc-ci/hi}{0.999}
\@namedef{res@det/kz/auroc-ci/lo}{0.997}
\@namedef{res@det/kz/auroc-heldout}{0.987}
\@namedef{res@det/kz/auroc-len120-220}{0.998}
\@namedef{res@det/kz/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/kazllm}{90.6}
\@namedef{res@det/kz/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-0.5/sherkala}{92.0}
\@namedef{res@det/kz/flag-by-gen-at-dev/g31fl}{99.8}
\@namedef{res@det/kz/flag-by-gen-at-dev/g35fl}{99.4}
\@namedef{res@det/kz/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/kz/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/kz/flag-by-gen-at-dev/kazllm}{57.6}
\@namedef{res@det/kz/flag-by-gen-at-dev/qwen}{98.4}
\@namedef{res@det/kz/flag-by-gen-at-dev/sherkala}{65.3}
\@namedef{res@det/kz/flag-gray-at-0.5/HP}{62.8}
\@namedef{res@det/kz/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/kz/flag-gray-at-0.5/MIX}{96.5}
\@namedef{res@det/kz/flag-gray-at-0.5/MT}{50.0}
\@namedef{res@det/kz/flag-gray-at-dev/HP}{9.0}
\@namedef{res@det/kz/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/kz/flag-gray-at-dev/MIX}{70.2}
\@namedef{res@det/kz/flag-gray-at-dev/MT}{8.8}
\@namedef{res@det/kz/fpr-at-0.5}{12.6}
\@namedef{res@det/kz/fpr-at-dev}{1.2}
\@namedef{res@det/kz/fpr-at-dev-ci-thr/hi}{3.3}
\@namedef{res@det/kz/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/kz/fpr-at-dev-ci/hi}{1.8}
\@namedef{res@det/kz/fpr-at-dev-ci/lo}{0.7}
\@namedef{res@det/kz/fpr-at-lenaware}{1.1}
\@namedef{res@det/kz/fpr-by-domain-at-0.5/encyclopedic}{10.0}
\@namedef{res@det/kz/fpr-by-domain-at-0.5/essay}{4.2}
\@namedef{res@det/kz/fpr-by-domain-at-0.5/news}{13.6}
\@namedef{res@det/kz/fpr-by-domain-at-0.5/web}{17.6}
\@namedef{res@det/kz/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/kz/fpr-by-domain-at-dev/essay}{0.5}
\@namedef{res@det/kz/fpr-by-domain-at-dev/news}{1.1}
\@namedef{res@det/kz/fpr-by-domain-at-dev/web}{2.8}
\@namedef{res@det/kz/fpr-by-len-at-0.5/120-160}{23.8}
\@namedef{res@det/kz/fpr-by-len-at-0.5/160-220}{10.4}
\@namedef{res@det/kz/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/kz/fpr-by-len-at-dev/120-160}{2.9}
\@namedef{res@det/kz/fpr-by-len-at-dev/160-220}{0.9}
\@namedef{res@det/kz/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/kz/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@det/kz/fpr-by-len-at-lenaware/160-220}{0.9}
\@namedef{res@det/kz/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/kz/script/canon-fpr-at-dev}{1.0}
\@namedef{res@det/kz/script/canon-tpr-at-dev}{98.7}
\@namedef{res@det/kz/script/hg-tpr-at-dev}{99.8}
\@namedef{res@det/kz/script/hg-tpr-orig-at-dev}{99.5}
\@namedef{res@det/kz/script/hgfold-tpr-at-dev}{99.5}
\@namedef{res@det/kz/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/kz/script/hghum-n}{103}
\@namedef{res@det/kz/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/kz/script/latin-fpr-at-dev}{0.6}
\@namedef{res@det/kz/script/latin-tpr-at-dev}{89.4}
\@namedef{res@det/kz/script/latin2021}{0.997}
\@namedef{res@det/kz/script/latin2021canon}{0.997}
\@namedef{res@det/kz/script/trunc100}{0.988}
\@namedef{res@det/kz/script/trunc50}{0.951}
\@namedef{res@det/kz/seed-range/fpr-at-dev/hi}{1.2}
\@namedef{res@det/kz/seed-range/fpr-at-dev/lo}{0.7}
\@namedef{res@det/kz/seed-range/fpr50-at-dev/hi}{6.1}
\@namedef{res@det/kz/seed-range/fpr50-at-dev/lo}{0.0}
\@namedef{res@det/kz/seed-range/gen/g31fl/hi}{99.8}
\@namedef{res@det/kz/seed-range/gen/g31fl/lo}{95.6}
\@namedef{res@det/kz/seed-range/gen/g35fl/hi}{99.0}
\@namedef{res@det/kz/seed-range/gen/g35fl/lo}{88.9}
\@namedef{res@det/kz/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/kz/seed-range/gen/gemma26/lo}{91.2}
\@namedef{res@det/kz/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/kz/seed-range/gen/gemma31/lo}{91.1}
\@namedef{res@det/kz/seed-range/gen/gptoss/hi}{98.4}
\@namedef{res@det/kz/seed-range/gen/gptoss/lo}{85.5}
\@namedef{res@det/kz/seed-range/gen/kazllm/hi}{63.5}
\@namedef{res@det/kz/seed-range/gen/kazllm/lo}{23.5}
\@namedef{res@det/kz/seed-range/gen/qwen/hi}{100.0}
\@namedef{res@det/kz/seed-range/gen/qwen/lo}{96.0}
\@namedef{res@det/kz/seed-range/gen/sherkala/hi}{80.0}
\@namedef{res@det/kz/seed-range/gen/sherkala/lo}{36.0}
\@namedef{res@det/kz/seed-range/tpr-at-dev/hi}{99.1}
\@namedef{res@det/kz/seed-range/tpr-at-dev/lo}{91.9}
\@namedef{res@det/kz/seed-range/tpr-heldout-at-dev/hi}{89.6}
\@namedef{res@det/kz/seed-range/tpr-heldout-at-dev/lo}{68.8}
\@namedef{res@det/kz/short/100/auroc}{0.988}
\@namedef{res@det/kz/short/100/fpr-at-0.5}{40.4}
\@namedef{res@det/kz/short/100/fpr-at-dev}{4.6}
\@namedef{res@det/kz/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/kz/short/100/fpr-at-devlen-ci-thr/hi}{4.3}
\@namedef{res@det/kz/short/100/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/kz/short/100/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@det/kz/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/kz/short/100/thr-devlen}{0.9970}
\@namedef{res@det/kz/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/kz/short/100/tpr-at-dev}{99.2}
\@namedef{res@det/kz/short/100/tpr-at-devlen}{91.4}
\@namedef{res@det/kz/short/50/auroc}{0.951}
\@namedef{res@det/kz/short/50/fpr-at-0.5}{82.2}
\@namedef{res@det/kz/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/kz/short/50/fpr-at-devlen}{1.0}
\@namedef{res@det/kz/short/50/fpr-at-devlen-ci-thr/hi}{4.3}
\@namedef{res@det/kz/short/50/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/kz/short/50/fpr-at-devlen-ci/hi}{2.3}
\@namedef{res@det/kz/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/kz/short/50/thr-devlen}{0.9963}
\@namedef{res@det/kz/short/50/tpr-at-0.5}{100.0}
\@namedef{res@det/kz/short/50/tpr-at-dev}{23.4}
\@namedef{res@det/kz/short/50/tpr-at-devlen}{33.8}
\@namedef{res@det/kz/thr-dev}{0.9965}
\@namedef{res@det/kz/thr-lenaware/120-160}{0.9970}
\@namedef{res@det/kz/thr-lenaware/160-220}{0.9961}
\@namedef{res@det/kz/thr-lenaware/220-320}{0.3998}
\@namedef{res@det/kz/tpr-at-0.5}{100.0}
\@namedef{res@det/kz/tpr-at-dev}{99.5}
\@namedef{res@det/kz/tpr-at-lenaware}{99.2}
\@namedef{res@det/kz/tpr-heldout-at-0.5}{96.8}
\@namedef{res@det/kz/tpr-heldout-at-dev}{86.0}
\@namedef{res@det/kzlen/auroc}{0.993}
\@namedef{res@det/kzlen/auroc-by-gen/g31fl}{0.993}
\@namedef{res@det/kzlen/auroc-by-gen/g35fl}{0.994}
\@namedef{res@det/kzlen/auroc-by-gen/gemma26}{0.991}
\@namedef{res@det/kzlen/auroc-by-gen/gemma31}{0.991}
\@namedef{res@det/kzlen/auroc-by-gen/gptoss}{0.992}
\@namedef{res@det/kzlen/auroc-by-gen/kazllm}{0.969}
\@namedef{res@det/kzlen/auroc-by-gen/qwen}{0.992}
\@namedef{res@det/kzlen/auroc-by-gen/sherkala}{0.949}
\@namedef{res@det/kzlen/auroc-ci/hi}{0.996}
\@namedef{res@det/kzlen/auroc-ci/lo}{0.990}
\@namedef{res@det/kzlen/auroc-heldout}{0.980}
\@namedef{res@det/kzlen/auroc-len120-220}{0.993}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/kazllm}{94.1}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/kzlen/flag-by-gen-at-0.5/sherkala}{88.0}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/g31fl}{60.6}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/g35fl}{72.4}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/gemma26}{58.8}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/gemma31}{49.4}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/gptoss}{54.8}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/kazllm}{36.5}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/qwen}{50.4}
\@namedef{res@det/kzlen/flag-by-gen-at-dev/sherkala}{40.0}
\@namedef{res@det/kzlen/flag-gray-at-0.5/HP}{56.4}
\@namedef{res@det/kzlen/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/kzlen/flag-gray-at-0.5/MIX}{97.1}
\@namedef{res@det/kzlen/flag-gray-at-0.5/MT}{44.2}
\@namedef{res@det/kzlen/flag-gray-at-dev/HP}{6.4}
\@namedef{res@det/kzlen/flag-gray-at-dev/MH}{82.8}
\@namedef{res@det/kzlen/flag-gray-at-dev/MIX}{62.0}
\@namedef{res@det/kzlen/flag-gray-at-dev/MT}{6.4}
\@namedef{res@det/kzlen/fpr-at-0.5}{11.8}
\@namedef{res@det/kzlen/fpr-at-dev}{0.8}
\@namedef{res@det/kzlen/fpr-at-dev-ci-thr/hi}{2.0}
\@namedef{res@det/kzlen/fpr-at-dev-ci-thr/lo}{0.1}
\@namedef{res@det/kzlen/fpr-at-dev-ci/hi}{1.3}
\@namedef{res@det/kzlen/fpr-at-dev-ci/lo}{0.5}
\@namedef{res@det/kzlen/fpr-at-lenaware}{1.3}
\@namedef{res@det/kzlen/fpr-by-domain-at-0.5/encyclopedic}{6.9}
\@namedef{res@det/kzlen/fpr-by-domain-at-0.5/essay}{6.9}
\@namedef{res@det/kzlen/fpr-by-domain-at-0.5/news}{15.3}
\@namedef{res@det/kzlen/fpr-by-domain-at-0.5/web}{14.4}
\@namedef{res@det/kzlen/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/kzlen/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/kzlen/fpr-by-domain-at-dev/news}{0.6}
\@namedef{res@det/kzlen/fpr-by-domain-at-dev/web}{2.2}
\@namedef{res@det/kzlen/fpr-by-len-at-0.5/120-160}{16.6}
\@namedef{res@det/kzlen/fpr-by-len-at-0.5/160-220}{11.0}
\@namedef{res@det/kzlen/fpr-by-len-at-0.5/220-320}{5.6}
\@namedef{res@det/kzlen/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@det/kzlen/fpr-by-len-at-dev/160-220}{0.7}
\@namedef{res@det/kzlen/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/kzlen/fpr-by-len-at-lenaware/120-160}{2.6}
\@namedef{res@det/kzlen/fpr-by-len-at-lenaware/160-220}{0.7}
\@namedef{res@det/kzlen/fpr-by-len-at-lenaware/220-320}{2.8}
\@namedef{res@det/kzlen/script/canon-fpr-at-dev}{1.0}
\@namedef{res@det/kzlen/script/canon-tpr-at-dev}{71.9}
\@namedef{res@det/kzlen/script/hg-tpr-at-dev}{65.0}
\@namedef{res@det/kzlen/script/hg-tpr-orig-at-dev}{62.6}
\@namedef{res@det/kzlen/script/hgfold-tpr-at-dev}{62.3}
\@namedef{res@det/kzlen/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/kzlen/script/hghum-n}{103}
\@namedef{res@det/kzlen/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/kzlen/script/latin-fpr-at-dev}{0.4}
\@namedef{res@det/kzlen/script/latin-tpr-at-dev}{62.3}
\@namedef{res@det/kzlen/script/latin2021}{0.996}
\@namedef{res@det/kzlen/script/latin2021canon}{0.993}
\@namedef{res@det/kzlen/script/trunc100}{0.989}
\@namedef{res@det/kzlen/script/trunc50}{0.977}
\@namedef{res@det/kzlen/seed-range/fpr-at-dev/hi}{1.1}
\@namedef{res@det/kzlen/seed-range/fpr-at-dev/lo}{0.5}
\@namedef{res@det/kzlen/seed-range/fpr50-at-dev/hi}{1.8}
\@namedef{res@det/kzlen/seed-range/fpr50-at-dev/lo}{0.8}
\@namedef{res@det/kzlen/seed-range/gen/g31fl/hi}{79.9}
\@namedef{res@det/kzlen/seed-range/gen/g31fl/lo}{8.3}
\@namedef{res@det/kzlen/seed-range/gen/g35fl/hi}{87.7}
\@namedef{res@det/kzlen/seed-range/gen/g35fl/lo}{18.4}
\@namedef{res@det/kzlen/seed-range/gen/gemma26/hi}{78.9}
\@namedef{res@det/kzlen/seed-range/gen/gemma26/lo}{8.8}
\@namedef{res@det/kzlen/seed-range/gen/gemma31/hi}{70.2}
\@namedef{res@det/kzlen/seed-range/gen/gemma31/lo}{6.5}
\@namedef{res@det/kzlen/seed-range/gen/gptoss/hi}{66.9}
\@namedef{res@det/kzlen/seed-range/gen/gptoss/lo}{7.3}
\@namedef{res@det/kzlen/seed-range/gen/kazllm/hi}{52.9}
\@namedef{res@det/kzlen/seed-range/gen/kazllm/lo}{9.4}
\@namedef{res@det/kzlen/seed-range/gen/qwen/hi}{61.6}
\@namedef{res@det/kzlen/seed-range/gen/qwen/lo}{12.0}
\@namedef{res@det/kzlen/seed-range/gen/sherkala/hi}{58.7}
\@namedef{res@det/kzlen/seed-range/gen/sherkala/lo}{6.7}
\@namedef{res@det/kzlen/seed-range/tpr-at-dev/hi}{80.1}
\@namedef{res@det/kzlen/seed-range/tpr-at-dev/lo}{12.7}
\@namedef{res@det/kzlen/seed-range/tpr-heldout-at-dev/hi}{64.3}
\@namedef{res@det/kzlen/seed-range/tpr-heldout-at-dev/lo}{7.7}
\@namedef{res@det/kzlen/short/100/auroc}{0.989}
\@namedef{res@det/kzlen/short/100/fpr-at-0.5}{15.2}
\@namedef{res@det/kzlen/short/100/fpr-at-dev}{1.3}
\@namedef{res@det/kzlen/short/100/fpr-at-devlen}{1.5}
\@namedef{res@det/kzlen/short/100/fpr-at-devlen-ci-thr/hi}{3.3}
\@namedef{res@det/kzlen/short/100/fpr-at-devlen-ci-thr/lo}{0.5}
\@namedef{res@det/kzlen/short/100/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@det/kzlen/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/kzlen/short/100/thr-devlen}{0.9877}
\@namedef{res@det/kzlen/short/100/tpr-at-0.5}{99.7}
\@namedef{res@det/kzlen/short/100/tpr-at-dev}{76.6}
\@namedef{res@det/kzlen/short/100/tpr-at-devlen}{84.8}
\@namedef{res@det/kzlen/short/50/auroc}{0.977}
\@namedef{res@det/kzlen/short/50/fpr-at-0.5}{22.3}
\@namedef{res@det/kzlen/short/50/fpr-at-dev}{1.5}
\@namedef{res@det/kzlen/short/50/fpr-at-devlen}{1.8}
\@namedef{res@det/kzlen/short/50/fpr-at-devlen-ci-thr/hi}{3.8}
\@namedef{res@det/kzlen/short/50/fpr-at-devlen-ci-thr/lo}{0.0}
\@namedef{res@det/kzlen/short/50/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/kzlen/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/kzlen/short/50/thr-devlen}{0.9886}
\@namedef{res@det/kzlen/short/50/tpr-at-0.5}{99.0}
\@namedef{res@det/kzlen/short/50/tpr-at-dev}{47.7}
\@namedef{res@det/kzlen/short/50/tpr-at-devlen}{54.1}
\@namedef{res@det/kzlen/thr-dev}{0.9890}
\@namedef{res@det/kzlen/thr-lenaware/120-160}{0.9870}
\@namedef{res@det/kzlen/thr-lenaware/160-220}{0.9890}
\@namedef{res@det/kzlen/thr-lenaware/220-320}{0.7602}
\@namedef{res@det/kzlen/tpr-at-0.5}{100.0}
\@namedef{res@det/kzlen/tpr-at-dev}{63.9}
\@namedef{res@det/kzlen/tpr-at-lenaware}{77.4}
\@namedef{res@det/kzlen/tpr-heldout-at-0.5}{96.8}
\@namedef{res@det/kzlen/tpr-heldout-at-dev}{47.7}
\@namedef{res@det/kznoaug/auroc}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/g31fl}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/kznoaug/auroc-by-gen/gemma26}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/gemma31}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/kazllm}{0.977}
\@namedef{res@det/kznoaug/auroc-by-gen/qwen}{0.997}
\@namedef{res@det/kznoaug/auroc-by-gen/sherkala}{0.967}
\@namedef{res@det/kznoaug/auroc-ci/hi}{0.999}
\@namedef{res@det/kznoaug/auroc-ci/lo}{0.995}
\@namedef{res@det/kznoaug/auroc-heldout}{0.988}
\@namedef{res@det/kznoaug/auroc-len120-220}{0.998}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/kazllm}{96.5}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-0.5/sherkala}{92.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/g31fl}{99.8}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/g35fl}{97.7}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/gemma26}{99.1}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/gptoss}{99.2}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/kazllm}{76.5}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/qwen}{98.4}
\@namedef{res@det/kznoaug/flag-by-gen-at-dev/sherkala}{80.0}
\@namedef{res@det/kznoaug/flag-gray-at-0.5/HP}{60.3}
\@namedef{res@det/kznoaug/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/kznoaug/flag-gray-at-0.5/MIX}{97.6}
\@namedef{res@det/kznoaug/flag-gray-at-0.5/MT}{53.5}
\@namedef{res@det/kznoaug/flag-gray-at-dev/HP}{14.1}
\@namedef{res@det/kznoaug/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/kznoaug/flag-gray-at-dev/MIX}{72.6}
\@namedef{res@det/kznoaug/flag-gray-at-dev/MT}{14.3}
\@namedef{res@det/kznoaug/fpr-at-0.5}{12.9}
\@namedef{res@det/kznoaug/fpr-at-dev}{1.0}
\@namedef{res@det/kznoaug/fpr-at-dev-ci-thr/hi}{3.7}
\@namedef{res@det/kznoaug/fpr-at-dev-ci-thr/lo}{0.3}
\@namedef{res@det/kznoaug/fpr-at-dev-ci/hi}{1.5}
\@namedef{res@det/kznoaug/fpr-at-dev-ci/lo}{0.6}
\@namedef{res@det/kznoaug/fpr-at-lenaware}{1.2}
\@namedef{res@det/kznoaug/fpr-by-domain-at-0.5/encyclopedic}{9.2}
\@namedef{res@det/kznoaug/fpr-by-domain-at-0.5/essay}{7.9}
\@namedef{res@det/kznoaug/fpr-by-domain-at-0.5/news}{14.3}
\@namedef{res@det/kznoaug/fpr-by-domain-at-0.5/web}{16.8}
\@namedef{res@det/kznoaug/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/kznoaug/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/kznoaug/fpr-by-domain-at-dev/news}{1.1}
\@namedef{res@det/kznoaug/fpr-by-domain-at-dev/web}{2.2}
\@namedef{res@det/kznoaug/fpr-by-len-at-0.5/120-160}{23.2}
\@namedef{res@det/kznoaug/fpr-by-len-at-0.5/160-220}{11.0}
\@namedef{res@det/kznoaug/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/kznoaug/fpr-by-len-at-dev/120-160}{2.9}
\@namedef{res@det/kznoaug/fpr-by-len-at-dev/160-220}{0.6}
\@namedef{res@det/kznoaug/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/kznoaug/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@det/kznoaug/fpr-by-len-at-lenaware/160-220}{1.0}
\@namedef{res@det/kznoaug/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/kznoaug/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/kznoaug/script/canon-tpr-at-dev}{90.2}
\@namedef{res@det/kznoaug/script/hg-tpr-at-dev}{16.9}
\@namedef{res@det/kznoaug/script/hg-tpr-orig-at-dev}{98.8}
\@namedef{res@det/kznoaug/script/hgfold-tpr-at-dev}{98.8}
\@namedef{res@det/kznoaug/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/kznoaug/script/hghum-n}{103}
\@namedef{res@det/kznoaug/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/kznoaug/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/kznoaug/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/kznoaug/script/latin2021}{0.705}
\@namedef{res@det/kznoaug/script/latin2021canon}{0.996}
\@namedef{res@det/kznoaug/script/trunc100}{0.992}
\@namedef{res@det/kznoaug/script/trunc50}{0.966}
\@namedef{res@det/kznoaug/seed-range/fpr-at-dev/hi}{1.4}
\@namedef{res@det/kznoaug/seed-range/fpr-at-dev/lo}{0.9}
\@namedef{res@det/kznoaug/seed-range/fpr50-at-dev/hi}{15.5}
\@namedef{res@det/kznoaug/seed-range/fpr50-at-dev/lo}{0.3}
\@namedef{res@det/kznoaug/seed-range/gen/g31fl/hi}{99.8}
\@namedef{res@det/kznoaug/seed-range/gen/g31fl/lo}{38.4}
\@namedef{res@det/kznoaug/seed-range/gen/g35fl/hi}{99.4}
\@namedef{res@det/kznoaug/seed-range/gen/g35fl/lo}{55.6}
\@namedef{res@det/kznoaug/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/kznoaug/seed-range/gen/gemma26/lo}{36.8}
\@namedef{res@det/kznoaug/seed-range/gen/gemma31/hi}{100.0}
\@namedef{res@det/kznoaug/seed-range/gen/gemma31/lo}{32.7}
\@namedef{res@det/kznoaug/seed-range/gen/gptoss/hi}{99.2}
\@namedef{res@det/kznoaug/seed-range/gen/gptoss/lo}{45.2}
\@namedef{res@det/kznoaug/seed-range/gen/kazllm/hi}{78.8}
\@namedef{res@det/kznoaug/seed-range/gen/kazllm/lo}{27.1}
\@namedef{res@det/kznoaug/seed-range/gen/qwen/hi}{99.2}
\@namedef{res@det/kznoaug/seed-range/gen/qwen/lo}{29.6}
\@namedef{res@det/kznoaug/seed-range/gen/sherkala/hi}{85.3}
\@namedef{res@det/kznoaug/seed-range/gen/sherkala/lo}{30.7}
\@namedef{res@det/kznoaug/seed-range/tpr-at-dev/hi}{99.5}
\@namedef{res@det/kznoaug/seed-range/tpr-at-dev/lo}{45.2}
\@namedef{res@det/kznoaug/seed-range/tpr-heldout-at-dev/hi}{93.4}
\@namedef{res@det/kznoaug/seed-range/tpr-heldout-at-dev/lo}{32.4}
\@namedef{res@det/kznoaug/short/100/auroc}{0.992}
\@namedef{res@det/kznoaug/short/100/fpr-at-0.5}{43.7}
\@namedef{res@det/kznoaug/short/100/fpr-at-dev}{5.6}
\@namedef{res@det/kznoaug/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/kznoaug/short/100/fpr-at-devlen-ci-thr/hi}{4.1}
\@namedef{res@det/kznoaug/short/100/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/kznoaug/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/kznoaug/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/kznoaug/short/100/thr-devlen}{0.9982}
\@namedef{res@det/kznoaug/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/kznoaug/short/100/tpr-at-dev}{99.2}
\@namedef{res@det/kznoaug/short/100/tpr-at-devlen}{95.9}
\@namedef{res@det/kznoaug/short/50/auroc}{0.966}
\@namedef{res@det/kznoaug/short/50/fpr-at-0.5}{82.2}
\@namedef{res@det/kznoaug/short/50/fpr-at-dev}{6.3}
\@namedef{res@det/kznoaug/short/50/fpr-at-devlen}{2.3}
\@namedef{res@det/kznoaug/short/50/fpr-at-devlen-ci-thr/hi}{5.3}
\@namedef{res@det/kznoaug/short/50/fpr-at-devlen-ci-thr/lo}{1.0}
\@namedef{res@det/kznoaug/short/50/fpr-at-devlen-ci/hi}{3.8}
\@namedef{res@det/kznoaug/short/50/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/kznoaug/short/50/thr-devlen}{0.9978}
\@namedef{res@det/kznoaug/short/50/tpr-at-0.5}{100.0}
\@namedef{res@det/kznoaug/short/50/tpr-at-dev}{84.3}
\@namedef{res@det/kznoaug/short/50/tpr-at-devlen}{63.2}
\@namedef{res@det/kznoaug/thr-dev}{0.9972}
\@namedef{res@det/kznoaug/thr-lenaware/120-160}{0.9980}
\@namedef{res@det/kznoaug/thr-lenaware/160-220}{0.9955}
\@namedef{res@det/kznoaug/thr-lenaware/220-320}{0.5159}
\@namedef{res@det/kznoaug/tpr-at-0.5}{100.0}
\@namedef{res@det/kznoaug/tpr-at-dev}{98.7}
\@namedef{res@det/kznoaug/tpr-at-lenaware}{97.6}
\@namedef{res@det/kznoaug/tpr-heldout-at-0.5}{98.0}
\@namedef{res@det/kznoaug/tpr-heldout-at-dev}{91.9}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc}{0.998}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/g35fl}{0.999}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/gemma26}{0.999}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/gptoss}{0.998}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/kazllm}{0.955}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-by-gen/sherkala}{0.943}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-ci/hi}{1.000}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-ci/lo}{0.997}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-heldout}{0.981}
\@namedef{res@det/logo-gemini-3.1-flash-lite/auroc-len120-220}{0.999}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/g35fl}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/gptoss}{99.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/kazllm}{67.1}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-0.5/sherkala}{76.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/g31fl}{99.8}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/g35fl}{99.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/gemma31}{99.4}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/gptoss}{98.4}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/kazllm}{48.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-by-gen-at-dev/sherkala}{60.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-0.5/HP}{32.1}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-0.5/MIX}{94.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-0.5/MT}{17.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-dev/HP}{10.3}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-dev/MH}{98.4}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-dev/MIX}{89.8}
\@namedef{res@det/logo-gemini-3.1-flash-lite/flag-gray-at-dev/MT}{8.8}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-at-0.5}{3.9}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-at-dev}{1.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-at-dev-ci/hi}{1.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-at-dev-ci/lo}{0.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-at-lenaware}{1.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-0.5/encyclopedic}{1.8}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-0.5/essay}{0.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-0.5/news}{4.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-0.5/web}{6.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-dev/encyclopedic}{0.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-dev/news}{1.3}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-domain-at-dev/web}{2.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-0.5/120-160}{5.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-0.5/160-220}{3.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-0.5/220-320}{0.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-dev/160-220}{1.1}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-lenaware/160-220}{1.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/fpr-by-len-at-lenaware/220-320}{4.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/canon-fpr-at-dev}{1.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/canon-tpr-at-dev}{99.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hg-tpr-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hg-tpr-orig-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hgfold-tpr-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hghum-n}{103}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/latin-fpr-at-dev}{0.8}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/latin-tpr-at-dev}{94.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/latin2021}{0.997}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/latin2021canon}{0.997}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/trunc100}{0.996}
\@namedef{res@det/logo-gemini-3.1-flash-lite/script/trunc50}{0.989}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/auroc}{0.996}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/fpr-at-0.5}{7.4}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/fpr-at-dev}{2.3}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/fpr-at-devlen}{2.3}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/fpr-at-devlen-ci/hi}{4.1}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/thr-devlen}{0.9840}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/tpr-at-0.5}{99.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/tpr-at-dev}{98.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/100/tpr-at-devlen}{98.2}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/auroc}{0.989}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/fpr-at-0.5}{10.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/fpr-at-dev}{4.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/fpr-at-devlen}{3.0}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/fpr-at-devlen-ci/hi}{5.1}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/fpr-at-devlen-ci/lo}{1.5}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/thr-devlen}{0.9879}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/tpr-at-0.5}{97.7}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/tpr-at-dev}{92.4}
\@namedef{res@det/logo-gemini-3.1-flash-lite/short/50/tpr-at-devlen}{90.9}
\@namedef{res@det/logo-gemini-3.1-flash-lite/thr-dev}{0.9833}
\@namedef{res@det/logo-gemini-3.1-flash-lite/thr-lenaware/120-160}{0.9847}
\@namedef{res@det/logo-gemini-3.1-flash-lite/thr-lenaware/160-220}{0.9740}
\@namedef{res@det/logo-gemini-3.1-flash-lite/thr-lenaware/220-320}{0.0533}
\@namedef{res@det/logo-gemini-3.1-flash-lite/tpr-at-0.5}{99.9}
\@namedef{res@det/logo-gemini-3.1-flash-lite/tpr-at-dev}{99.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/tpr-at-lenaware}{99.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/tpr-heldout-at-0.5}{89.6}
\@namedef{res@det/logo-gemini-3.1-flash-lite/tpr-heldout-at-dev}{83.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/g31fl}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/g35fl}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/gemma26}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/gemma31}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/gptoss}{0.999}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/kazllm}{0.953}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/qwen}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-by-gen/sherkala}{0.948}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-ci/hi}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-ci/lo}{0.999}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-heldout}{0.982}
\@namedef{res@det/logo-gemini-3.5-flash-lite/auroc-len120-220}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/g35fl}{99.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/gptoss}{98.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/kazllm}{50.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-0.5/sherkala}{61.3}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/g35fl}{99.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/gptoss}{98.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/kazllm}{51.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-by-gen-at-dev/sherkala}{66.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-0.5/HP}{9.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-0.5/MIX}{85.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-0.5/MT}{9.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-dev/HP}{14.1}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-dev/MH}{100.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-dev/MIX}{88.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/flag-gray-at-dev/MT}{10.2}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-at-0.5}{1.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-at-dev}{1.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-at-dev-ci/hi}{2.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-at-dev-ci/lo}{1.2}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-at-lenaware}{1.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-0.5/encyclopedic}{0.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-0.5/essay}{0.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-0.5/news}{1.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-0.5/web}{1.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-dev/encyclopedic}{1.3}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-dev/news}{1.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-domain-at-dev/web}{2.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-0.5/120-160}{2.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-0.5/160-220}{1.1}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-0.5/220-320}{0.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-dev/120-160}{3.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-dev/160-220}{1.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-lenaware/120-160}{4.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-lenaware/160-220}{0.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/canon-fpr-at-dev}{2.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/canon-tpr-at-dev}{99.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hg-tpr-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hg-tpr-orig-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hgfold-tpr-at-dev}{99.5}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hghum-n}{103}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/latin-fpr-at-dev}{3.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/latin-tpr-at-dev}{99.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/latin2021}{0.998}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/latin2021canon}{1.000}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/trunc100}{0.997}
\@namedef{res@det/logo-gemini-3.5-flash-lite/script/trunc50}{0.988}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/auroc}{0.997}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/fpr-at-0.5}{2.5}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/fpr-at-dev}{3.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/fpr-at-devlen}{2.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/fpr-at-devlen-ci/hi}{3.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/thr-devlen}{0.8206}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/tpr-at-0.5}{98.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/tpr-at-dev}{99.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/100/tpr-at-devlen}{98.2}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/auroc}{0.988}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/fpr-at-0.5}{6.1}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/fpr-at-dev}{6.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/fpr-at-devlen}{2.0}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/fpr-at-devlen-ci/hi}{3.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/thr-devlen}{0.9813}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/tpr-at-0.5}{94.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/tpr-at-dev}{95.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/short/50/tpr-at-devlen}{86.5}
\@namedef{res@det/logo-gemini-3.5-flash-lite/thr-dev}{0.2637}
\@namedef{res@det/logo-gemini-3.5-flash-lite/thr-lenaware/120-160}{0.2337}
\@namedef{res@det/logo-gemini-3.5-flash-lite/thr-lenaware/160-220}{0.6210}
\@namedef{res@det/logo-gemini-3.5-flash-lite/thr-lenaware/220-320}{0.0148}
\@namedef{res@det/logo-gemini-3.5-flash-lite/tpr-at-0.5}{99.6}
\@namedef{res@det/logo-gemini-3.5-flash-lite/tpr-at-dev}{99.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/tpr-at-lenaware}{99.7}
\@namedef{res@det/logo-gemini-3.5-flash-lite/tpr-heldout-at-0.5}{83.9}
\@namedef{res@det/logo-gemini-3.5-flash-lite/tpr-heldout-at-dev}{85.1}
\@namedef{res@det/logo-gpt-oss-120b/auroc}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/g35fl}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/kazllm}{0.965}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/auroc-by-gen/sherkala}{0.953}
\@namedef{res@det/logo-gpt-oss-120b/auroc-ci/hi}{0.999}
\@namedef{res@det/logo-gpt-oss-120b/auroc-ci/lo}{0.996}
\@namedef{res@det/logo-gpt-oss-120b/auroc-heldout}{0.984}
\@namedef{res@det/logo-gpt-oss-120b/auroc-len120-220}{0.998}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/g35fl}{99.8}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/gptoss}{99.2}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/kazllm}{61.2}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-0.5/sherkala}{73.3}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/g35fl}{99.6}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/gptoss}{94.4}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/kazllm}{49.4}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-by-gen-at-dev/sherkala}{62.7}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-0.5/HP}{16.7}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-0.5/MIX}{88.1}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-0.5/MT}{10.5}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-dev/HP}{7.7}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-dev/MH}{93.8}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-dev/MIX}{82.1}
\@namedef{res@det/logo-gpt-oss-120b/flag-gray-at-dev/MT}{7.0}
\@namedef{res@det/logo-gpt-oss-120b/fpr-at-0.5}{1.5}
\@namedef{res@det/logo-gpt-oss-120b/fpr-at-dev}{0.6}
\@namedef{res@det/logo-gpt-oss-120b/fpr-at-dev-ci/hi}{1.0}
\@namedef{res@det/logo-gpt-oss-120b/fpr-at-dev-ci/lo}{0.3}
\@namedef{res@det/logo-gpt-oss-120b/fpr-at-lenaware}{0.9}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-0.5/encyclopedic}{0.8}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-0.5/essay}{0.5}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-0.5/news}{1.3}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-0.5/web}{2.8}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-dev/news}{0.9}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-domain-at-dev/web}{1.1}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-0.5/120-160}{2.6}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-0.5/160-220}{1.2}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-0.5/220-320}{1.4}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-dev/160-220}{0.3}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-lenaware/120-160}{2.3}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-lenaware/160-220}{0.3}
\@namedef{res@det/logo-gpt-oss-120b/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/logo-gpt-oss-120b/script/canon-fpr-at-dev}{1.2}
\@namedef{res@det/logo-gpt-oss-120b/script/canon-tpr-at-dev}{99.0}
\@namedef{res@det/logo-gpt-oss-120b/script/hg-tpr-at-dev}{99.0}
\@namedef{res@det/logo-gpt-oss-120b/script/hg-tpr-orig-at-dev}{99.3}
\@namedef{res@det/logo-gpt-oss-120b/script/hgfold-tpr-at-dev}{99.3}
\@namedef{res@det/logo-gpt-oss-120b/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/logo-gpt-oss-120b/script/hghum-n}{103}
\@namedef{res@det/logo-gpt-oss-120b/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/logo-gpt-oss-120b/script/latin-fpr-at-dev}{0.6}
\@namedef{res@det/logo-gpt-oss-120b/script/latin-tpr-at-dev}{91.7}
\@namedef{res@det/logo-gpt-oss-120b/script/latin2021}{0.997}
\@namedef{res@det/logo-gpt-oss-120b/script/latin2021canon}{0.997}
\@namedef{res@det/logo-gpt-oss-120b/script/trunc100}{0.993}
\@namedef{res@det/logo-gpt-oss-120b/script/trunc50}{0.977}
\@namedef{res@det/logo-gpt-oss-120b/short/100/auroc}{0.993}
\@namedef{res@det/logo-gpt-oss-120b/short/100/fpr-at-0.5}{4.1}
\@namedef{res@det/logo-gpt-oss-120b/short/100/fpr-at-dev}{3.0}
\@namedef{res@det/logo-gpt-oss-120b/short/100/fpr-at-devlen}{2.0}
\@namedef{res@det/logo-gpt-oss-120b/short/100/fpr-at-devlen-ci/hi}{3.6}
\@namedef{res@det/logo-gpt-oss-120b/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/logo-gpt-oss-120b/short/100/thr-devlen}{0.9866}
\@namedef{res@det/logo-gpt-oss-120b/short/100/tpr-at-0.5}{99.2}
\@namedef{res@det/logo-gpt-oss-120b/short/100/tpr-at-dev}{98.2}
\@namedef{res@det/logo-gpt-oss-120b/short/100/tpr-at-devlen}{96.2}
\@namedef{res@det/logo-gpt-oss-120b/short/50/auroc}{0.977}
\@namedef{res@det/logo-gpt-oss-120b/short/50/fpr-at-0.5}{12.7}
\@namedef{res@det/logo-gpt-oss-120b/short/50/fpr-at-dev}{6.6}
\@namedef{res@det/logo-gpt-oss-120b/short/50/fpr-at-devlen}{1.3}
\@namedef{res@det/logo-gpt-oss-120b/short/50/fpr-at-devlen-ci/hi}{2.3}
\@namedef{res@det/logo-gpt-oss-120b/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/logo-gpt-oss-120b/short/50/thr-devlen}{0.9907}
\@namedef{res@det/logo-gpt-oss-120b/short/50/tpr-at-0.5}{97.5}
\@namedef{res@det/logo-gpt-oss-120b/short/50/tpr-at-dev}{94.2}
\@namedef{res@det/logo-gpt-oss-120b/short/50/tpr-at-devlen}{58.6}
\@namedef{res@det/logo-gpt-oss-120b/thr-dev}{0.9715}
\@namedef{res@det/logo-gpt-oss-120b/thr-lenaware/120-160}{0.8683}
\@namedef{res@det/logo-gpt-oss-120b/thr-lenaware/160-220}{0.9754}
\@namedef{res@det/logo-gpt-oss-120b/thr-lenaware/220-320}{0.0164}
\@namedef{res@det/logo-gpt-oss-120b/tpr-at-0.5}{99.8}
\@namedef{res@det/logo-gpt-oss-120b/tpr-at-dev}{99.3}
\@namedef{res@det/logo-gpt-oss-120b/tpr-at-lenaware}{99.7}
\@namedef{res@det/logo-gpt-oss-120b/tpr-heldout-at-0.5}{88.0}
\@namedef{res@det/logo-gpt-oss-120b/tpr-heldout-at-dev}{83.9}
\@namedef{res@det/logo-qwen3.8-27b/auroc}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/g31fl}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/g35fl}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/gemma26}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/gemma31}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/kazllm}{0.944}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/qwen}{0.998}
\@namedef{res@det/logo-qwen3.8-27b/auroc-by-gen/sherkala}{0.943}
\@namedef{res@det/logo-qwen3.8-27b/auroc-ci/hi}{0.999}
\@namedef{res@det/logo-qwen3.8-27b/auroc-ci/lo}{0.995}
\@namedef{res@det/logo-qwen3.8-27b/auroc-heldout}{0.978}
\@namedef{res@det/logo-qwen3.8-27b/auroc-len120-220}{0.997}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/g35fl}{99.8}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/gptoss}{99.2}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/kazllm}{51.8}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-0.5/sherkala}{72.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/g35fl}{99.8}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/gemma26}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/gemma31}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/gptoss}{98.4}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/kazllm}{36.5}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-by-gen-at-dev/sherkala}{62.7}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-0.5/HP}{29.5}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-0.5/MH}{98.4}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-0.5/MIX}{94.4}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-0.5/MT}{14.0}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-dev/HP}{14.1}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-dev/MH}{98.4}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-dev/MIX}{90.3}
\@namedef{res@det/logo-qwen3.8-27b/flag-gray-at-dev/MT}{7.3}
\@namedef{res@det/logo-qwen3.8-27b/fpr-at-0.5}{2.7}
\@namedef{res@det/logo-qwen3.8-27b/fpr-at-dev}{1.1}
\@namedef{res@det/logo-qwen3.8-27b/fpr-at-dev-ci/hi}{1.6}
\@namedef{res@det/logo-qwen3.8-27b/fpr-at-dev-ci/lo}{0.6}
\@namedef{res@det/logo-qwen3.8-27b/fpr-at-lenaware}{1.2}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-0.5/encyclopedic}{1.1}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-0.5/essay}{0.0}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-0.5/news}{3.0}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-0.5/web}{5.2}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-dev/news}{1.7}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-domain-at-dev/web}{1.9}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-0.5/120-160}{4.3}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-0.5/160-220}{2.5}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-0.5/220-320}{0.7}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-dev/120-160}{2.3}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-dev/160-220}{0.9}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-lenaware/120-160}{2.3}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-lenaware/160-220}{0.9}
\@namedef{res@det/logo-qwen3.8-27b/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/logo-qwen3.8-27b/script/canon-fpr-at-dev}{1.2}
\@namedef{res@det/logo-qwen3.8-27b/script/canon-tpr-at-dev}{99.7}
\@namedef{res@det/logo-qwen3.8-27b/script/hg-tpr-at-dev}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/script/hg-tpr-orig-at-dev}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/script/hgfold-tpr-at-dev}{100.0}
\@namedef{res@det/logo-qwen3.8-27b/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/logo-qwen3.8-27b/script/hghum-n}{103}
\@namedef{res@det/logo-qwen3.8-27b/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/logo-qwen3.8-27b/script/latin-fpr-at-dev}{0.8}
\@namedef{res@det/logo-qwen3.8-27b/script/latin-tpr-at-dev}{98.0}
\@namedef{res@det/logo-qwen3.8-27b/script/latin2021}{0.998}
\@namedef{res@det/logo-qwen3.8-27b/script/latin2021canon}{0.996}
\@namedef{res@det/logo-qwen3.8-27b/script/trunc100}{0.995}
\@namedef{res@det/logo-qwen3.8-27b/script/trunc50}{0.983}
\@namedef{res@det/logo-qwen3.8-27b/short/100/auroc}{0.995}
\@namedef{res@det/logo-qwen3.8-27b/short/100/fpr-at-0.5}{3.6}
\@namedef{res@det/logo-qwen3.8-27b/short/100/fpr-at-dev}{1.8}
\@namedef{res@det/logo-qwen3.8-27b/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/logo-qwen3.8-27b/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/logo-qwen3.8-27b/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/logo-qwen3.8-27b/short/100/thr-devlen}{0.9781}
\@namedef{res@det/logo-qwen3.8-27b/short/100/tpr-at-0.5}{99.5}
\@namedef{res@det/logo-qwen3.8-27b/short/100/tpr-at-dev}{98.5}
\@namedef{res@det/logo-qwen3.8-27b/short/100/tpr-at-devlen}{98.5}
\@namedef{res@det/logo-qwen3.8-27b/short/50/auroc}{0.983}
\@namedef{res@det/logo-qwen3.8-27b/short/50/fpr-at-0.5}{7.4}
\@namedef{res@det/logo-qwen3.8-27b/short/50/fpr-at-dev}{3.8}
\@namedef{res@det/logo-qwen3.8-27b/short/50/fpr-at-devlen}{1.8}
\@namedef{res@det/logo-qwen3.8-27b/short/50/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@det/logo-qwen3.8-27b/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/logo-qwen3.8-27b/short/50/thr-devlen}{0.9871}
\@namedef{res@det/logo-qwen3.8-27b/short/50/tpr-at-0.5}{98.0}
\@namedef{res@det/logo-qwen3.8-27b/short/50/tpr-at-dev}{93.7}
\@namedef{res@det/logo-qwen3.8-27b/short/50/tpr-at-devlen}{89.1}
\@namedef{res@det/logo-qwen3.8-27b/thr-dev}{0.9668}
\@namedef{res@det/logo-qwen3.8-27b/thr-lenaware/120-160}{0.9719}
\@namedef{res@det/logo-qwen3.8-27b/thr-lenaware/160-220}{0.9727}
\@namedef{res@det/logo-qwen3.8-27b/thr-lenaware/220-320}{0.3689}
\@namedef{res@det/logo-qwen3.8-27b/tpr-at-0.5}{99.8}
\@namedef{res@det/logo-qwen3.8-27b/tpr-at-dev}{99.8}
\@namedef{res@det/logo-qwen3.8-27b/tpr-at-lenaware}{99.8}
\@namedef{res@det/logo-qwen3.8-27b/tpr-heldout-at-0.5}{86.0}
\@namedef{res@det/logo-qwen3.8-27b/tpr-heldout-at-dev}{81.4}
\@namedef{res@det/logo/g31fl/auroc}{0.998}
\@namedef{res@det/logo/g31fl/auroc-when-trained}{0.996}
\@namedef{res@det/logo/g31fl/fpr-at-dev}{1.2}
\@namedef{res@det/logo/g31fl/tpr-at-dev}{99.8}
\@namedef{res@det/logo/g31fl/tpr-at-dev-when-trained}{100.0}
\@namedef{res@det/logo/g35fl/auroc}{1.000}
\@namedef{res@det/logo/g35fl/auroc-when-trained}{0.997}
\@namedef{res@det/logo/g35fl/fpr-at-dev}{1.9}
\@namedef{res@det/logo/g35fl/tpr-at-dev}{99.6}
\@namedef{res@det/logo/g35fl/tpr-at-dev-when-trained}{99.8}
\@namedef{res@det/logo/gptoss/auroc}{0.997}
\@namedef{res@det/logo/gptoss/auroc-when-trained}{0.996}
\@namedef{res@det/logo/gptoss/fpr-at-dev}{0.6}
\@namedef{res@det/logo/gptoss/tpr-at-dev}{94.4}
\@namedef{res@det/logo/gptoss/tpr-at-dev-when-trained}{99.2}
\@namedef{res@det/logo/qwen/auroc}{0.998}
\@namedef{res@det/logo/qwen/auroc-when-trained}{0.997}
\@namedef{res@det/logo/qwen/fpr-at-dev}{1.1}
\@namedef{res@det/logo/qwen/tpr-at-dev}{100.0}
\@namedef{res@det/logo/qwen/tpr-at-dev-when-trained}{100.0}
\@namedef{res@det/n-combos}{five}
\@namedef{res@det/n/H-dev}{391}
\@namedef{res@det/n/H-test}{1,530}
\@namedef{res@det/n/H-train-zs}{2,281}
\@namedef{res@det/n/M-heldout-topicdisjoint}{442}
\@namedef{res@det/n/M-indist}{1,274}
\@namedef{res@det/n/dev-cluster-share}{a fifth}
\@namedef{res@det/n/dev-clusters}{7}
\@namedef{res@det/xlmr/auroc}{0.998}
\@namedef{res@det/xlmr/auroc-by-gen/g31fl}{0.998}
\@namedef{res@det/xlmr/auroc-by-gen/g35fl}{0.997}
\@namedef{res@det/xlmr/auroc-by-gen/gemma26}{0.998}
\@namedef{res@det/xlmr/auroc-by-gen/gemma31}{0.998}
\@namedef{res@det/xlmr/auroc-by-gen/gptoss}{0.997}
\@namedef{res@det/xlmr/auroc-by-gen/kazllm}{0.972}
\@namedef{res@det/xlmr/auroc-by-gen/qwen}{0.999}
\@namedef{res@det/xlmr/auroc-by-gen/sherkala}{0.933}
\@namedef{res@det/xlmr/auroc-ci/hi}{0.999}
\@namedef{res@det/xlmr/auroc-ci/lo}{0.996}
\@namedef{res@det/xlmr/auroc-heldout}{0.982}
\@namedef{res@det/xlmr/auroc-len120-220}{0.998}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/g31fl}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/g35fl}{99.8}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/gemma26}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/gemma31}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/gptoss}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/kazllm}{94.1}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/qwen}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-0.5/sherkala}{90.7}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/g31fl}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/g35fl}{98.7}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/gemma26}{99.1}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/gemma31}{99.4}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/gptoss}{97.6}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/kazllm}{69.4}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/qwen}{100.0}
\@namedef{res@det/xlmr/flag-by-gen-at-dev/sherkala}{64.0}
\@namedef{res@det/xlmr/flag-gray-at-0.5/HP}{37.2}
\@namedef{res@det/xlmr/flag-gray-at-0.5/MH}{100.0}
\@namedef{res@det/xlmr/flag-gray-at-0.5/MIX}{96.3}
\@namedef{res@det/xlmr/flag-gray-at-0.5/MT}{45.0}
\@namedef{res@det/xlmr/flag-gray-at-dev/HP}{6.4}
\@namedef{res@det/xlmr/flag-gray-at-dev/MH}{98.4}
\@namedef{res@det/xlmr/flag-gray-at-dev/MIX}{68.8}
\@namedef{res@det/xlmr/flag-gray-at-dev/MT}{17.0}
\@namedef{res@det/xlmr/fpr-at-0.5}{9.9}
\@namedef{res@det/xlmr/fpr-at-dev}{1.6}
\@namedef{res@det/xlmr/fpr-at-dev-ci-thr/hi}{2.7}
\@namedef{res@det/xlmr/fpr-at-dev-ci-thr/lo}{0.7}
\@namedef{res@det/xlmr/fpr-at-dev-ci/hi}{2.1}
\@namedef{res@det/xlmr/fpr-at-dev-ci/lo}{1.0}
\@namedef{res@det/xlmr/fpr-at-lenaware}{2.2}
\@namedef{res@det/xlmr/fpr-by-domain-at-0.5/encyclopedic}{5.0}
\@namedef{res@det/xlmr/fpr-by-domain-at-0.5/essay}{6.9}
\@namedef{res@det/xlmr/fpr-by-domain-at-0.5/news}{11.1}
\@namedef{res@det/xlmr/fpr-by-domain-at-0.5/web}{14.2}
\@namedef{res@det/xlmr/fpr-by-domain-at-dev/encyclopedic}{0.0}
\@namedef{res@det/xlmr/fpr-by-domain-at-dev/essay}{1.4}
\@namedef{res@det/xlmr/fpr-by-domain-at-dev/news}{1.9}
\@namedef{res@det/xlmr/fpr-by-domain-at-dev/web}{2.6}
\@namedef{res@det/xlmr/fpr-by-len-at-0.5/120-160}{16.9}
\@namedef{res@det/xlmr/fpr-by-len-at-0.5/160-220}{8.5}
\@namedef{res@det/xlmr/fpr-by-len-at-0.5/220-320}{3.5}
\@namedef{res@det/xlmr/fpr-by-len-at-dev/120-160}{2.6}
\@namedef{res@det/xlmr/fpr-by-len-at-dev/160-220}{1.4}
\@namedef{res@det/xlmr/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/xlmr/fpr-by-len-at-lenaware/120-160}{2.6}
\@namedef{res@det/xlmr/fpr-by-len-at-lenaware/160-220}{1.6}
\@namedef{res@det/xlmr/fpr-by-len-at-lenaware/220-320}{5.6}
\@namedef{res@det/xlmr/script/canon-fpr-at-dev}{1.8}
\@namedef{res@det/xlmr/script/canon-tpr-at-dev}{98.5}
\@namedef{res@det/xlmr/script/hg-tpr-at-dev}{27.1}
\@namedef{res@det/xlmr/script/hg-tpr-orig-at-dev}{99.3}
\@namedef{res@det/xlmr/script/hgfold-tpr-at-dev}{99.3}
\@namedef{res@det/xlmr/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/xlmr/script/hghum-n}{103}
\@namedef{res@det/xlmr/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/xlmr/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/xlmr/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/xlmr/script/latin2021}{0.875}
\@namedef{res@det/xlmr/script/latin2021canon}{0.994}
\@namedef{res@det/xlmr/script/trunc100}{0.990}
\@namedef{res@det/xlmr/script/trunc50}{0.972}
\@namedef{res@det/xlmr/seed-range/fpr-at-dev/hi}{1.3}
\@namedef{res@det/xlmr/seed-range/fpr-at-dev/lo}{1.0}
\@namedef{res@det/xlmr/seed-range/fpr50-at-dev/hi}{2.0}
\@namedef{res@det/xlmr/seed-range/fpr50-at-dev/lo}{0.0}
\@namedef{res@det/xlmr/seed-range/gen/g31fl/hi}{100.0}
\@namedef{res@det/xlmr/seed-range/gen/g31fl/lo}{75.3}
\@namedef{res@det/xlmr/seed-range/gen/g35fl/hi}{99.8}
\@namedef{res@det/xlmr/seed-range/gen/g35fl/lo}{66.1}
\@namedef{res@det/xlmr/seed-range/gen/gemma26/hi}{100.0}
\@namedef{res@det/xlmr/seed-range/gen/gemma26/lo}{82.5}
\@namedef{res@det/xlmr/seed-range/gen/gemma31/hi}{99.4}
\@namedef{res@det/xlmr/seed-range/gen/gemma31/lo}{74.4}
\@namedef{res@det/xlmr/seed-range/gen/gptoss/hi}{97.6}
\@namedef{res@det/xlmr/seed-range/gen/gptoss/lo}{79.8}
\@namedef{res@det/xlmr/seed-range/gen/kazllm/hi}{68.2}
\@namedef{res@det/xlmr/seed-range/gen/kazllm/lo}{32.9}
\@namedef{res@det/xlmr/seed-range/gen/qwen/hi}{100.0}
\@namedef{res@det/xlmr/seed-range/gen/qwen/lo}{78.4}
\@namedef{res@det/xlmr/seed-range/gen/sherkala/hi}{68.0}
\@namedef{res@det/xlmr/seed-range/gen/sherkala/lo}{28.0}
\@namedef{res@det/xlmr/seed-range/tpr-at-dev/hi}{99.7}
\@namedef{res@det/xlmr/seed-range/tpr-at-dev/lo}{72.3}
\@namedef{res@det/xlmr/seed-range/tpr-heldout-at-dev/hi}{88.2}
\@namedef{res@det/xlmr/seed-range/tpr-heldout-at-dev/lo}{62.4}
\@namedef{res@det/xlmr/short/100/auroc}{0.990}
\@namedef{res@det/xlmr/short/100/fpr-at-0.5}{18.8}
\@namedef{res@det/xlmr/short/100/fpr-at-dev}{2.8}
\@namedef{res@det/xlmr/short/100/fpr-at-devlen}{2.8}
\@namedef{res@det/xlmr/short/100/fpr-at-devlen-ci-thr/hi}{4.6}
\@namedef{res@det/xlmr/short/100/fpr-at-devlen-ci-thr/lo}{0.8}
\@namedef{res@det/xlmr/short/100/fpr-at-devlen-ci/hi}{4.6}
\@namedef{res@det/xlmr/short/100/fpr-at-devlen-ci/lo}{1.5}
\@namedef{res@det/xlmr/short/100/thr-devlen}{0.9987}
\@namedef{res@det/xlmr/short/100/tpr-at-0.5}{100.0}
\@namedef{res@det/xlmr/short/100/tpr-at-dev}{95.7}
\@namedef{res@det/xlmr/short/100/tpr-at-devlen}{96.4}
\@namedef{res@det/xlmr/short/50/auroc}{0.972}
\@namedef{res@det/xlmr/short/50/fpr-at-0.5}{21.1}
\@namedef{res@det/xlmr/short/50/fpr-at-dev}{0.3}
\@namedef{res@det/xlmr/short/50/fpr-at-devlen}{3.0}
\@namedef{res@det/xlmr/short/50/fpr-at-devlen-ci-thr/hi}{5.3}
\@namedef{res@det/xlmr/short/50/fpr-at-devlen-ci-thr/lo}{0.3}
\@namedef{res@det/xlmr/short/50/fpr-at-devlen-ci/hi}{4.6}
\@namedef{res@det/xlmr/short/50/fpr-at-devlen-ci/lo}{1.5}
\@namedef{res@det/xlmr/short/50/thr-devlen}{0.9984}
\@namedef{res@det/xlmr/short/50/tpr-at-0.5}{100.0}
\@namedef{res@det/xlmr/short/50/tpr-at-dev}{14.7}
\@namedef{res@det/xlmr/short/50/tpr-at-devlen}{66.0}
\@namedef{res@det/xlmr/thr-dev}{0.9988}
\@namedef{res@det/xlmr/thr-lenaware/120-160}{0.9988}
\@namedef{res@det/xlmr/thr-lenaware/160-220}{0.9987}
\@namedef{res@det/xlmr/thr-lenaware/220-320}{0.3539}
\@namedef{res@det/xlmr/tpr-at-0.5}{99.9}
\@namedef{res@det/xlmr/tpr-at-dev}{99.2}
\@namedef{res@det/xlmr/tpr-at-lenaware}{99.2}
\@namedef{res@det/xlmr/tpr-heldout-at-0.5}{97.3}
\@namedef{res@det/xlmr/tpr-heldout-at-dev}{87.6}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc}{0.931}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/g31fl}{0.958}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/g35fl}{0.874}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/gemma26}{0.999}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/gemma31}{0.991}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/gptoss}{0.999}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/kazllm}{0.955}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/qwen}{0.988}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-by-gen/sherkala}{0.960}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-ci/hi}{0.940}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-ci/lo}{0.921}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-heldout}{0.981}
\@namedef{res@det/zs:gemma4-e2b:binoculars/auroc-len120-220}{0.936}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/g31fl}{55.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/g35fl}{27.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/gemma26}{95.6}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/gemma31}{86.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/gptoss}{96.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/kazllm}{50.6}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/qwen}{78.4}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-by-gen-at-dev/sherkala}{74.7}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-gray-at-dev/HP}{7.7}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-gray-at-dev/MH}{20.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-gray-at-dev/MIX}{35.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/flag-gray-at-dev/MT}{8.2}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-at-dev}{0.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-at-dev-ci/hi}{1.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-at-dev-ci/lo}{0.5}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-at-lenaware}{0.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-domain-at-dev/encyclopedic}{1.1}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-domain-at-dev/essay}{1.9}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-domain-at-dev/web}{0.9}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-dev/120-160}{1.1}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-dev/160-220}{0.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-lenaware/120-160}{1.1}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-lenaware/160-220}{0.9}
\@namedef{res@det/zs:gemma4-e2b:binoculars/fpr-by-len-at-lenaware/220-320}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/canon-fpr-at-dev}{0.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/canon-tpr-at-dev}{37.2}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hg-tpr-at-dev}{12.5}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hg-tpr-orig-at-dev}{49.1}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hgfold-tpr-at-dev}{48.4}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hghum-n}{103}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/latin2021}{0.346}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/latin2021canon}{0.917}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/trunc100}{0.942}
\@namedef{res@det/zs:gemma4-e2b:binoculars/script/trunc50}{0.895}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/auroc}{0.942}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/fpr-at-dev}{0.5}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/fpr-at-devlen}{0.5}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/fpr-at-devlen-ci/hi}{1.5}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/thr-devlen}{-0.8724}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/tpr-at-dev}{49.7}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/100/tpr-at-devlen}{48.7}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/auroc}{0.895}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/fpr-at-dev}{3.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/thr-devlen}{-0.8486}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/tpr-at-dev}{50.0}
\@namedef{res@det/zs:gemma4-e2b:binoculars/short/50/tpr-at-devlen}{40.1}
\@namedef{res@det/zs:gemma4-e2b:binoculars/thr-dev}{-0.8750}
\@namedef{res@det/zs:gemma4-e2b:binoculars/thr-lenaware/120-160}{-0.8779}
\@namedef{res@det/zs:gemma4-e2b:binoculars/thr-lenaware/160-220}{-0.8778}
\@namedef{res@det/zs:gemma4-e2b:binoculars/thr-lenaware/220-320}{-0.8579}
\@namedef{res@det/zs:gemma4-e2b:binoculars/tpr-at-dev}{50.3}
\@namedef{res@det/zs:gemma4-e2b:binoculars/tpr-at-lenaware}{51.6}
\@namedef{res@det/zs:gemma4-e2b:binoculars/tpr-heldout-at-dev}{79.9}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc}{0.761}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/g31fl}{0.819}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/g35fl}{0.672}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/gemma26}{0.809}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/gemma31}{0.810}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/gptoss}{0.933}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/kazllm}{0.737}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/qwen}{0.729}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-by-gen/sherkala}{0.933}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-ci/hi}{0.777}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-ci/lo}{0.743}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-heldout}{0.817}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/auroc-len120-220}{0.767}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/g31fl}{11.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/g35fl}{2.7}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/gemma26}{11.4}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/gemma31}{8.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/gptoss}{42.7}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/kazllm}{27.1}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/qwen}{11.2}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-by-gen-at-dev/sherkala}{48.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-gray-at-dev/HP}{11.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-gray-at-dev/MH}{3.1}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-gray-at-dev/MIX}{7.8}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/flag-gray-at-dev/MT}{1.2}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-at-dev}{0.7}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-at-dev-ci/hi}{1.1}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-at-dev-ci/lo}{0.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-at-lenaware}{0.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-domain-at-dev/news}{0.6}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-domain-at-dev/web}{1.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-dev/120-160}{1.4}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-dev/160-220}{0.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-lenaware/120-160}{0.9}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-lenaware/160-220}{0.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/fpr-by-len-at-lenaware/220-320}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/canon-fpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/canon-tpr-at-dev}{4.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hg-tpr-orig-at-dev}{11.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hgfold-tpr-at-dev}{10.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/latin-tpr-at-dev}{0.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/latin2021}{0.452}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/latin2021canon}{0.725}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/trunc100}{0.795}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/script/trunc50}{0.763}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/auroc}{0.795}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/fpr-at-dev}{0.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/thr-devlen}{1.5662}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/tpr-at-dev}{8.6}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/100/tpr-at-devlen}{13.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/auroc}{0.763}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/fpr-at-dev}{0.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/fpr-at-devlen}{1.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/fpr-at-devlen-ci/hi}{2.5}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/thr-devlen}{1.5499}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/tpr-at-dev}{3.3}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/short/50/tpr-at-devlen}{7.9}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/thr-dev}{1.8371}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/thr-lenaware/120-160}{1.8660}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/thr-lenaware/160-220}{1.8282}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/thr-lenaware/220-320}{1.6988}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/tpr-at-dev}{10.8}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/tpr-at-lenaware}{10.6}
\@namedef{res@det/zs:gemma4-e2b:obs-fdg/tpr-heldout-at-dev}{19.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc}{0.579}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/g31fl}{0.592}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/g35fl}{0.497}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/gemma26}{0.773}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/gemma31}{0.735}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/gptoss}{0.765}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/kazllm}{0.704}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/qwen}{0.684}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-by-gen/sherkala}{0.917}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-ci/hi}{0.598}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-ci/lo}{0.557}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-heldout}{0.770}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/auroc-len120-220}{0.553}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/g31fl}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/g35fl}{0.6}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/gemma26}{7.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/gemma31}{6.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/gptoss}{5.6}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/kazllm}{24.7}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/qwen}{4.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-by-gen-at-dev/sherkala}{38.7}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-gray-at-dev/HP}{1.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-gray-at-dev/MH}{0.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-gray-at-dev/MIX}{0.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/flag-gray-at-dev/MT}{10.2}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-at-dev}{0.7}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-at-dev-ci/hi}{1.1}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-at-dev-ci/lo}{0.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-at-lenaware}{0.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-domain-at-dev/encyclopedic}{0.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-domain-at-dev/essay}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-domain-at-dev/web}{0.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-dev/120-160}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-dev/160-220}{0.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-lenaware/120-160}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-lenaware/160-220}{0.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/canon-tpr-at-dev}{1.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hg-tpr-orig-at-dev}{2.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hgfold-tpr-at-dev}{2.2}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/latin-fpr-at-dev}{85.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/latin-tpr-at-dev}{89.7}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/latin2021}{0.605}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/latin2021canon}{0.507}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/trunc100}{0.543}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/script/trunc50}{0.557}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/auroc}{0.543}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/fpr-at-dev}{14.2}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/fpr-at-devlen}{0.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/fpr-at-devlen-ci/hi}{1.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/thr-devlen}{-36.5874}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/tpr-at-dev}{17.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/100/tpr-at-devlen}{0.5}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/auroc}{0.557}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/fpr-at-dev}{91.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/thr-devlen}{-23.3082}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/tpr-at-dev}{93.9}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/short/50/tpr-at-devlen}{1.3}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/thr-dev}{-45.5503}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/thr-lenaware/120-160}{-44.5481}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/thr-lenaware/160-220}{-46.6662}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/thr-lenaware/220-320}{-46.1211}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/tpr-at-dev}{1.8}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/tpr-at-lenaware}{1.4}
\@namedef{res@det/zs:gemma4-e2b:perf-fdg/tpr-heldout-at-dev}{15.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc}{0.664}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/g31fl}{0.643}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/g35fl}{0.617}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/gemma26}{0.718}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/gemma31}{0.707}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/gptoss}{0.872}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/kazllm}{0.783}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/qwen}{0.731}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-by-gen/sherkala}{0.831}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-ci/hi}{0.681}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-ci/lo}{0.646}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-heldout}{0.745}
\@namedef{res@det/zs:llama3.2-3b:binoculars/auroc-len120-220}{0.662}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/g31fl}{1.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/g35fl}{1.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/gemma26}{3.5}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/gemma31}{3.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/gptoss}{17.7}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/kazllm}{17.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/qwen}{8.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-by-gen-at-dev/sherkala}{21.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-gray-at-dev/HP}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-gray-at-dev/MH}{1.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-gray-at-dev/MIX}{2.9}
\@namedef{res@det/zs:llama3.2-3b:binoculars/flag-gray-at-dev/MT}{2.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-at-dev}{1.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-at-dev-ci/hi}{2.1}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-at-dev-ci/lo}{0.9}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-at-lenaware}{1.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-domain-at-dev/encyclopedic}{2.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-domain-at-dev/essay}{3.2}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-domain-at-dev/news}{0.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-domain-at-dev/web}{0.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-dev/120-160}{0.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-dev/160-220}{1.7}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-lenaware/120-160}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-lenaware/160-220}{1.8}
\@namedef{res@det/zs:llama3.2-3b:binoculars/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/canon-fpr-at-dev}{0.2}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/canon-tpr-at-dev}{2.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hg-tpr-orig-at-dev}{2.2}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hgfold-tpr-at-dev}{2.2}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hghum-n}{103}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/latin2021}{0.440}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/latin2021canon}{0.625}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/trunc100}{0.630}
\@namedef{res@det/zs:llama3.2-3b:binoculars/script/trunc50}{0.588}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/auroc}{0.630}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/fpr-at-dev}{1.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/fpr-at-devlen}{1.5}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/fpr-at-devlen-ci/hi}{2.8}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/thr-devlen}{-0.9135}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/tpr-at-dev}{3.8}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/100/tpr-at-devlen}{3.8}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/auroc}{0.588}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/fpr-at-dev}{4.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/fpr-at-devlen}{0.5}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/fpr-at-devlen-ci/hi}{1.3}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/thr-devlen}{-0.8670}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/tpr-at-dev}{6.1}
\@namedef{res@det/zs:llama3.2-3b:binoculars/short/50/tpr-at-devlen}{0.8}
\@namedef{res@det/zs:llama3.2-3b:binoculars/thr-dev}{-0.9126}
\@namedef{res@det/zs:llama3.2-3b:binoculars/thr-lenaware/120-160}{-0.9001}
\@namedef{res@det/zs:llama3.2-3b:binoculars/thr-lenaware/160-220}{-0.9149}
\@namedef{res@det/zs:llama3.2-3b:binoculars/thr-lenaware/220-320}{-0.9104}
\@namedef{res@det/zs:llama3.2-3b:binoculars/tpr-at-dev}{3.6}
\@namedef{res@det/zs:llama3.2-3b:binoculars/tpr-at-lenaware}{3.0}
\@namedef{res@det/zs:llama3.2-3b:binoculars/tpr-heldout-at-dev}{9.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc}{0.814}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/g31fl}{0.812}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/g35fl}{0.763}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/gemma26}{0.904}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/gemma31}{0.877}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/gptoss}{0.971}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/kazllm}{0.905}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/qwen}{0.876}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-by-gen/sherkala}{0.948}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-ci/hi}{0.828}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-ci/lo}{0.799}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-heldout}{0.902}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/auroc-len120-220}{0.818}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/g31fl}{12.1}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/g35fl}{9.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/gemma26}{19.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/gemma31}{19.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/gptoss}{55.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/kazllm}{40.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/qwen}{24.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-by-gen-at-dev/sherkala}{57.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-gray-at-dev/HP}{3.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-gray-at-dev/MH}{4.7}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-gray-at-dev/MIX}{5.1}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/flag-gray-at-dev/MT}{4.1}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-at-dev}{1.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-at-dev-ci/hi}{1.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-at-dev-ci/lo}{0.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-at-lenaware}{1.1}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-domain-at-dev/encyclopedic}{2.1}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-domain-at-dev/essay}{0.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-domain-at-dev/news}{0.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-domain-at-dev/web}{0.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-dev/120-160}{1.4}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-dev/160-220}{0.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-lenaware/120-160}{2.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-lenaware/160-220}{0.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/canon-fpr-at-dev}{0.4}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/canon-tpr-at-dev}{9.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hg-tpr-orig-at-dev}{14.9}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hgfold-tpr-at-dev}{14.9}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/latin-tpr-at-dev}{0.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/latin2021}{0.466}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/latin2021canon}{0.791}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/trunc100}{0.816}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/script/trunc50}{0.743}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/auroc}{0.816}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/fpr-at-dev}{0.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/fpr-at-devlen}{0.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/fpr-at-devlen-ci/hi}{0.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/thr-devlen}{2.0329}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/tpr-at-dev}{17.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/100/tpr-at-devlen}{16.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/auroc}{0.743}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/fpr-at-dev}{0.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/thr-devlen}{1.9898}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/tpr-at-dev}{5.3}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/short/50/tpr-at-devlen}{5.6}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/thr-dev}{2.0115}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/thr-lenaware/120-160}{1.7956}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/thr-lenaware/160-220}{1.9856}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/thr-lenaware/220-320}{2.0185}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/tpr-at-dev}{16.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/tpr-at-lenaware}{20.5}
\@namedef{res@det/zs:llama3.2-3b:obs-fdg/tpr-heldout-at-dev}{29.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc}{0.693}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/g31fl}{0.691}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/g35fl}{0.646}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/gemma26}{0.793}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/gemma31}{0.780}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/gptoss}{0.821}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/kazllm}{0.703}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/qwen}{0.777}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-by-gen/sherkala}{0.744}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-ci/hi}{0.710}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-ci/lo}{0.675}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-heldout}{0.763}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/auroc-len120-220}{0.696}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/g31fl}{5.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/g35fl}{3.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/gemma26}{11.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/gemma31}{11.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/gptoss}{24.2}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/kazllm}{9.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/qwen}{11.2}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-by-gen-at-dev/sherkala}{16.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-gray-at-dev/HP}{2.6}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-gray-at-dev/MH}{1.6}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-gray-at-dev/MIX}{3.6}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/flag-gray-at-dev/MT}{1.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-at-dev}{1.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-at-dev-ci/hi}{1.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-at-dev-ci/lo}{0.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-at-lenaware}{1.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-domain-at-dev/encyclopedic}{2.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-domain-at-dev/web}{1.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-dev/120-160}{1.1}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-dev/160-220}{1.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-lenaware/120-160}{1.1}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-lenaware/160-220}{1.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/canon-fpr-at-dev}{1.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/canon-tpr-at-dev}{4.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hg-tpr-orig-at-dev}{9.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hgfold-tpr-at-dev}{9.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/latin-fpr-at-dev}{46.9}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/latin-tpr-at-dev}{64.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/latin2021}{0.626}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/latin2021canon}{0.677}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/trunc100}{0.729}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/script/trunc50}{0.653}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/auroc}{0.729}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/fpr-at-dev}{1.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/thr-devlen}{3.9175}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/tpr-at-dev}{9.4}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/100/tpr-at-devlen}{5.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/auroc}{0.653}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/fpr-at-dev}{0.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/fpr-at-devlen}{1.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/thr-devlen}{3.4433}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/tpr-at-dev}{0.5}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/short/50/tpr-at-devlen}{2.3}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/thr-dev}{3.7773}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/thr-lenaware/120-160}{3.7980}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/thr-lenaware/160-220}{3.7877}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/thr-lenaware/220-320}{3.6950}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/tpr-at-dev}{7.1}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/tpr-at-lenaware}{7.1}
\@namedef{res@det/zs:llama3.2-3b:perf-fdg/tpr-heldout-at-dev}{12.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc}{0.731}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/g31fl}{0.807}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/g35fl}{0.769}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/gemma26}{0.619}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/gemma31}{0.642}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/gptoss}{0.563}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/kazllm}{0.477}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/qwen}{0.436}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-by-gen/sherkala}{0.808}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-ci/hi}{0.749}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-ci/lo}{0.714}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-heldout}{0.632}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/auroc-len120-220}{0.738}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/g31fl}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/g35fl}{1.1}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/gemma31}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/gptoss}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/kazllm}{1.2}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/qwen}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-by-gen-at-dev/sherkala}{1.3}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-gray-at-dev/HP}{2.6}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-gray-at-dev/MH}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-gray-at-dev/MIX}{1.2}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/flag-gray-at-dev/MT}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-at-dev}{1.4}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-at-dev-ci/hi}{2.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-at-dev-ci/lo}{0.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-at-lenaware}{1.8}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-domain-at-dev/news}{1.1}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-domain-at-dev/web}{3.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-dev/160-220}{1.5}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-lenaware/160-220}{1.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/canon-tpr-at-dev}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hg-tpr-orig-at-dev}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hgfold-tpr-at-dev}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hghum-fold-at-dev}{3.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hghum-n}{103}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/hghum-raw-at-dev}{2.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/latin2021}{0.426}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/latin2021canon}{0.699}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/trunc100}{0.674}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/script/trunc50}{0.621}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/auroc}{0.674}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/fpr-at-dev}{3.8}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/thr-devlen}{-0.5136}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/tpr-at-dev}{2.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/100/tpr-at-devlen}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/auroc}{0.621}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/fpr-at-dev}{8.4}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/fpr-at-devlen}{1.5}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/thr-devlen}{-0.4561}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/tpr-at-dev}{6.3}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/short/50/tpr-at-devlen}{0.5}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/thr-dev}{-0.5432}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/thr-lenaware/120-160}{-0.4973}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/thr-lenaware/160-220}{-0.5586}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/thr-lenaware/220-320}{-0.5672}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/tpr-at-dev}{0.9}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/tpr-at-lenaware}{0.7}
\@namedef{res@det/zs:mgpt-1.3b:binoculars/tpr-heldout-at-dev}{0.5}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc}{0.808}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/g31fl}{0.845}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/g35fl}{0.768}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/gemma26}{0.850}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/gemma31}{0.863}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/gptoss}{0.877}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/kazllm}{0.810}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/qwen}{0.762}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-by-gen/sherkala}{0.915}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-ci/hi}{0.824}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-ci/lo}{0.794}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-heldout}{0.858}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/auroc-len120-220}{0.808}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/g31fl}{10.1}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/g35fl}{5.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/gemma26}{16.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/gemma31}{15.5}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/gptoss}{27.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/kazllm}{40.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/qwen}{10.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-by-gen-at-dev/sherkala}{52.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-gray-at-dev/HP}{6.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-gray-at-dev/MH}{6.2}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-gray-at-dev/MIX}{10.6}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/flag-gray-at-dev/MT}{1.5}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-at-dev}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-at-dev-ci/hi}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-at-dev-ci/lo}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-at-lenaware}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-domain-at-dev/encyclopedic}{1.1}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-domain-at-dev/essay}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-domain-at-dev/news}{0.9}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-domain-at-dev/web}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-dev/160-220}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-lenaware/120-160}{1.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-lenaware/160-220}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/fpr-by-len-at-lenaware/220-320}{1.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/canon-fpr-at-dev}{0.2}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/canon-tpr-at-dev}{4.5}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hg-tpr-orig-at-dev}{10.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hgfold-tpr-at-dev}{10.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/latin2021}{0.341}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/latin2021canon}{0.764}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/trunc100}{0.843}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/script/trunc50}{0.774}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/auroc}{0.843}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/fpr-at-dev}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/fpr-at-devlen}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/fpr-at-devlen-ci/hi}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/thr-devlen}{1.7446}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/tpr-at-dev}{15.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/100/tpr-at-devlen}{10.4}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/auroc}{0.774}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/fpr-at-dev}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/fpr-at-devlen}{0.5}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/fpr-at-devlen-ci/hi}{1.3}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/thr-devlen}{1.7964}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/tpr-at-dev}{12.7}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/short/50/tpr-at-devlen}{7.9}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/thr-dev}{1.5616}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/thr-lenaware/120-160}{1.6026}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/thr-lenaware/160-220}{1.5600}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/thr-lenaware/220-320}{1.3547}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/tpr-at-dev}{10.0}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/tpr-at-lenaware}{9.6}
\@namedef{res@det/zs:mgpt-1.3b:obs-fdg/tpr-heldout-at-dev}{26.7}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc}{0.849}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/g31fl}{0.908}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/g35fl}{0.820}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/gemma26}{0.849}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/gemma31}{0.855}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/gptoss}{0.842}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/kazllm}{0.736}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/qwen}{0.743}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-by-gen/sherkala}{0.864}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-ci/hi}{0.863}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-ci/lo}{0.835}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-heldout}{0.832}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/auroc-len120-220}{0.859}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/g31fl}{13.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/g35fl}{6.3}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/gemma26}{9.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/gemma31}{9.5}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/gptoss}{14.5}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/kazllm}{27.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/qwen}{6.4}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-by-gen-at-dev/sherkala}{40.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-gray-at-dev/HP}{5.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-gray-at-dev/MH}{3.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-gray-at-dev/MIX}{10.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/flag-gray-at-dev/MT}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-at-dev}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-at-dev-ci/hi}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-at-dev-ci/lo}{0.3}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-at-lenaware}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-domain-at-dev/encyclopedic}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-domain-at-dev/essay}{1.4}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-domain-at-dev/web}{0.4}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-dev/120-160}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-dev/160-220}{0.4}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-dev/220-320}{2.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-lenaware/120-160}{0.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-lenaware/160-220}{0.4}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/canon-fpr-at-dev}{0.2}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/canon-tpr-at-dev}{3.3}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hg-tpr-orig-at-dev}{9.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hgfold-tpr-at-dev}{9.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hghum-fold-at-dev}{1.9}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/latin2021}{0.480}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/latin2021canon}{0.786}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/trunc100}{0.837}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/script/trunc50}{0.786}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/auroc}{0.837}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/fpr-at-dev}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/thr-devlen}{0.7593}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/tpr-at-dev}{16.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/100/tpr-at-devlen}{16.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/auroc}{0.786}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/fpr-at-dev}{3.6}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/fpr-at-devlen}{2.0}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/fpr-at-devlen-ci/hi}{3.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/thr-devlen}{1.0328}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/tpr-at-dev}{18.5}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/short/50/tpr-at-devlen}{13.2}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/thr-dev}{0.7353}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/thr-lenaware/120-160}{0.5713}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/thr-lenaware/160-220}{0.7865}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/thr-lenaware/220-320}{0.6513}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/tpr-at-dev}{9.8}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/tpr-at-lenaware}{11.3}
\@namedef{res@det/zs:mgpt-1.3b:perf-fdg/tpr-heldout-at-dev}{18.1}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc}{0.509}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/g31fl}{0.453}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/g35fl}{0.500}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/gemma26}{0.453}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/gemma31}{0.459}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/gptoss}{0.733}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/kazllm}{0.709}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/qwen}{0.545}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-by-gen/sherkala}{0.770}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-ci/hi}{0.527}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-ci/lo}{0.487}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-heldout}{0.558}
\@namedef{res@det/zs:qwen3-4b:binoculars/auroc-len120-220}{0.507}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/g31fl}{0.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/g35fl}{1.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/gemma31}{1.2}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/gptoss}{5.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/kazllm}{8.2}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/qwen}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-by-gen-at-dev/sherkala}{8.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-gray-at-dev/HP}{3.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-gray-at-dev/MH}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-gray-at-dev/MIX}{4.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/flag-gray-at-dev/MT}{0.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-at-dev-ci/hi}{1.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-at-dev-ci/lo}{0.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-at-lenaware}{1.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-domain-at-dev/encyclopedic}{1.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-domain-at-dev/essay}{1.4}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-domain-at-dev/news}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-domain-at-dev/web}{1.7}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-dev/120-160}{0.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-dev/160-220}{1.2}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-lenaware/120-160}{1.4}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-lenaware/160-220}{1.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/canon-tpr-at-dev}{0.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hg-tpr-at-dev}{0.7}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hg-tpr-orig-at-dev}{2.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hgfold-tpr-at-dev}{2.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hghum-fold-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hghum-n}{103}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/hghum-raw-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/latin2021}{0.402}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/latin2021canon}{0.460}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/trunc100}{0.559}
\@namedef{res@det/zs:qwen3-4b:binoculars/script/trunc50}{0.585}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/auroc}{0.559}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/fpr-at-dev}{1.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/thr-devlen}{-0.8596}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/tpr-at-dev}{2.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/100/tpr-at-devlen}{1.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/auroc}{0.585}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/fpr-at-dev}{4.8}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/fpr-at-devlen}{1.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/thr-devlen}{-0.8291}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/tpr-at-dev}{9.4}
\@namedef{res@det/zs:qwen3-4b:binoculars/short/50/tpr-at-devlen}{2.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/thr-dev}{-0.8722}
\@namedef{res@det/zs:qwen3-4b:binoculars/thr-lenaware/120-160}{-0.8917}
\@namedef{res@det/zs:qwen3-4b:binoculars/thr-lenaware/160-220}{-0.8772}
\@namedef{res@det/zs:qwen3-4b:binoculars/thr-lenaware/220-320}{-0.8622}
\@namedef{res@det/zs:qwen3-4b:binoculars/tpr-at-dev}{1.3}
\@namedef{res@det/zs:qwen3-4b:binoculars/tpr-at-lenaware}{2.1}
\@namedef{res@det/zs:qwen3-4b:binoculars/tpr-heldout-at-dev}{3.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc}{0.475}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/g31fl}{0.424}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/g35fl}{0.459}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/gemma26}{0.424}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/gemma31}{0.408}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/gptoss}{0.721}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/kazllm}{0.711}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/qwen}{0.500}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-by-gen/sherkala}{0.732}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-ci/hi}{0.493}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-ci/lo}{0.454}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-heldout}{0.525}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/auroc-len120-220}{0.479}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/g31fl}{0.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/g35fl}{1.5}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/gemma31}{0.6}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/gptoss}{6.5}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/kazllm}{12.9}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/qwen}{0.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-by-gen-at-dev/sherkala}{9.3}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-gray-at-dev/HP}{5.1}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-gray-at-dev/MH}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-gray-at-dev/MIX}{4.3}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/flag-gray-at-dev/MT}{0.9}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-at-dev}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-at-dev-ci/hi}{2.1}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-at-dev-ci/lo}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-at-lenaware}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-domain-at-dev/encyclopedic}{2.6}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-domain-at-dev/essay}{0.9}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-domain-at-dev/web}{1.9}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-dev/120-160}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-dev/160-220}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-dev/220-320}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-lenaware/160-220}{1.4}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/fpr-by-len-at-lenaware/220-320}{0.7}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/canon-fpr-at-dev}{0.6}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/canon-tpr-at-dev}{0.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hg-tpr-orig-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hgfold-tpr-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hghum-fold-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/latin-fpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/latin2021}{0.389}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/latin2021canon}{0.423}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/trunc100}{0.505}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/script/trunc50}{0.577}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/auroc}{0.505}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/fpr-at-dev}{1.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/fpr-at-devlen}{2.3}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/fpr-at-devlen-ci/hi}{3.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/thr-devlen}{1.5957}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/tpr-at-dev}{2.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/100/tpr-at-devlen}{2.3}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/auroc}{0.577}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/fpr-at-dev}{2.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/fpr-at-devlen}{0.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/fpr-at-devlen-ci/hi}{1.5}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/thr-devlen}{2.0041}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/tpr-at-dev}{2.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/short/50/tpr-at-devlen}{1.0}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/thr-dev}{1.7075}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/thr-lenaware/120-160}{1.5611}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/thr-lenaware/160-220}{1.6760}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/thr-lenaware/220-320}{1.9461}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/tpr-at-dev}{1.5}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/tpr-at-lenaware}{1.8}
\@namedef{res@det/zs:qwen3-4b:obs-fdg/tpr-heldout-at-dev}{4.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc}{0.718}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/g31fl}{0.695}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/g35fl}{0.660}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/gemma26}{0.856}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/gemma31}{0.812}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/gptoss}{0.936}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/kazllm}{0.863}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/qwen}{0.835}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-by-gen/sherkala}{0.909}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-ci/hi}{0.733}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-ci/lo}{0.700}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-heldout}{0.849}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/auroc-len120-220}{0.718}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/g31fl}{4.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/g35fl}{3.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/gemma26}{14.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/gemma31}{14.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/gptoss}{36.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/kazllm}{41.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/qwen}{13.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-by-gen-at-dev/sherkala}{46.7}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-gray-at-dev/HP}{0.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-gray-at-dev/MH}{0.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-gray-at-dev/MIX}{5.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/flag-gray-at-dev/MT}{3.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-at-dev}{1.9}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-at-dev-ci/hi}{2.7}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-at-dev-ci/lo}{1.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-at-lenaware}{2.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-domain-at-dev/encyclopedic}{0.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-domain-at-dev/essay}{8.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-domain-at-dev/web}{1.5}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-dev/120-160}{2.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-dev/160-220}{1.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-dev/220-320}{2.1}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-lenaware/120-160}{2.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-lenaware/160-220}{1.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/canon-fpr-at-dev}{1.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/canon-tpr-at-dev}{3.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hg-tpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hg-tpr-orig-at-dev}{8.1}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hgfold-tpr-at-dev}{8.1}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hghum-fold-at-dev}{1.9}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hghum-n}{103}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/hghum-raw-at-dev}{1.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/latin-fpr-at-dev}{0.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/latin-tpr-at-dev}{0.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/latin2021}{0.525}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/latin2021canon}{0.697}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/trunc100}{0.699}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/script/trunc50}{0.652}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/auroc}{0.699}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/fpr-at-dev}{1.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/fpr-at-devlen}{1.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/fpr-at-devlen-ci/hi}{3.1}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/thr-devlen}{-10.4742}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/tpr-at-dev}{12.7}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/100/tpr-at-devlen}{12.7}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/auroc}{0.652}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/fpr-at-dev}{38.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/fpr-at-devlen}{1.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/thr-devlen}{-5.8602}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/tpr-at-dev}{62.2}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/short/50/tpr-at-devlen}{3.6}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/thr-dev}{-10.4939}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/thr-lenaware/120-160}{-10.9480}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/thr-lenaware/160-220}{-10.6079}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/thr-lenaware/220-320}{-9.8425}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/tpr-at-dev}{7.8}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/tpr-at-lenaware}{9.3}
\@namedef{res@det/zs:qwen3-4b:perf-fdg/tpr-heldout-at-dev}{24.9}
\@namedef{res@devrep/aug/fpr}{1.3}
\@namedef{res@devrep/aug/fpr-web}{0.0}
\@namedef{res@devrep/aug/fpr50}{6.4}
\@namedef{res@devrep/aug/tpr-gemma}{100.0}
\@namedef{res@devrep/aug/tpr-indist}{98.5}
\@namedef{res@devrep/aug/tpr-kazllm}{33.3}
\@namedef{res@devrep/aug/tpr-sherkala}{57.1}
\@namedef{res@devrep/auglen-lenthr/fpr}{1.5}
\@namedef{res@devrep/auglen-lenthr/fpr-web}{0.9}
\@namedef{res@devrep/auglen-lenthr/fpr50}{1.3}
\@namedef{res@devrep/auglen-lenthr/tpr-gemma}{100.0}
\@namedef{res@devrep/auglen-lenthr/tpr-indist}{98.5}
\@namedef{res@devrep/auglen-lenthr/tpr-kazllm}{33.3}
\@namedef{res@devrep/auglen-lenthr/tpr-sherkala}{57.1}
\@namedef{res@devrep/auglen/fpr}{1.5}
\@namedef{res@devrep/auglen/fpr-web}{0.9}
\@namedef{res@devrep/auglen/fpr50}{3.3}
\@namedef{res@devrep/auglen/tpr-gemma}{100.0}
\@namedef{res@devrep/auglen/tpr-indist}{98.5}
\@namedef{res@devrep/auglen/tpr-kazllm}{33.3}
\@namedef{res@devrep/auglen/tpr-sherkala}{57.1}
\@namedef{res@devrep/base/fpr}{1.3}
\@namedef{res@devrep/base/fpr-web}{0.0}
\@namedef{res@devrep/base/fpr50}{2.3}
\@namedef{res@devrep/base/tpr-gemma}{100.0}
\@namedef{res@devrep/base/tpr-indist}{95.6}
\@namedef{res@devrep/base/tpr-kazllm}{33.3}
\@namedef{res@devrep/base/tpr-sherkala}{57.1}
\@namedef{res@devrep/base05/fpr}{9.5}
\@namedef{res@devrep/base05/fpr-web}{11.7}
\@namedef{res@devrep/base05/fpr50}{21.7}
\@namedef{res@devrep/base05/tpr-gemma}{100.0}
\@namedef{res@devrep/base05/tpr-indist}{99.3}
\@namedef{res@devrep/base05/tpr-kazllm}{77.8}
\@namedef{res@devrep/base05/tpr-sherkala}{78.6}
\@namedef{res@devrep/combo-aug/fpr}{1.3}
\@namedef{res@devrep/combo-aug/fpr-web}{0.9}
\@namedef{res@devrep/combo-aug/fpr50}{2.6}
\@namedef{res@devrep/combo-aug/tpr-gemma}{91.4}
\@namedef{res@devrep/combo-aug/tpr-indist}{89.7}
\@namedef{res@devrep/combo-aug/tpr-kazllm}{55.6}
\@namedef{res@devrep/combo-aug/tpr-sherkala}{64.3}
\@namedef{res@devrep/combo-auglen/fpr}{1.5}
\@namedef{res@devrep/combo-auglen/fpr-web}{0.9}
\@namedef{res@devrep/combo-auglen/fpr50}{2.3}
\@namedef{res@devrep/combo-auglen/tpr-gemma}{96.6}
\@namedef{res@devrep/combo-auglen/tpr-indist}{89.0}
\@namedef{res@devrep/combo-auglen/tpr-kazllm}{63.0}
\@namedef{res@devrep/combo-auglen/tpr-sherkala}{64.3}
\@namedef{res@devrep/combo-base/fpr}{1.5}
\@namedef{res@devrep/combo-base/fpr-web}{0.9}
\@namedef{res@devrep/combo-base/fpr50}{2.6}
\@namedef{res@devrep/combo-base/tpr-gemma}{91.4}
\@namedef{res@devrep/combo-base/tpr-indist}{86.0}
\@namedef{res@devrep/combo-base/tpr-kazllm}{51.9}
\@namedef{res@devrep/combo-base/tpr-sherkala}{64.3}
\@namedef{res@devrep/combo/fpr}{1.5}
\@namedef{res@devrep/combo/fpr-web}{0.9}
\@namedef{res@devrep/combo/fpr50}{2.3}
\@namedef{res@devrep/combo/tpr-gemma}{96.6}
\@namedef{res@devrep/combo/tpr-indist}{89.0}
\@namedef{res@devrep/combo/tpr-kazllm}{63.0}
\@namedef{res@devrep/combo/tpr-sherkala}{64.3}
\@namedef{res@devrep/kz/fpr}{1.5}
\@namedef{res@devrep/kz/fpr-web}{1.8}
\@namedef{res@devrep/kz/fpr50}{4.3}
\@namedef{res@devrep/kz/tpr-gemma}{98.3}
\@namedef{res@devrep/kz/tpr-indist}{97.1}
\@namedef{res@devrep/kz/tpr-kazllm}{37.0}
\@namedef{res@devrep/kz/tpr-sherkala}{46.4}
\@namedef{res@devrep/kzlen/fpr}{2.8}
\@namedef{res@devrep/kzlen/fpr-web}{4.5}
\@namedef{res@devrep/kzlen/fpr50}{2.0}
\@namedef{res@devrep/kzlen/tpr-gemma}{63.8}
\@namedef{res@devrep/kzlen/tpr-indist}{71.3}
\@namedef{res@devrep/kzlen/tpr-kazllm}{37.0}
\@namedef{res@devrep/kzlen/tpr-sherkala}{46.4}
\@namedef{res@devrep/kznoaug/fpr}{1.0}
\@namedef{res@devrep/kznoaug/fpr-web}{0.0}
\@namedef{res@devrep/kznoaug/fpr50}{6.1}
\@namedef{res@devrep/kznoaug/tpr-gemma}{96.6}
\@namedef{res@devrep/kznoaug/tpr-indist}{97.8}
\@namedef{res@devrep/kznoaug/tpr-kazllm}{63.0}
\@namedef{res@devrep/kznoaug/tpr-sherkala}{60.7}
\@namedef{res@devrep/n-fit-clusters}{six}
\@namedef{res@devrep/n-h}{391}
\@namedef{res@devrep/n-m}{249}
\@namedef{res@devrep/n/fpr}{391}
\@namedef{res@devrep/n/fpr-web}{111}
\@namedef{res@devrep/n/fpr50}{391}
\@namedef{res@devrep/n/tpr-gemma}{58}
\@namedef{res@devrep/n/tpr-indist}{136}
\@namedef{res@devrep/n/tpr-kazllm}{27}
\@namedef{res@devrep/n/tpr-sherkala}{28}
\@namedef{res@ext/antiplagiat-claim}{1}
\@namedef{res@ext/antiplagiat-date}{7 Apr 2025}
\@namedef{res@ext/cc100-years}{2018}
\@namedef{res@ext/coling25-kk-samples}{2,471}
\@namedef{res@ext/encoder-params}{0.28}
\@namedef{res@ext/human-study-acc}{79.67}
\@namedef{res@ext/human-study-pairs}{300}
\@namedef{res@ext/max-languages}{22}
\@namedef{res@ext/statcounter-month}{September 2026}
\@namedef{res@ext/statcounter-share}{94}
\@namedef{res@ext/turnitin-accessed}{11 Oct 2026}
\@namedef{res@ext/turnitin-langs}{English, Spanish, Japanese, Arabic, Dutch, German and Turkish}
\@namedef{res@ext/turnitin-n-langs}{seven}
\@namedef{res@ext/wiki-dump-date}{1 May 2022}
\@namedef{res@ext/wiki-import-year}{2011}
\@namedef{res@ext/zs-params}{1.3B--5.1B}
\@namedef{res@falseflags/base/0.5/per1000}{76}
\@namedef{res@falseflags/base/dev/per1000}{8}
\@namedef{res@falseflags/combo-auglen+bino/dev/per1000}{9}
\@namedef{res@falseflags/ots-desklib-deberta/0.5/per1000}{593}
\@namedef{res@falseflags/ots-fakespot-roberta/0.5/per1000}{255}
\@namedef{res@falseflags/ots-hc3-roberta/0.5/per1000}{0}
\@namedef{res@falseflags/ots-openai-roberta/0.5/per1000}{118}
\@namedef{res@falseflags/ots-tmr-roberta/0.5/per1000}{814}
\@namedef{res@fdr/base/0.5/5}{60}
\@namedef{res@fdr/base/dev/5}{15}
\@namedef{res@fdr/combo-auglen+bino/dev/5}{17}
\@namedef{res@fdr/ots-desklib-deberta/0.5/5}{94}
\@namedef{res@fdr/ots-fakespot-roberta/0.5/5}{93}
\@namedef{res@fdr/ots-hc3-roberta/0.5/5}{--}
\@namedef{res@fdr/ots-openai-roberta/0.5/5}{92}
\@namedef{res@fdr/ots-tmr-roberta/0.5/5}{97}
\@namedef{res@flag/all/argmin-global}{Qwen3.8-27B}
\@namedef{res@flag/all/min-global}{85.6}
\@namedef{res@flag/alllen/argmin-global}{gpt-oss-120b}
\@namedef{res@flag/alllen/min-global}{91.1}
\@namedef{res@flag/aug/argmin-global}{gpt-oss-120b}
\@namedef{res@flag/aug/min-global}{98.4}
\@namedef{res@flag/auglen/argmin-global}{gpt-oss-120b}
\@namedef{res@flag/auglen/min-global}{99.2}
\@namedef{res@flag/base/argmin-global}{Qwen3.8-27B}
\@namedef{res@flag/base/min-global}{96.8}
\@namedef{res@flag/kz/argmin-global}{Qwen3.8-27B}
\@namedef{res@flag/kz/min-global}{98.4}
\@namedef{res@flag/kzlen/argmin-global}{Gemma 4 31B}
\@namedef{res@flag/kzlen/min-global}{49.4}
\@namedef{res@flag/kznoaug/argmin-global}{Gemini 3.5 Flash-Lite}
\@namedef{res@flag/kznoaug/min-global}{97.7}
\@namedef{res@flag/xlmr/argmin-global}{gpt-oss-120b}
\@namedef{res@flag/xlmr/min-global}{97.6}
\@namedef{res@len/h-median}{175}
\@namedef{res@len/h-under120}{0.5}
\@namedef{res@len/kazllm-median}{141}
\@namedef{res@len/kazllm-under120}{34.0}
\@namedef{res@len/m-median}{153}
\@namedef{res@len/m-under120}{18.5}
\@namedef{res@len/sherkala-median}{112}
\@namedef{res@len/sherkala-under120}{64.4}
\@namedef{res@lenratio/argmin}{Sherkala-8B-Chat}
\@namedef{res@lenratio/g31fl/median}{80}
\@namedef{res@lenratio/g35fl/median}{74}
\@namedef{res@lenratio/gemma26/median}{77}
\@namedef{res@lenratio/gemma31/median}{76}
\@namedef{res@lenratio/gptoss/median}{84}
\@namedef{res@lenratio/kazllm/median}{72}
\@namedef{res@lenratio/max}{88}
\@namedef{res@lenratio/min}{53}
\@namedef{res@lenratio/qwen/median}{88}
\@namedef{res@lenratio/sherkala/median}{53}
\@namedef{res@ling/0/d}{+0.50}
\@namedef{res@ling/0/h}{0.92}
\@namedef{res@ling/0/m}{0.96}
\@namedef{res@ling/0/name}{MATTR(50)}
\@namedef{res@ling/0/q}{6e-292}
\@namedef{res@ling/1/d}{+0.27}
\@namedef{res@ling/1/h}{13.31}
\@namedef{res@ling/1/m}{15.30}
\@namedef{res@ling/1/name}{mean sentence length}
\@namedef{res@ling/1/q}{1e-87}
\@namedef{res@ling/2/d}{-0.62}
\@namedef{res@ling/2/h}{6.26}
\@namedef{res@ling/2/m}{4.09}
\@namedef{res@ling/2/name}{sentence length SD}
\@namedef{res@ling/2/q}{0e+00}
\@namedef{res@ling/3/d}{+0.12}
\@namedef{res@ling/3/h}{0.00}
\@namedef{res@ling/3/m}{0.00}
\@namedef{res@ling/3/name}{'болып табылады' per 1k words}
\@namedef{res@ling/3/q}{1e-40}
\@namedef{res@ling/4/d}{+0.37}
\@namedef{res@ling/4/h}{0.15}
\@namedef{res@ling/4/m}{0.16}
\@namedef{res@ling/4/name}{Kazakh-specific letter share}
\@namedef{res@ling/4/q}{1e-160}
\@namedef{res@ling/5/d}{+0.27}
\@namedef{res@ling/5/h}{6.68}
\@namedef{res@ling/5/m}{6.93}
\@namedef{res@ling/5/name}{mean word length}
\@namedef{res@ling/5/q}{3e-84}
\@namedef{res@ling/6/d}{+0.11}
\@namedef{res@ling/6/h}{0.91}
\@namedef{res@ling/6/m}{1.00}
\@namedef{res@ling/6/name}{commas per sentence}
\@namedef{res@ling/6/q}{1e-14}
\@namedef{res@ling/7/d}{-0.29}
\@namedef{res@ling/7/h}{3.83}
\@namedef{res@ling/7/m}{2.78}
\@namedef{res@ling/7/name}{-ған/-ген participles per 100 words}
\@namedef{res@ling/7/q}{2e-96}
\@namedef{res@ling/8/d}{+0.17}
\@namedef{res@ling/8/h}{0.85}
\@namedef{res@ling/8/m}{1.39}
\@namedef{res@ling/8/name}{'және' per 100 words}
\@namedef{res@ling/8/q}{7e-38}
\@namedef{res@ling/n-human}{3,811}
\@namedef{res@ling/n-machine}{3,363}
\@namedef{res@logo/min-global-out}{94.4}
\@namedef{res@ots/desklib-deberta/auroc}{0.537}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/g31fl}{0.515}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/g35fl}{0.568}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/gemma26}{0.491}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/gemma31}{0.471}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/gptoss}{0.498}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/kazllm}{0.610}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/qwen}{0.539}
\@namedef{res@ots/desklib-deberta/auroc-by-gen/sherkala}{0.562}
\@namedef{res@ots/desklib-deberta/auroc-ci/hi}{0.556}
\@namedef{res@ots/desklib-deberta/auroc-ci/lo}{0.516}
\@namedef{res@ots/desklib-deberta/auroc-heldout}{0.518}
\@namedef{res@ots/desklib-deberta/auroc-len120-220}{0.533}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/g31fl}{65.4}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/g35fl}{73.4}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/gemma26}{62.3}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/gemma31}{62.5}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/gptoss}{62.9}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/kazllm}{72.9}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/qwen}{67.2}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-0.5/sherkala}{69.3}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/g31fl}{0.2}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/g35fl}{0.6}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/gemma31}{0.0}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/gptoss}{0.0}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/kazllm}{1.2}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/qwen}{0.0}
\@namedef{res@ots/desklib-deberta/flag-by-gen-at-dev/sherkala}{1.3}
\@namedef{res@ots/desklib-deberta/flag-gray-at-0.5/HP}{43.6}
\@namedef{res@ots/desklib-deberta/flag-gray-at-0.5/MH}{78.1}
\@namedef{res@ots/desklib-deberta/flag-gray-at-0.5/MIX}{63.4}
\@namedef{res@ots/desklib-deberta/flag-gray-at-0.5/MT}{64.3}
\@namedef{res@ots/desklib-deberta/flag-gray-at-dev/HP}{0.0}
\@namedef{res@ots/desklib-deberta/flag-gray-at-dev/MH}{0.0}
\@namedef{res@ots/desklib-deberta/flag-gray-at-dev/MIX}{1.8}
\@namedef{res@ots/desklib-deberta/flag-gray-at-dev/MT}{1.8}
\@namedef{res@ots/desklib-deberta/fpr-at-0.5}{59.3}
\@namedef{res@ots/desklib-deberta/fpr-at-dev}{2.5}
\@namedef{res@ots/desklib-deberta/fpr-at-dev-ci/hi}{3.3}
\@namedef{res@ots/desklib-deberta/fpr-at-dev-ci/lo}{1.8}
\@namedef{res@ots/desklib-deberta/fpr-at-lenaware}{3.4}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-0.5/encyclopedic}{48.3}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-0.5/essay}{79.6}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-0.5/news}{56.8}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-0.5/web}{61.5}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-dev/encyclopedic}{1.1}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-dev/essay}{13.0}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@ots/desklib-deberta/fpr-by-domain-at-dev/web}{1.1}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-0.5/120-160}{52.1}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-0.5/160-220}{62.1}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-0.5/220-320}{56.6}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-dev/120-160}{0.9}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-dev/160-220}{3.0}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-dev/220-320}{2.8}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-lenaware/160-220}{3.3}
\@namedef{res@ots/desklib-deberta/fpr-by-len-at-lenaware/220-320}{8.4}
\@namedef{res@ots/desklib-deberta/script/canon-fpr-at-dev}{2.8}
\@namedef{res@ots/desklib-deberta/script/canon-tpr-at-dev}{0.5}
\@namedef{res@ots/desklib-deberta/script/hg-tpr-at-dev}{0.0}
\@namedef{res@ots/desklib-deberta/script/hg-tpr-orig-at-dev}{0.7}
\@namedef{res@ots/desklib-deberta/script/hgfold-tpr-at-dev}{0.7}
\@namedef{res@ots/desklib-deberta/script/hghum-fold-at-dev}{1.0}
\@namedef{res@ots/desklib-deberta/script/hghum-n}{103}
\@namedef{res@ots/desklib-deberta/script/hghum-raw-at-dev}{1.0}
\@namedef{res@ots/desklib-deberta/script/latin-fpr-at-dev}{0.0}
\@namedef{res@ots/desklib-deberta/script/latin-tpr-at-dev}{0.0}
\@namedef{res@ots/desklib-deberta/script/latin2021}{0.579}
\@namedef{res@ots/desklib-deberta/script/latin2021canon}{0.486}
\@namedef{res@ots/desklib-deberta/script/trunc100}{0.538}
\@namedef{res@ots/desklib-deberta/script/trunc50}{0.542}
\@namedef{res@ots/desklib-deberta/short/100/auroc}{0.538}
\@namedef{res@ots/desklib-deberta/short/100/fpr-at-0.5}{60.4}
\@namedef{res@ots/desklib-deberta/short/100/fpr-at-dev}{1.3}
\@namedef{res@ots/desklib-deberta/short/100/fpr-at-devlen}{1.5}
\@namedef{res@ots/desklib-deberta/short/100/fpr-at-devlen-ci/hi}{2.8}
\@namedef{res@ots/desklib-deberta/short/100/fpr-at-devlen-ci/lo}{0.5}
\@namedef{res@ots/desklib-deberta/short/100/thr-devlen}{0.9678}
\@namedef{res@ots/desklib-deberta/short/100/tpr-at-0.5}{71.3}
\@namedef{res@ots/desklib-deberta/short/100/tpr-at-dev}{0.5}
\@namedef{res@ots/desklib-deberta/short/100/tpr-at-devlen}{0.8}
\@namedef{res@ots/desklib-deberta/short/50/auroc}{0.542}
\@namedef{res@ots/desklib-deberta/short/50/fpr-at-0.5}{82.0}
\@namedef{res@ots/desklib-deberta/short/50/fpr-at-dev}{3.6}
\@namedef{res@ots/desklib-deberta/short/50/fpr-at-devlen}{1.8}
\@namedef{res@ots/desklib-deberta/short/50/fpr-at-devlen-ci/hi}{3.3}
\@namedef{res@ots/desklib-deberta/short/50/fpr-at-devlen-ci/lo}{0.8}
\@namedef{res@ots/desklib-deberta/short/50/thr-devlen}{0.9845}
\@namedef{res@ots/desklib-deberta/short/50/tpr-at-0.5}{85.8}
\@namedef{res@ots/desklib-deberta/short/50/tpr-at-dev}{1.8}
\@namedef{res@ots/desklib-deberta/short/50/tpr-at-devlen}{0.0}
\@namedef{res@ots/desklib-deberta/thr-dev}{0.9702}
\@namedef{res@ots/desklib-deberta/thr-lenaware/120-160}{0.9621}
\@namedef{res@ots/desklib-deberta/thr-lenaware/160-220}{0.9677}
\@namedef{res@ots/desklib-deberta/thr-lenaware/220-320}{0.9208}
\@namedef{res@ots/desklib-deberta/tpr-at-0.5}{68.6}
\@namedef{res@ots/desklib-deberta/tpr-at-dev}{0.3}
\@namedef{res@ots/desklib-deberta/tpr-at-lenaware}{0.7}
\@namedef{res@ots/desklib-deberta/tpr-heldout-at-0.5}{65.6}
\@namedef{res@ots/desklib-deberta/tpr-heldout-at-dev}{0.5}
\@namedef{res@ots/fakespot-roberta/auroc}{0.621}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/g31fl}{0.613}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/g35fl}{0.620}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/gemma26}{0.584}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/gemma31}{0.624}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/gptoss}{0.629}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/kazllm}{0.624}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/qwen}{0.655}
\@namedef{res@ots/fakespot-roberta/auroc-by-gen/sherkala}{0.676}
\@namedef{res@ots/fakespot-roberta/auroc-ci/hi}{0.644}
\@namedef{res@ots/fakespot-roberta/auroc-ci/lo}{0.604}
\@namedef{res@ots/fakespot-roberta/auroc-heldout}{0.623}
\@namedef{res@ots/fakespot-roberta/auroc-len120-220}{0.623}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/g31fl}{34.6}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/g35fl}{33.5}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/gemma26}{29.8}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/gemma31}{35.1}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/gptoss}{37.9}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/kazllm}{42.4}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/qwen}{41.6}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-0.5/sherkala}{46.7}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/g31fl}{0.8}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/g35fl}{1.9}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/gemma26}{0.9}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/gemma31}{1.2}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/gptoss}{0.8}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/kazllm}{2.4}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/qwen}{1.6}
\@namedef{res@ots/fakespot-roberta/flag-by-gen-at-dev/sherkala}{1.3}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-0.5/HP}{19.2}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-0.5/MH}{32.8}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-0.5/MIX}{37.0}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-0.5/MT}{27.2}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-dev/HP}{0.0}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-dev/MH}{1.6}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-dev/MIX}{3.8}
\@namedef{res@ots/fakespot-roberta/flag-gray-at-dev/MT}{1.2}
\@namedef{res@ots/fakespot-roberta/fpr-at-0.5}{25.5}
\@namedef{res@ots/fakespot-roberta/fpr-at-dev}{2.0}
\@namedef{res@ots/fakespot-roberta/fpr-at-dev-ci/hi}{2.7}
\@namedef{res@ots/fakespot-roberta/fpr-at-dev-ci/lo}{1.4}
\@namedef{res@ots/fakespot-roberta/fpr-at-lenaware}{2.4}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-0.5/encyclopedic}{27.2}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-0.5/essay}{33.3}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-0.5/news}{21.3}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-0.5/web}{24.7}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-dev/encyclopedic}{1.3}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-dev/essay}{2.8}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-dev/news}{2.1}
\@namedef{res@ots/fakespot-roberta/fpr-by-domain-at-dev/web}{1.9}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-0.5/120-160}{20.6}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-0.5/160-220}{27.1}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-0.5/220-320}{25.9}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-dev/120-160}{1.7}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-dev/160-220}{2.2}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-lenaware/120-160}{1.7}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-lenaware/160-220}{2.7}
\@namedef{res@ots/fakespot-roberta/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@ots/fakespot-roberta/script/canon-fpr-at-dev}{2.0}
\@namedef{res@ots/fakespot-roberta/script/canon-tpr-at-dev}{2.3}
\@namedef{res@ots/fakespot-roberta/script/hg-tpr-at-dev}{1.2}
\@namedef{res@ots/fakespot-roberta/script/hg-tpr-orig-at-dev}{1.0}
\@namedef{res@ots/fakespot-roberta/script/hgfold-tpr-at-dev}{1.0}
\@namedef{res@ots/fakespot-roberta/script/hghum-fold-at-dev}{1.0}
\@namedef{res@ots/fakespot-roberta/script/hghum-n}{103}
\@namedef{res@ots/fakespot-roberta/script/hghum-raw-at-dev}{1.0}
\@namedef{res@ots/fakespot-roberta/script/latin-fpr-at-dev}{0.0}
\@namedef{res@ots/fakespot-roberta/script/latin-tpr-at-dev}{0.3}
\@namedef{res@ots/fakespot-roberta/script/latin2021}{0.701}
\@namedef{res@ots/fakespot-roberta/script/latin2021canon}{0.634}
\@namedef{res@ots/fakespot-roberta/script/trunc100}{0.580}
\@namedef{res@ots/fakespot-roberta/script/trunc50}{0.470}
\@namedef{res@ots/fakespot-roberta/short/100/auroc}{0.580}
\@namedef{res@ots/fakespot-roberta/short/100/fpr-at-0.5}{36.5}
\@namedef{res@ots/fakespot-roberta/short/100/fpr-at-dev}{2.3}
\@namedef{res@ots/fakespot-roberta/short/100/fpr-at-devlen}{2.3}
\@namedef{res@ots/fakespot-roberta/short/100/fpr-at-devlen-ci/hi}{4.1}
\@namedef{res@ots/fakespot-roberta/short/100/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@ots/fakespot-roberta/short/100/thr-devlen}{0.9886}
\@namedef{res@ots/fakespot-roberta/short/100/tpr-at-0.5}{46.2}
\@namedef{res@ots/fakespot-roberta/short/100/tpr-at-dev}{1.3}
\@namedef{res@ots/fakespot-roberta/short/100/tpr-at-devlen}{1.0}
\@namedef{res@ots/fakespot-roberta/short/50/auroc}{0.470}
\@namedef{res@ots/fakespot-roberta/short/50/fpr-at-0.5}{87.6}
\@namedef{res@ots/fakespot-roberta/short/50/fpr-at-dev}{57.6}
\@namedef{res@ots/fakespot-roberta/short/50/fpr-at-devlen}{1.5}
\@namedef{res@ots/fakespot-roberta/short/50/fpr-at-devlen-ci/hi}{3.0}
\@namedef{res@ots/fakespot-roberta/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@ots/fakespot-roberta/short/50/thr-devlen}{0.9992}
\@namedef{res@ots/fakespot-roberta/short/50/tpr-at-0.5}{84.3}
\@namedef{res@ots/fakespot-roberta/short/50/tpr-at-dev}{55.8}
\@namedef{res@ots/fakespot-roberta/short/50/tpr-at-devlen}{0.5}
\@namedef{res@ots/fakespot-roberta/thr-dev}{0.9852}
\@namedef{res@ots/fakespot-roberta/thr-lenaware/120-160}{0.9872}
\@namedef{res@ots/fakespot-roberta/thr-lenaware/160-220}{0.9826}
\@namedef{res@ots/fakespot-roberta/thr-lenaware/220-320}{0.9604}
\@namedef{res@ots/fakespot-roberta/tpr-at-0.5}{35.2}
\@namedef{res@ots/fakespot-roberta/tpr-at-dev}{1.3}
\@namedef{res@ots/fakespot-roberta/tpr-at-lenaware}{1.3}
\@namedef{res@ots/fakespot-roberta/tpr-heldout-at-0.5}{37.1}
\@namedef{res@ots/fakespot-roberta/tpr-heldout-at-dev}{1.4}
\@namedef{res@ots/hc3-roberta/auroc}{0.499}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/g31fl}{0.543}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/g35fl}{0.452}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/gemma26}{0.576}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/gemma31}{0.482}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/gptoss}{0.459}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/kazllm}{0.522}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/qwen}{0.554}
\@namedef{res@ots/hc3-roberta/auroc-by-gen/sherkala}{0.517}
\@namedef{res@ots/hc3-roberta/auroc-ci/hi}{0.519}
\@namedef{res@ots/hc3-roberta/auroc-ci/lo}{0.476}
\@namedef{res@ots/hc3-roberta/auroc-heldout}{0.520}
\@namedef{res@ots/hc3-roberta/auroc-len120-220}{0.499}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/g31fl}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/g35fl}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/gemma26}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/gemma31}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/gptoss}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/kazllm}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/qwen}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-0.5/sherkala}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/g31fl}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/g35fl}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/gemma26}{0.9}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/gemma31}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/gptoss}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/kazllm}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/qwen}{0.0}
\@namedef{res@ots/hc3-roberta/flag-by-gen-at-dev/sherkala}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-0.5/HP}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-0.5/MH}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-0.5/MIX}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-0.5/MT}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-dev/HP}{2.6}
\@namedef{res@ots/hc3-roberta/flag-gray-at-dev/MH}{0.0}
\@namedef{res@ots/hc3-roberta/flag-gray-at-dev/MIX}{0.4}
\@namedef{res@ots/hc3-roberta/flag-gray-at-dev/MT}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-at-dev}{0.5}
\@namedef{res@ots/hc3-roberta/fpr-at-dev-ci/hi}{0.9}
\@namedef{res@ots/hc3-roberta/fpr-at-dev-ci/lo}{0.2}
\@namedef{res@ots/hc3-roberta/fpr-at-lenaware}{1.2}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-0.5/encyclopedic}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-0.5/essay}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-0.5/news}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-0.5/web}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-dev/essay}{1.4}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-dev/news}{0.2}
\@namedef{res@ots/hc3-roberta/fpr-by-domain-at-dev/web}{0.6}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-0.5/120-160}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-0.5/160-220}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-0.5/220-320}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-dev/120-160}{0.0}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-dev/160-220}{0.7}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-dev/220-320}{0.7}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-lenaware/120-160}{2.6}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-lenaware/160-220}{0.7}
\@namedef{res@ots/hc3-roberta/fpr-by-len-at-lenaware/220-320}{2.1}
\@namedef{res@ots/hc3-roberta/script/canon-fpr-at-dev}{0.4}
\@namedef{res@ots/hc3-roberta/script/canon-tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/hg-tpr-at-dev}{0.5}
\@namedef{res@ots/hc3-roberta/script/hg-tpr-orig-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/hgfold-tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/hghum-fold-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/hghum-n}{103}
\@namedef{res@ots/hc3-roberta/script/hghum-raw-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/latin-fpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/latin-tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/script/latin2021}{0.522}
\@namedef{res@ots/hc3-roberta/script/latin2021canon}{0.498}
\@namedef{res@ots/hc3-roberta/script/trunc100}{0.556}
\@namedef{res@ots/hc3-roberta/script/trunc50}{0.558}
\@namedef{res@ots/hc3-roberta/short/100/auroc}{0.556}
\@namedef{res@ots/hc3-roberta/short/100/fpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/short/100/fpr-at-dev}{1.3}
\@namedef{res@ots/hc3-roberta/short/100/fpr-at-devlen}{2.3}
\@namedef{res@ots/hc3-roberta/short/100/fpr-at-devlen-ci/hi}{4.1}
\@namedef{res@ots/hc3-roberta/short/100/fpr-at-devlen-ci/lo}{1.0}
\@namedef{res@ots/hc3-roberta/short/100/thr-devlen}{0.0080}
\@namedef{res@ots/hc3-roberta/short/100/tpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/short/100/tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/short/100/tpr-at-devlen}{0.5}
\@namedef{res@ots/hc3-roberta/short/50/auroc}{0.558}
\@namedef{res@ots/hc3-roberta/short/50/fpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/short/50/fpr-at-dev}{1.0}
\@namedef{res@ots/hc3-roberta/short/50/fpr-at-devlen}{1.0}
\@namedef{res@ots/hc3-roberta/short/50/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@ots/hc3-roberta/short/50/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@ots/hc3-roberta/short/50/thr-devlen}{0.0132}
\@namedef{res@ots/hc3-roberta/short/50/tpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/short/50/tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/short/50/tpr-at-devlen}{0.0}
\@namedef{res@ots/hc3-roberta/thr-dev}{0.0131}
\@namedef{res@ots/hc3-roberta/thr-lenaware/120-160}{0.0069}
\@namedef{res@ots/hc3-roberta/thr-lenaware/160-220}{0.0145}
\@namedef{res@ots/hc3-roberta/thr-lenaware/220-320}{0.0073}
\@namedef{res@ots/hc3-roberta/tpr-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/tpr-at-dev}{0.0}
\@namedef{res@ots/hc3-roberta/tpr-at-lenaware}{0.5}
\@namedef{res@ots/hc3-roberta/tpr-heldout-at-0.5}{0.0}
\@namedef{res@ots/hc3-roberta/tpr-heldout-at-dev}{0.2}
\@namedef{res@ots/max-essay-fpr}{79.6}
\@namedef{res@ots/max-tpr-dev}{1.3}
\@namedef{res@ots/maxfpr}{81.4}
\@namedef{res@ots/n}{five}
\@namedef{res@ots/openai-roberta/auroc}{0.650}
\@namedef{res@ots/openai-roberta/auroc-by-gen/g31fl}{0.645}
\@namedef{res@ots/openai-roberta/auroc-by-gen/g35fl}{0.646}
\@namedef{res@ots/openai-roberta/auroc-by-gen/gemma26}{0.624}
\@namedef{res@ots/openai-roberta/auroc-by-gen/gemma31}{0.587}
\@namedef{res@ots/openai-roberta/auroc-by-gen/gptoss}{0.657}
\@namedef{res@ots/openai-roberta/auroc-by-gen/kazllm}{0.584}
\@namedef{res@ots/openai-roberta/auroc-by-gen/qwen}{0.675}
\@namedef{res@ots/openai-roberta/auroc-by-gen/sherkala}{0.581}
\@namedef{res@ots/openai-roberta/auroc-ci/hi}{0.666}
\@namedef{res@ots/openai-roberta/auroc-ci/lo}{0.630}
\@namedef{res@ots/openai-roberta/auroc-heldout}{0.595}
\@namedef{res@ots/openai-roberta/auroc-len120-220}{0.654}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/g31fl}{18.5}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/g35fl}{19.3}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/gemma26}{22.8}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/gemma31}{14.9}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/gptoss}{25.0}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/kazllm}{10.6}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/qwen}{20.0}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-0.5/sherkala}{16.0}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/g31fl}{0.8}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/g35fl}{1.3}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/gemma31}{0.0}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/gptoss}{0.8}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/kazllm}{1.2}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/qwen}{1.6}
\@namedef{res@ots/openai-roberta/flag-by-gen-at-dev/sherkala}{2.7}
\@namedef{res@ots/openai-roberta/flag-gray-at-0.5/HP}{3.8}
\@namedef{res@ots/openai-roberta/flag-gray-at-0.5/MH}{25.0}
\@namedef{res@ots/openai-roberta/flag-gray-at-0.5/MIX}{12.5}
\@namedef{res@ots/openai-roberta/flag-gray-at-0.5/MT}{12.3}
\@namedef{res@ots/openai-roberta/flag-gray-at-dev/HP}{0.0}
\@namedef{res@ots/openai-roberta/flag-gray-at-dev/MH}{0.0}
\@namedef{res@ots/openai-roberta/flag-gray-at-dev/MIX}{0.8}
\@namedef{res@ots/openai-roberta/flag-gray-at-dev/MT}{1.5}
\@namedef{res@ots/openai-roberta/fpr-at-0.5}{11.8}
\@namedef{res@ots/openai-roberta/fpr-at-dev}{1.6}
\@namedef{res@ots/openai-roberta/fpr-at-dev-ci/hi}{2.2}
\@namedef{res@ots/openai-roberta/fpr-at-dev-ci/lo}{1.0}
\@namedef{res@ots/openai-roberta/fpr-at-lenaware}{3.5}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-0.5/encyclopedic}{7.1}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-0.5/essay}{22.7}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-0.5/news}{11.5}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-0.5/web}{10.8}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-dev/encyclopedic}{0.3}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-dev/essay}{5.6}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-dev/news}{1.1}
\@namedef{res@ots/openai-roberta/fpr-by-domain-at-dev/web}{1.3}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-0.5/120-160}{8.9}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-0.5/160-220}{12.0}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-0.5/220-320}{16.8}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-dev/120-160}{0.6}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-dev/160-220}{1.6}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-dev/220-320}{3.5}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-lenaware/120-160}{9.7}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-lenaware/160-220}{1.2}
\@namedef{res@ots/openai-roberta/fpr-by-len-at-lenaware/220-320}{4.9}
\@namedef{res@ots/openai-roberta/script/canon-fpr-at-dev}{2.2}
\@namedef{res@ots/openai-roberta/script/canon-tpr-at-dev}{0.8}
\@namedef{res@ots/openai-roberta/script/hg-tpr-at-dev}{0.0}
\@namedef{res@ots/openai-roberta/script/hg-tpr-orig-at-dev}{0.7}
\@namedef{res@ots/openai-roberta/script/hgfold-tpr-at-dev}{0.7}
\@namedef{res@ots/openai-roberta/script/hghum-fold-at-dev}{7.8}
\@namedef{res@ots/openai-roberta/script/hghum-n}{103}
\@namedef{res@ots/openai-roberta/script/hghum-raw-at-dev}{9.7}
\@namedef{res@ots/openai-roberta/script/latin-fpr-at-dev}{15.3}
\@namedef{res@ots/openai-roberta/script/latin-tpr-at-dev}{9.3}
\@namedef{res@ots/openai-roberta/script/latin2021}{0.496}
\@namedef{res@ots/openai-roberta/script/latin2021canon}{0.635}
\@namedef{res@ots/openai-roberta/script/trunc100}{0.668}
\@namedef{res@ots/openai-roberta/script/trunc50}{0.668}
\@namedef{res@ots/openai-roberta/short/100/auroc}{0.668}
\@namedef{res@ots/openai-roberta/short/100/fpr-at-0.5}{11.7}
\@namedef{res@ots/openai-roberta/short/100/fpr-at-dev}{1.0}
\@namedef{res@ots/openai-roberta/short/100/fpr-at-devlen}{1.0}
\@namedef{res@ots/openai-roberta/short/100/fpr-at-devlen-ci/hi}{2.0}
\@namedef{res@ots/openai-roberta/short/100/fpr-at-devlen-ci/lo}{0.3}
\@namedef{res@ots/openai-roberta/short/100/thr-devlen}{0.8119}
\@namedef{res@ots/openai-roberta/short/100/tpr-at-0.5}{18.5}
\@namedef{res@ots/openai-roberta/short/100/tpr-at-dev}{1.0}
\@namedef{res@ots/openai-roberta/short/100/tpr-at-devlen}{1.0}
\@namedef{res@ots/openai-roberta/short/50/auroc}{0.668}
\@namedef{res@ots/openai-roberta/short/50/fpr-at-0.5}{9.9}
\@namedef{res@ots/openai-roberta/short/50/fpr-at-dev}{2.0}
\@namedef{res@ots/openai-roberta/short/50/fpr-at-devlen}{0.8}
\@namedef{res@ots/openai-roberta/short/50/fpr-at-devlen-ci/hi}{1.8}
\@namedef{res@ots/openai-roberta/short/50/fpr-at-devlen-ci/lo}{0.0}
\@namedef{res@ots/openai-roberta/short/50/thr-devlen}{0.8524}
\@namedef{res@ots/openai-roberta/short/50/tpr-at-0.5}{19.5}
\@namedef{res@ots/openai-roberta/short/50/tpr-at-dev}{1.0}
\@namedef{res@ots/openai-roberta/short/50/tpr-at-devlen}{0.5}
\@namedef{res@ots/openai-roberta/thr-dev}{0.8066}
\@namedef{res@ots/openai-roberta/thr-lenaware/120-160}{0.4858}
\@namedef{res@ots/openai-roberta/thr-lenaware/160-220}{0.8565}
\@namedef{res@ots/openai-roberta/thr-lenaware/220-320}{0.7857}
\@namedef{res@ots/openai-roberta/tpr-at-0.5}{19.6}
\@namedef{res@ots/openai-roberta/tpr-at-dev}{1.1}
\@namedef{res@ots/openai-roberta/tpr-at-lenaware}{10.5}
\@namedef{res@ots/openai-roberta/tpr-heldout-at-0.5}{16.3}
\@namedef{res@ots/openai-roberta/tpr-heldout-at-dev}{0.7}
\@namedef{res@ots/tmr-roberta/auroc}{0.292}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/g31fl}{0.350}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/g35fl}{0.287}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/gemma26}{0.445}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/gemma31}{0.474}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/gptoss}{0.193}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/kazllm}{0.319}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/qwen}{0.175}
\@namedef{res@ots/tmr-roberta/auroc-by-gen/sherkala}{0.199}
\@namedef{res@ots/tmr-roberta/auroc-ci/hi}{0.311}
\@namedef{res@ots/tmr-roberta/auroc-ci/lo}{0.274}
\@namedef{res@ots/tmr-roberta/auroc-heldout}{0.390}
\@namedef{res@ots/tmr-roberta/auroc-len120-220}{0.280}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/g31fl}{59.2}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/g35fl}{56.7}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/gemma26}{74.6}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/gemma31}{73.2}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/gptoss}{33.1}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/kazllm}{56.5}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/qwen}{24.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-0.5/sherkala}{34.7}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/g31fl}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/g35fl}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/gemma26}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/gemma31}{0.6}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/gptoss}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/kazllm}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/qwen}{0.0}
\@namedef{res@ots/tmr-roberta/flag-by-gen-at-dev/sherkala}{0.0}
\@namedef{res@ots/tmr-roberta/flag-gray-at-0.5/HP}{78.2}
\@namedef{res@ots/tmr-roberta/flag-gray-at-0.5/MH}{84.4}
\@namedef{res@ots/tmr-roberta/flag-gray-at-0.5/MIX}{13.9}
\@namedef{res@ots/tmr-roberta/flag-gray-at-0.5/MT}{83.0}
\@namedef{res@ots/tmr-roberta/flag-gray-at-dev/HP}{2.6}
\@namedef{res@ots/tmr-roberta/flag-gray-at-dev/MH}{0.0}
\@namedef{res@ots/tmr-roberta/flag-gray-at-dev/MIX}{0.0}
\@namedef{res@ots/tmr-roberta/flag-gray-at-dev/MT}{5.0}
\@namedef{res@ots/tmr-roberta/fpr-at-0.5}{81.4}
\@namedef{res@ots/tmr-roberta/fpr-at-dev}{2.1}
\@namedef{res@ots/tmr-roberta/fpr-at-dev-ci/hi}{2.9}
\@namedef{res@ots/tmr-roberta/fpr-at-dev-ci/lo}{1.4}
\@namedef{res@ots/tmr-roberta/fpr-at-lenaware}{2.3}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-0.5/encyclopedic}{80.2}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-0.5/essay}{70.4}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-0.5/news}{88.7}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-0.5/web}{80.0}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-dev/encyclopedic}{1.1}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-dev/essay}{2.3}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-dev/news}{3.0}
\@namedef{res@ots/tmr-roberta/fpr-by-domain-at-dev/web}{1.9}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-0.5/120-160}{87.1}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-0.5/160-220}{81.3}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-0.5/220-320}{67.8}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-dev/120-160}{3.7}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-dev/160-220}{1.8}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-dev/220-320}{0.0}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-lenaware/120-160}{4.6}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-lenaware/160-220}{1.8}
\@namedef{res@ots/tmr-roberta/fpr-by-len-at-lenaware/220-320}{0.0}
\@namedef{res@ots/tmr-roberta/script/canon-fpr-at-dev}{1.6}
\@namedef{res@ots/tmr-roberta/script/canon-tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/script/hg-tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/script/hg-tpr-orig-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/script/hgfold-tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/script/hghum-fold-at-dev}{1.9}
\@namedef{res@ots/tmr-roberta/script/hghum-n}{103}
\@namedef{res@ots/tmr-roberta/script/hghum-raw-at-dev}{1.9}
\@namedef{res@ots/tmr-roberta/script/latin-fpr-at-dev}{4.4}
\@namedef{res@ots/tmr-roberta/script/latin-tpr-at-dev}{0.5}
\@namedef{res@ots/tmr-roberta/script/latin2021}{0.274}
\@namedef{res@ots/tmr-roberta/script/latin2021canon}{0.293}
\@namedef{res@ots/tmr-roberta/script/trunc100}{0.673}
\@namedef{res@ots/tmr-roberta/script/trunc50}{0.655}
\@namedef{res@ots/tmr-roberta/short/100/auroc}{0.673}
\@namedef{res@ots/tmr-roberta/short/100/fpr-at-0.5}{9.4}
\@namedef{res@ots/tmr-roberta/short/100/fpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/short/100/fpr-at-devlen}{3.3}
\@namedef{res@ots/tmr-roberta/short/100/fpr-at-devlen-ci/hi}{5.3}
\@namedef{res@ots/tmr-roberta/short/100/fpr-at-devlen-ci/lo}{1.8}
\@namedef{res@ots/tmr-roberta/short/100/thr-devlen}{0.8066}
\@namedef{res@ots/tmr-roberta/short/100/tpr-at-0.5}{16.2}
\@namedef{res@ots/tmr-roberta/short/100/tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/short/100/tpr-at-devlen}{2.8}
\@namedef{res@ots/tmr-roberta/short/50/auroc}{0.655}
\@namedef{res@ots/tmr-roberta/short/50/fpr-at-0.5}{14.2}
\@namedef{res@ots/tmr-roberta/short/50/fpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/short/50/fpr-at-devlen}{4.3}
\@namedef{res@ots/tmr-roberta/short/50/fpr-at-devlen-ci/hi}{6.6}
\@namedef{res@ots/tmr-roberta/short/50/fpr-at-devlen-ci/lo}{2.5}
\@namedef{res@ots/tmr-roberta/short/50/thr-devlen}{0.8358}
\@namedef{res@ots/tmr-roberta/short/50/tpr-at-0.5}{23.1}
\@namedef{res@ots/tmr-roberta/short/50/tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/short/50/tpr-at-devlen}{3.0}
\@namedef{res@ots/tmr-roberta/thr-dev}{0.9777}
\@namedef{res@ots/tmr-roberta/thr-lenaware/120-160}{0.9771}
\@namedef{res@ots/tmr-roberta/thr-lenaware/160-220}{0.9777}
\@namedef{res@ots/tmr-roberta/thr-lenaware/220-320}{0.9742}
\@namedef{res@ots/tmr-roberta/tpr-at-0.5}{52.2}
\@namedef{res@ots/tmr-roberta/tpr-at-dev}{0.0}
\@namedef{res@ots/tmr-roberta/tpr-at-lenaware}{0.0}
\@namedef{res@ots/tmr-roberta/tpr-heldout-at-0.5}{63.8}
\@namedef{res@ots/tmr-roberta/tpr-heldout-at-dev}{0.2}
\@namedef{res@overlap/kazllm/mean}{1.1}
\@namedef{res@overlap/kazllm/p95}{6.7}
\@namedef{res@overlap/sherkala/mean}{1.1}
\@namedef{res@overlap/sherkala/p95}{8.4}
\@namedef{res@ppv/base/0.5/5}{40.4}
\@namedef{res@ppv/base/dev/5}{85.5}
\@namedef{res@ppv/combo-auglen+bino/dev/5}{83.0}
\@namedef{res@ppv/ots-desklib-deberta/0.5/5}{5.7}
\@namedef{res@ppv/ots-fakespot-roberta/0.5/5}{6.9}
\@namedef{res@ppv/ots-hc3-roberta/0.5/5}{--}
\@namedef{res@ppv/ots-openai-roberta/0.5/5}{7.7}
\@namedef{res@ppv/ots-tmr-roberta/0.5/5}{3.4}
\@namedef{res@qc/mixed-script-drops}{60}
\@namedef{res@qc/mixed-script-drops-g35fl}{38}
\@namedef{res@seedspan/all/fpr-at-dev}{0.6--0.7}
\@namedef{res@seedspan/all/fpr50-at-dev}{0.0--0.8}
\@namedef{res@seedspan/all/tpr-at-dev}{44.8--90.3}
\@namedef{res@seedspan/all/tpr-heldout-at-dev}{31.9--78.1}
\@namedef{res@seedspan/alllen/fpr-at-dev}{0.5--1.0}
\@namedef{res@seedspan/alllen/fpr50-at-dev}{0.8--1.5}
\@namedef{res@seedspan/alllen/tpr-at-dev}{92.2--98.0}
\@namedef{res@seedspan/alllen/tpr-heldout-at-dev}{82.4--86.2}
\@namedef{res@seedspan/allnoaug/fpr-at-dev}{0.5--2.4}
\@namedef{res@seedspan/allnoaug/fpr50-at-dev}{0.0--23.9}
\@namedef{res@seedspan/allnoaug/tpr-at-dev}{77.9--99.8}
\@namedef{res@seedspan/allnoaug/tpr-heldout-at-dev}{58.8--94.6}
\@namedef{res@seedspan/aug/fpr-at-dev}{0.5--1.0}
\@namedef{res@seedspan/aug/fpr50-at-dev}{0.0--6.3}
\@namedef{res@seedspan/aug/tpr-at-dev}{32.4--99.7}
\@namedef{res@seedspan/aug/tpr-heldout-at-dev}{20.1--84.8}
\@namedef{res@seedspan/auglen/fpr-at-dev}{1.5--2.2}
\@namedef{res@seedspan/auglen/fpr50-at-dev}{1.3--4.8}
\@namedef{res@seedspan/auglen/tpr-at-dev}{77.2--99.8}
\@namedef{res@seedspan/auglen/tpr-heldout-at-dev}{58.1--86.2}
\@namedef{res@seedspan/base/fpr-at-dev}{0.5--1.5}
\@namedef{res@seedspan/base/fpr50-at-dev}{0.8--2.3}
\@namedef{res@seedspan/base/tpr-at-dev}{89.3--99.8}
\@namedef{res@seedspan/base/tpr-heldout-at-dev}{61.5--86.9}
\@namedef{res@seedspan/kz/fpr-at-dev}{0.7--1.2}
\@namedef{res@seedspan/kz/fpr50-at-dev}{0.0--6.1}
\@namedef{res@seedspan/kz/tpr-at-dev}{91.9--99.1}
\@namedef{res@seedspan/kz/tpr-heldout-at-dev}{68.8--89.6}
\@namedef{res@seedspan/kzlen/fpr-at-dev}{0.5--1.1}
\@namedef{res@seedspan/kzlen/fpr50-at-dev}{0.8--1.8}
\@namedef{res@seedspan/kzlen/tpr-at-dev}{12.7--80.1}
\@namedef{res@seedspan/kzlen/tpr-heldout-at-dev}{7.7--64.3}
\@namedef{res@seedspan/kznoaug/fpr-at-dev}{0.9--1.4}
\@namedef{res@seedspan/kznoaug/fpr50-at-dev}{0.3--15.5}
\@namedef{res@seedspan/kznoaug/tpr-at-dev}{45.2--99.5}
\@namedef{res@seedspan/kznoaug/tpr-heldout-at-dev}{32.4--93.4}
\@namedef{res@seedspan/xlmr/fpr-at-dev}{1.0--1.3}
\@namedef{res@seedspan/xlmr/fpr50-at-dev}{0.0--2.0}
\@namedef{res@seedspan/xlmr/tpr-at-dev}{72.3--99.7}
\@namedef{res@seedspan/xlmr/tpr-heldout-at-dev}{62.4--88.2}
\@namedef{res@val/dates/encyclopedic/dated}{1,081}
\@namedef{res@val/dates/encyclopedic/max}{30 Apr 2022}
\@namedef{res@val/dates/encyclopedic/n}{1,081}
\@namedef{res@val/dates/essay/dated}{561}
\@namedef{res@val/dates/essay/max}{29 Nov 2022}
\@namedef{res@val/dates/essay/n}{561}
\@namedef{res@val/dates/news/dated}{1,095}
\@namedef{res@val/dates/news/max}{29 Nov 2022}
\@namedef{res@val/dates/news/n}{1,095}
\@namedef{res@val/dates/web/dated}{0}
\@namedef{res@val/dates/web/n}{1,074}
\@namedef{res@val/digits/base/auroc-nodigit}{0.993}
\@namedef{res@val/digits/base/flagged-nodigit}{5}
\@namedef{res@val/digits/base/fpr-digit}{0.6}
\@namedef{res@val/digits/base/fpr-nodigit}{2.4}
\@namedef{res@val/digits/combo/auroc-nodigit}{0.979}
\@namedef{res@val/digits/combo/flagged-nodigit}{7}
\@namedef{res@val/digits/combo/fpr-digit}{0.5}
\@namedef{res@val/digits/combo/fpr-nodigit}{3.3}
\@namedef{res@val/digits/h}{86}
\@namedef{res@val/digits/m}{28}
\@namedef{res@val/digits/n-h-nodigit}{209}
\@namedef{res@val/digits/n-h-nodigit-essay}{99}
\@namedef{res@val/family/auglen/gemma}{100.0}
\@namedef{res@val/family/auglen/kz}{58.1}
\@namedef{res@val/family/combo/gemma}{92.9}
\@namedef{res@val/family/combo/kz}{66.2}
\@namedef{res@val/family/n-gemma}{282}
\@namedef{res@val/family/n-kz}{160}
\@namedef{res@val/latin/max-fpr-high}{85}
\@namedef{res@val/latin/max-tpr-low}{0.5}
\@namedef{res@val/latin/min-fpr-high}{15}
\@namedef{res@val/latin/n}{20}
\@namedef{res@val/latin/n-high}{three}
\@namedef{res@val/latin/n-low}{17}
\@namedef{res@val/pools/dev-rows-any}{0}
\@namedef{res@val/pools/kz-gemma-rows}{0}
\@namedef{res@val/pools/kz-rows}{216}
\@namedef{res@val/pools/main-heldout-rows}{0}
\@namedef{res@val/pools/main-test-rows}{0}
\@namedef{res@val/split/dev-encyclopedic}{176}
\@namedef{res@val/split/dev-essay}{0}
\@namedef{res@val/split/dev-news}{104}
\@namedef{res@val/split/dev-web}{111}
\@namedef{res@val/split/essay-test-clusters}{three}
\@namedef{res@val/split/essay-train-clusters}{five}
\@namedef{res@val/split/n-neardup}{0}
\@namedef{res@val/split/shared-clusters}{0}
\@namedef{res@val/split/test-clusters}{29}
\@namedef{res@val/split/train-clusters}{39}
\@namedef{res@val/surface/auroc}{0.979}
\@namedef{res@val/surface/auroc-heldout}{0.946}
\@namedef{res@val/surface/auroc-len120-220}{0.979}
\@namedef{res@val/surface/fpr-at-dev}{2.2}
\@namedef{res@val/surface/n-features}{23}
\@namedef{res@val/surface/tpr-at-dev}{78.8}
\@namedef{res@val/surface/tpr-heldout-at-dev}{71.3}
\@namedef{res@val/templates/n}{3,844}
\@namedef{res@val/templates/other}{0}
\@namedef{res@val/thr/hi}{2.6}
\@namedef{res@val/thr/lo}{0.4}
\@namedef{res@val/thr/mean}{1.3}
\@namedef{res@val/thr/p-above}{29}
\@namedef{res@zs/best-tpr}{50.3}
\@namedef{res@zs/max-fpr-dev}{1.4}
\@namedef{res@zs/min-fpr-dev}{0.6}
\@namedef{res@zs/second-tpr}{16.5}
\makeatother
\newcommand{\RESotsList}{Fakespot RoBERTa, OpenAI RoBERTa, HC3 RoBERTa, TMR RoBERTa and Desklib DeBERTa}
\newcommand{\RESotsIDs}{\url{fakespot-ai/roberta-base-ai-text-detection-v1}, \url{openai-community/roberta-base-openai-detector}, \url{Hello-SimpleAI/chatgpt-detector-roberta}, \url{Oxidane/tmr-ai-text-detector} and \url{desklib/ai-text-detector-v1.01}}
\newcommand{\RESnHuman}{\res{corpus/n-human}}
\newcommand{\RESnMachine}{\res{corpus/n-nonhuman}}
\newcommand{\RESnGen}{\res{corpus/n-gen}}
\newcommand{\RESnOutlets}{\res{corpus/n-outlets}}
\newcommand{\RESnEduHosts}{\res{corpus/n-edu-hosts}}


==> results_extra.tex <==
\makeatletter
\@namedef{res@x/aud1/mt-m}{9}
\@namedef{res@x/aud1/n-gens}{five}
\@namedef{res@x/aud1/n-h}{52}
\@namedef{res@x/aud1/n-m}{48}
\@namedef{res@x/aud1/screen-only-h}{11}
\@namedef{res@x/aud1/screen-only-m}{5}
\@namedef{res@x/aud2/essay-n}{13}
\@namedef{res@x/aud2/essay-valid}{6}
\@namedef{res@x/ci/base/gemma4/boot/hi}{100.0}
\@namedef{res@x/ci/base/gemma4/boot/lo}{59.8}
\@namedef{res@x/ci/base/gemma4/cp/hi}{100.0}
\@namedef{res@x/ci/base/gemma4/cp/lo}{98.7}
\@namedef{res@x/ci/base/gemma4/k}{282}
\@namedef{res@x/ci/base/gemma4/n}{282}
\@namedef{res@x/ci/base/kazllm/boot/hi}{80.0}
\@namedef{res@x/ci/base/kazllm/boot/lo}{4.7}
\@namedef{res@x/ci/base/kazllm/cp/hi}{58.2}
\@namedef{res@x/ci/base/kazllm/cp/lo}{36.1}
\@namedef{res@x/ci/base/kazllm/k}{40}
\@namedef{res@x/ci/base/kazllm/n}{85}
\@namedef{res@x/ci/base/kz/boot/hi}{79.8}
\@namedef{res@x/ci/base/kz/boot/lo}{8.1}
\@namedef{res@x/ci/base/kz/cp/hi}{62.3}
\@namedef{res@x/ci/base/kz/cp/lo}{46.3}
\@namedef{res@x/ci/base/kz/k}{87}
\@namedef{res@x/ci/base/kz/n}{160}
\@namedef{res@x/ci/base/sherkala/boot/hi}{84.0}
\@namedef{res@x/ci/base/sherkala/boot/lo}{9.3}
\@namedef{res@x/ci/base/sherkala/cp/hi}{73.6}
\@namedef{res@x/ci/base/sherkala/cp/lo}{50.7}
\@namedef{res@x/ci/base/sherkala/k}{47}
\@namedef{res@x/ci/base/sherkala/n}{75}
\@namedef{res@x/ci/bino/gemma4/cp/hi}{93.3}
\@namedef{res@x/ci/bino/gemma4/cp/lo}{86.0}
\@namedef{res@x/ci/bino/gemma4/k}{254}
\@namedef{res@x/ci/bino/gemma4/n}{282}
\@namedef{res@x/ci/bino/kazllm/cp/hi}{61.6}
\@namedef{res@x/ci/bino/kazllm/cp/lo}{39.5}
\@namedef{res@x/ci/bino/kazllm/k}{43}
\@namedef{res@x/ci/bino/kazllm/n}{85}
\@namedef{res@x/ci/bino/kz/cp/hi}{69.4}
\@namedef{res@x/ci/bino/kz/cp/lo}{53.9}
\@namedef{res@x/ci/bino/kz/k}{99}
\@namedef{res@x/ci/bino/kz/n}{160}
\@namedef{res@x/ci/bino/sherkala/cp/hi}{84.0}
\@namedef{res@x/ci/bino/sherkala/cp/lo}{63.3}
\@namedef{res@x/ci/bino/sherkala/k}{56}
\@namedef{res@x/ci/bino/sherkala/n}{75}
\@namedef{res@x/dep/auglen/fpr}{1.9}
\@namedef{res@x/dep/auglen/fpr-ci/hi}{3.2}
\@namedef{res@x/dep/auglen/fpr-ci/lo}{0.4}
\@namedef{res@x/dep/auglen/fpr-essay}{0.5}
\@namedef{res@x/dep/auglen/fpr-web}{3.2}
\@namedef{res@x/dep/auglen/fpr50}{1.3}
\@namedef{res@x/dep/auglen/gemma4}{99.3}
\@namedef{res@x/dep/auglen/gemma4/boot/hi}{100.0}
\@namedef{res@x/dep/auglen/gemma4/boot/lo}{71.7}
\@namedef{res@x/dep/auglen/gemma4/cp/hi}{99.9}
\@namedef{res@x/dep/auglen/gemma4/cp/lo}{97.5}
\@namedef{res@x/dep/auglen/gemma4/k}{280}
\@namedef{res@x/dep/auglen/gemma4/n}{282}
\@namedef{res@x/dep/auglen/gray/HP}{15.4}
\@namedef{res@x/dep/auglen/gray/MH}{98.4}
\@namedef{res@x/dep/auglen/gray/MIX}{90.3}
\@namedef{res@x/dep/auglen/gray/MT}{9.4}
\@namedef{res@x/dep/auglen/hgfold}{99.0}
\@namedef{res@x/dep/auglen/kazllm}{45.9}
\@namedef{res@x/dep/auglen/kazllm/boot/hi}{58.8}
\@namedef{res@x/dep/auglen/kazllm/boot/lo}{24.1}
\@namedef{res@x/dep/auglen/kazllm/cp/hi}{57.0}
\@namedef{res@x/dep/auglen/kazllm/cp/lo}{35.0}
\@namedef{res@x/dep/auglen/kazllm/k}{39}
\@namedef{res@x/dep/auglen/kazllm/n}{85}
\@namedef{res@x/dep/auglen/kz}{53.1}
\@namedef{res@x/dep/auglen/kz/boot/hi}{63.4}
\@namedef{res@x/dep/auglen/kz/boot/lo}{34.8}
\@namedef{res@x/dep/auglen/kz/cp/hi}{61.0}
\@namedef{res@x/dep/auglen/kz/cp/lo}{45.1}
\@namedef{res@x/dep/auglen/kz/k}{85}
\@namedef{res@x/dep/auglen/kz/n}{160}
\@namedef{res@x/dep/auglen/latin-canon}{99.2}
\@namedef{res@x/dep/auglen/latin-canon-fpr}{1.8}
\@namedef{res@x/dep/auglen/ppv5}{72.4}
\@namedef{res@x/dep/auglen/sherkala}{61.3}
\@namedef{res@x/dep/auglen/sherkala/boot/hi}{73.3}
\@namedef{res@x/dep/auglen/sherkala/boot/lo}{43.3}
\@namedef{res@x/dep/auglen/sherkala/cp/hi}{72.4}
\@namedef{res@x/dep/auglen/sherkala/cp/lo}{49.4}
\@namedef{res@x/dep/auglen/sherkala/k}{46}
\@namedef{res@x/dep/auglen/sherkala/n}{75}
\@namedef{res@x/dep/auglen/tpr}{98.7}
\@namedef{res@x/dep/auglen/tpr-heldout}{82.6}
\@namedef{res@x/dep/auglen/tpr50}{67.3}
\@namedef{res@x/dep/combo-aug/fpr}{0.4}
\@namedef{res@x/dep/combo-aug/fpr-ci/hi}{1.9}
\@namedef{res@x/dep/combo-aug/fpr-ci/lo}{0.1}
\@namedef{res@x/dep/combo-aug/fpr-essay}{0.9}
\@namedef{res@x/dep/combo-aug/fpr-web}{0.4}
\@namedef{res@x/dep/combo-aug/fpr50}{0.8}
\@namedef{res@x/dep/combo-aug/gemma4}{94.3}
\@namedef{res@x/dep/combo-aug/gray/HP}{3.8}
\@namedef{res@x/dep/combo-aug/gray/MH}{85.9}
\@namedef{res@x/dep/combo-aug/gray/MIX}{63.9}
\@namedef{res@x/dep/combo-aug/gray/MT}{5.3}
\@namedef{res@x/dep/combo-aug/hgfold}{86.8}
\@namedef{res@x/dep/combo-aug/kazllm}{48.2}
\@namedef{res@x/dep/combo-aug/kz}{57.5}
\@namedef{res@x/dep/combo-aug/latin-canon}{82.9}
\@namedef{res@x/dep/combo-aug/latin-canon-fpr}{0.6}
\@namedef{res@x/dep/combo-aug/ppv5}{92.0}
\@namedef{res@x/dep/combo-aug/sherkala}{68.0}
\@namedef{res@x/dep/combo-aug/tpr}{87.2}
\@namedef{res@x/dep/combo-aug/tpr-heldout}{81.0}
\@namedef{res@x/dep/combo-aug/tpr50}{39.6}
\@namedef{res@x/dep/combo/fpr}{0.9}
\@namedef{res@x/dep/combo/fpr-ci/hi}{2.7}
\@namedef{res@x/dep/combo/fpr-ci/lo}{0.4}
\@namedef{res@x/dep/combo/fpr-essay}{0.9}
\@namedef{res@x/dep/combo/fpr-web}{1.5}
\@namedef{res@x/dep/combo/fpr50}{1.0}
\@namedef{res@x/dep/combo/gemma4}{92.9}
\@namedef{res@x/dep/combo/gemma4/boot/hi}{100.0}
\@namedef{res@x/dep/combo/gemma4/boot/lo}{82.3}
\@namedef{res@x/dep/combo/gemma4/cp/hi}{95.6}
\@namedef{res@x/dep/combo/gemma4/cp/lo}{89.3}
\@namedef{res@x/dep/combo/gemma4/k}{262}
\@namedef{res@x/dep/combo/gemma4/n}{282}
\@namedef{res@x/dep/combo/gray/HP}{9.0}
\@namedef{res@x/dep/combo/gray/MH}{87.5}
\@namedef{res@x/dep/combo/gray/MIX}{84.1}
\@namedef{res@x/dep/combo/gray/MT}{8.8}
\@namedef{res@x/dep/combo/hgfold}{84.1}
\@namedef{res@x/dep/combo/kazllm}{57.6}
\@namedef{res@x/dep/combo/kazllm/boot/hi}{74.1}
\@namedef{res@x/dep/combo/kazllm/boot/lo}{44.1}
\@namedef{res@x/dep/combo/kazllm/cp/hi}{68.3}
\@namedef{res@x/dep/combo/kazllm/cp/lo}{46.4}
\@namedef{res@x/dep/combo/kazllm/k}{49}
\@namedef{res@x/dep/combo/kazllm/n}{85}
\@namedef{res@x/dep/combo/kz}{61.3}
\@namedef{res@x/dep/combo/kz/boot/hi}{76.7}
\@namedef{res@x/dep/combo/kz/boot/lo}{54.5}
\@namedef{res@x/dep/combo/kz/cp/hi}{68.8}
\@namedef{res@x/dep/combo/kz/cp/lo}{53.2}
\@namedef{res@x/dep/combo/kz/k}{98}
\@namedef{res@x/dep/combo/kz/n}{160}
\@namedef{res@x/dep/combo/latin-canon}{85.2}
\@namedef{res@x/dep/combo/latin-canon-fpr}{1.0}
\@namedef{res@x/dep/combo/ppv5}{82.9}
\@namedef{res@x/dep/combo/ppv5-at-hi}{62}
\@namedef{res@x/dep/combo/sherkala}{65.3}
\@namedef{res@x/dep/combo/sherkala/boot/hi}{87.4}
\@namedef{res@x/dep/combo/sherkala/boot/lo}{58.7}
\@namedef{res@x/dep/combo/sherkala/cp/hi}{76.0}
\@namedef{res@x/dep/combo/sherkala/cp/lo}{53.5}
\@namedef{res@x/dep/combo/sherkala/k}{49}
\@namedef{res@x/dep/combo/sherkala/n}{75}
\@namedef{res@x/dep/combo/tpr}{85.2}
\@namedef{res@x/dep/combo/tpr-heldout}{81.4}
\@namedef{res@x/dep/combo/tpr50}{41.1}
\@namedef{res@x/dep/kzlen/fpr}{0.8}
\@namedef{res@x/dep/kzlen/fpr-ci/hi}{2.0}
\@namedef{res@x/dep/kzlen/fpr-ci/lo}{0.1}
\@namedef{res@x/dep/kzlen/fpr-essay}{0.0}
\@namedef{res@x/dep/kzlen/fpr-web}{2.2}
\@namedef{res@x/dep/kzlen/fpr50}{1.8}
\@namedef{res@x/dep/kzlen/gemma4}{53.2}
\@namedef{res@x/dep/kzlen/gemma4/boot/hi}{93.5}
\@namedef{res@x/dep/kzlen/gemma4/boot/lo}{3.8}
\@namedef{res@x/dep/kzlen/gemma4/cp/hi}{59.1}
\@namedef{res@x/dep/kzlen/gemma4/cp/lo}{47.2}
\@namedef{res@x/dep/kzlen/gemma4/k}{150}
\@namedef{res@x/dep/kzlen/gemma4/n}{282}
\@namedef{res@x/dep/kzlen/gray/HP}{6.4}
\@namedef{res@x/dep/kzlen/gray/MH}{84.4}
\@namedef{res@x/dep/kzlen/gray/MIX}{62.0}
\@namedef{res@x/dep/kzlen/gray/MT}{6.4}
\@namedef{res@x/dep/kzlen/hgfold}{63.3}
\@namedef{res@x/dep/kzlen/kazllm}{41.2}
\@namedef{res@x/dep/kzlen/kazllm/boot/hi}{72.4}
\@namedef{res@x/dep/kzlen/kazllm/boot/lo}{10.6}
\@namedef{res@x/dep/kzlen/kazllm/cp/hi}{52.4}
\@namedef{res@x/dep/kzlen/kazllm/cp/lo}{30.6}
\@namedef{res@x/dep/kzlen/kazllm/k}{35}
\@namedef{res@x/dep/kzlen/kazllm/n}{85}
\@namedef{res@x/dep/kzlen/kz}{42.5}
\@namedef{res@x/dep/kzlen/kz/boot/hi}{72.3}
\@namedef{res@x/dep/kzlen/kz/boot/lo}{15.0}
\@namedef{res@x/dep/kzlen/kz/cp/hi}{50.6}
\@namedef{res@x/dep/kzlen/kz/cp/lo}{34.7}
\@namedef{res@x/dep/kzlen/kz/k}{68}
\@namedef{res@x/dep/kzlen/kz/n}{160}
\@namedef{res@x/dep/kzlen/latin-canon}{72.4}
\@namedef{res@x/dep/kzlen/latin-canon-fpr}{1.0}
\@namedef{res@x/dep/kzlen/ppv5}{79.0}
\@namedef{res@x/dep/kzlen/sherkala}{44.0}
\@namedef{res@x/dep/kzlen/sherkala/boot/hi}{75.4}
\@namedef{res@x/dep/kzlen/sherkala/boot/lo}{16.0}
\@namedef{res@x/dep/kzlen/sherkala/cp/hi}{55.9}
\@namedef{res@x/dep/kzlen/sherkala/cp/lo}{32.5}
\@namedef{res@x/dep/kzlen/sherkala/k}{33}
\@namedef{res@x/dep/kzlen/sherkala/n}{75}
\@namedef{res@x/dep/kzlen/tpr}{64.8}
\@namedef{res@x/dep/kzlen/tpr-heldout}{49.3}
\@namedef{res@x/dep/kzlen/tpr50}{54.1}
\@namedef{res@x/devdep/auglen/fpr}{1.5}
\@namedef{res@x/devdep/auglen/fpr-web}{0.9}
\@namedef{res@x/devdep/auglen/fpr50}{1.3}
\@namedef{res@x/devdep/auglen/tpr-gemma}{98.3}
\@namedef{res@x/devdep/auglen/tpr-indist}{97.1}
\@namedef{res@x/devdep/auglen/tpr-kazllm}{29.6}
\@namedef{res@x/devdep/auglen/tpr-kazllm/k}{8}
\@namedef{res@x/devdep/auglen/tpr-sherkala}{57.1}
\@namedef{res@x/devdep/auglen/tpr-sherkala/k}{16}
\@namedef{res@x/devdep/combo-aug/fpr}{1.3}
\@namedef{res@x/devdep/combo-aug/fpr-web}{0.9}
\@namedef{res@x/devdep/combo-aug/fpr50}{2.6}
\@namedef{res@x/devdep/combo-aug/tpr-gemma}{91.4}
\@namedef{res@x/devdep/combo-aug/tpr-indist}{89.7}
\@namedef{res@x/devdep/combo-aug/tpr-kazllm}{51.9}
\@namedef{res@x/devdep/combo-aug/tpr-kazllm/k}{14}
\@namedef{res@x/devdep/combo-aug/tpr-sherkala}{64.3}
\@namedef{res@x/devdep/combo-aug/tpr-sherkala/k}{18}
\@namedef{res@x/devdep/combo-auglen/fpr}{1.5}
\@namedef{res@x/devdep/combo-auglen/fpr-web}{0.9}
\@namedef{res@x/devdep/combo-auglen/fpr50}{2.3}
\@namedef{res@x/devdep/combo-auglen/tpr-gemma}{96.6}
\@namedef{res@x/devdep/combo-auglen/tpr-indist}{89.0}
\@namedef{res@x/devdep/combo-auglen/tpr-kazllm}{63.0}
\@namedef{res@x/devdep/combo-auglen/tpr-kazllm/k}{17}
\@namedef{res@x/devdep/combo-auglen/tpr-sherkala}{64.3}
\@namedef{res@x/devdep/combo-auglen/tpr-sherkala/k}{18}
\@namedef{res@x/devdep/combo-base/fpr}{1.5}
\@namedef{res@x/devdep/combo-base/fpr-web}{0.9}
\@namedef{res@x/devdep/combo-base/fpr50}{2.6}
\@namedef{res@x/devdep/combo-base/tpr-gemma}{91.4}
\@namedef{res@x/devdep/combo-base/tpr-indist}{86.0}
\@namedef{res@x/devdep/combo-base/tpr-kazllm}{48.1}
\@namedef{res@x/devdep/combo-base/tpr-kazllm/k}{13}
\@namedef{res@x/devdep/combo-base/tpr-sherkala}{64.3}
\@namedef{res@x/devdep/combo-base/tpr-sherkala/k}{18}
\@namedef{res@x/devdep/combo/fpr}{1.5}
\@namedef{res@x/devdep/combo/fpr-web}{0.9}
\@namedef{res@x/devdep/combo/fpr50}{2.3}
\@namedef{res@x/devdep/combo/tpr-gemma}{96.6}
\@namedef{res@x/devdep/combo/tpr-indist}{89.0}
\@namedef{res@x/devdep/combo/tpr-kazllm}{63.0}
\@namedef{res@x/devdep/combo/tpr-sherkala}{64.3}
\@namedef{res@x/devdep/kzlen/fpr}{2.8}
\@namedef{res@x/devdep/kzlen/fpr-web}{4.5}
\@namedef{res@x/devdep/kzlen/fpr50}{2.0}
\@namedef{res@x/devdep/kzlen/tpr-gemma}{63.8}
\@namedef{res@x/devdep/kzlen/tpr-indist}{70.6}
\@namedef{res@x/devdep/kzlen/tpr-kazllm}{37.0}
\@namedef{res@x/devdep/kzlen/tpr-sherkala}{46.4}
\@namedef{res@x/falseflags/base/dev/hi}{37}
\@namedef{res@x/falseflags/base/dev/lo}{1}
\@namedef{res@x/hg/all}{5.2}
\@namedef{res@x/hg/test}{6.7}
\@namedef{res@x/human/under110}{4}
\@namedef{res@x/kz/under110}{65}
\@namedef{res@x/mc/aug/only-first}{20}
\@namedef{res@x/mc/aug/only-second}{27}
\@namedef{res@x/mc/aug/p}{0.38}
\@namedef{res@x/mc/augcombo/only-first}{3}
\@namedef{res@x/mc/augcombo/only-second}{9}
\@namedef{res@x/mc/augcombo/p}{0.15}
\@namedef{res@x/mc/auglen/only-first}{14}
\@namedef{res@x/mc/auglen/only-second}{27}
\@namedef{res@x/mc/auglen/p}{0.06}
\@namedef{res@x/mc/base/only-first}{23}
\@namedef{res@x/mc/base/only-second}{22}
\@namedef{res@x/mc/base/p}{1.00}
\@namedef{res@x/release/fpr}{0.9}
\@namedef{res@x/release/kazllm}{55.3}
\@namedef{res@x/release/kz}{60.0}
\@namedef{res@x/release/sherkala}{65.3}
\@namedef{res@x/release/tpr}{88.8}
\@namedef{res@x/release/tpr-ho}{81.9}
\@namedef{res@x/zs/gemma4-e2b:binoculars/auroc}{0.931}
\@namedef{res@x/zs/gemma4-e2b:binoculars/fpr}{0.8}
\@namedef{res@x/zs/gemma4-e2b:binoculars/tpr}{50.3}
\@namedef{res@x/zs/gemma4-e2b:binoculars/tpr-heldout}{79.9}
\@namedef{res@x/zs/gemma4-e2b:obs_entropy/auroc}{0.713}
\@namedef{res@x/zs/gemma4-e2b:obs_entropy/fpr}{2.0}
\@namedef{res@x/zs/gemma4-e2b:obs_entropy/tpr}{0.9}
\@namedef{res@x/zs/gemma4-e2b:obs_entropy/tpr-heldout}{1.1}
\@namedef{res@x/zs/gemma4-e2b:obs_fdg/auroc}{0.761}
\@namedef{res@x/zs/gemma4-e2b:obs_fdg/fpr}{0.7}
\@namedef{res@x/zs/gemma4-e2b:obs_fdg/tpr}{10.8}
\@namedef{res@x/zs/gemma4-e2b:obs_fdg/tpr-heldout}{19.5}
\@namedef{res@x/zs/gemma4-e2b:obs_ll/auroc}{0.770}
\@namedef{res@x/zs/gemma4-e2b:obs_ll/fpr}{1.8}
\@namedef{res@x/zs/gemma4-e2b:obs_ll/tpr}{1.9}
\@namedef{res@x/zs/gemma4-e2b:obs_ll/tpr-heldout}{6.3}
\@namedef{res@x/zs/gemma4-e2b:obs_logrank/auroc}{0.756}
\@namedef{res@x/zs/gemma4-e2b:obs_logrank/fpr}{1.5}
\@namedef{res@x/zs/gemma4-e2b:obs_logrank/tpr}{1.9}
\@namedef{res@x/zs/gemma4-e2b:obs_logrank/tpr-heldout}{5.4}
\@namedef{res@x/zs/gemma4-e2b:obs_lrr/auroc}{0.616}
\@namedef{res@x/zs/gemma4-e2b:obs_lrr/fpr}{1.4}
\@namedef{res@x/zs/gemma4-e2b:obs_lrr/tpr}{1.6}
\@namedef{res@x/zs/gemma4-e2b:obs_lrr/tpr-heldout}{6.8}
\@namedef{res@x/zs/gemma4-e2b:perf_entropy/auroc}{0.855}
\@namedef{res@x/zs/gemma4-e2b:perf_entropy/fpr}{1.8}
\@namedef{res@x/zs/gemma4-e2b:perf_entropy/tpr}{18.7}
\@namedef{res@x/zs/gemma4-e2b:perf_entropy/tpr-heldout}{31.0}
\@namedef{res@x/zs/gemma4-e2b:perf_fdg/auroc}{0.579}
\@namedef{res@x/zs/gemma4-e2b:perf_fdg/fpr}{0.7}
\@namedef{res@x/zs/gemma4-e2b:perf_fdg/tpr}{1.8}
\@namedef{res@x/zs/gemma4-e2b:perf_fdg/tpr-heldout}{15.6}
\@namedef{res@x/zs/gemma4-e2b:perf_ll/auroc}{0.870}
\@namedef{res@x/zs/gemma4-e2b:perf_ll/fpr}{1.6}
\@namedef{res@x/zs/gemma4-e2b:perf_ll/tpr}{11.1}
\@namedef{res@x/zs/gemma4-e2b:perf_ll/tpr-heldout}{33.5}
\@namedef{res@x/zs/gemma4-e2b:perf_logrank/auroc}{0.893}
\@namedef{res@x/zs/gemma4-e2b:perf_logrank/fpr}{2.1}
\@namedef{res@x/zs/gemma4-e2b:perf_logrank/tpr}{23.7}
\@namedef{res@x/zs/gemma4-e2b:perf_logrank/tpr-heldout}{48.9}
\@namedef{res@x/zs/gemma4-e2b:perf_lrr/auroc}{0.835}
\@namedef{res@x/zs/gemma4-e2b:perf_lrr/fpr}{1.7}
\@namedef{res@x/zs/gemma4-e2b:perf_lrr/tpr}{20.2}
\@namedef{res@x/zs/gemma4-e2b:perf_lrr/tpr-heldout}{22.2}
\@namedef{res@x/zs/llama3.2-3b:binoculars/auroc}{0.664}
\@namedef{res@x/zs/llama3.2-3b:binoculars/fpr}{1.4}
\@namedef{res@x/zs/llama3.2-3b:binoculars/tpr}{3.6}
\@namedef{res@x/zs/llama3.2-3b:binoculars/tpr-heldout}{9.3}
\@namedef{res@x/zs/llama3.2-3b:obs_entropy/auroc}{0.536}
\@namedef{res@x/zs/llama3.2-3b:obs_entropy/fpr}{3.5}
\@namedef{res@x/zs/llama3.2-3b:obs_entropy/tpr}{0.1}
\@namedef{res@x/zs/llama3.2-3b:obs_entropy/tpr-heldout}{1.8}
\@namedef{res@x/zs/llama3.2-3b:obs_fdg/auroc}{0.814}
\@namedef{res@x/zs/llama3.2-3b:obs_fdg/fpr}{1.0}
\@namedef{res@x/zs/llama3.2-3b:obs_fdg/tpr}{16.5}
\@namedef{res@x/zs/llama3.2-3b:obs_fdg/tpr-heldout}{29.9}
\@namedef{res@x/zs/llama3.2-3b:obs_ll/auroc}{0.637}
\@namedef{res@x/zs/llama3.2-3b:obs_ll/fpr}{3.9}
\@namedef{res@x/zs/llama3.2-3b:obs_ll/tpr}{2.1}
\@namedef{res@x/zs/llama3.2-3b:obs_ll/tpr-heldout}{6.3}
\@namedef{res@x/zs/llama3.2-3b:obs_logrank/auroc}{0.638}
\@namedef{res@x/zs/llama3.2-3b:obs_logrank/fpr}{3.7}
\@namedef{res@x/zs/llama3.2-3b:obs_logrank/tpr}{2.7}
\@namedef{res@x/zs/llama3.2-3b:obs_logrank/tpr-heldout}{7.0}
\@namedef{res@x/zs/llama3.2-3b:obs_lrr/auroc}{0.599}
\@namedef{res@x/zs/llama3.2-3b:obs_lrr/fpr}{1.8}
\@namedef{res@x/zs/llama3.2-3b:obs_lrr/tpr}{2.0}
\@namedef{res@x/zs/llama3.2-3b:obs_lrr/tpr-heldout}{5.2}
\@namedef{res@x/zs/llama3.2-3b:perf_entropy/auroc}{0.373}
\@namedef{res@x/zs/llama3.2-3b:perf_entropy/fpr}{2.2}
\@namedef{res@x/zs/llama3.2-3b:perf_entropy/tpr}{0.0}
\@namedef{res@x/zs/llama3.2-3b:perf_entropy/tpr-heldout}{0.7}
\@namedef{res@x/zs/llama3.2-3b:perf_fdg/auroc}{0.693}
\@namedef{res@x/zs/llama3.2-3b:perf_fdg/fpr}{1.3}
\@namedef{res@x/zs/llama3.2-3b:perf_fdg/tpr}{7.1}
\@namedef{res@x/zs/llama3.2-3b:perf_fdg/tpr-heldout}{12.0}
\@namedef{res@x/zs/llama3.2-3b:perf_ll/auroc}{0.483}
\@namedef{res@x/zs/llama3.2-3b:perf_ll/fpr}{2.9}
\@namedef{res@x/zs/llama3.2-3b:perf_ll/tpr}{0.0}
\@namedef{res@x/zs/llama3.2-3b:perf_ll/tpr-heldout}{2.0}
\@namedef{res@x/zs/llama3.2-3b:perf_logrank/auroc}{0.506}
\@namedef{res@x/zs/llama3.2-3b:perf_logrank/fpr}{3.3}
\@namedef{res@x/zs/llama3.2-3b:perf_logrank/tpr}{0.3}
\@namedef{res@x/zs/llama3.2-3b:perf_logrank/tpr-heldout}{2.7}
\@namedef{res@x/zs/llama3.2-3b:perf_lrr/auroc}{0.596}
\@namedef{res@x/zs/llama3.2-3b:perf_lrr/fpr}{1.9}
\@namedef{res@x/zs/llama3.2-3b:perf_lrr/tpr}{1.4}
\@namedef{res@x/zs/llama3.2-3b:perf_lrr/tpr-heldout}{5.9}
\@namedef{res@x/zs/max-fpr}{3.9}
\@namedef{res@x/zs/mgpt-1.3b:binoculars/auroc}{0.731}
\@namedef{res@x/zs/mgpt-1.3b:binoculars/fpr}{1.4}
\@namedef{res@x/zs/mgpt-1.3b:binoculars/tpr}{0.9}
\@namedef{res@x/zs/mgpt-1.3b:binoculars/tpr-heldout}{0.5}
\@namedef{res@x/zs/mgpt-1.3b:obs_entropy/auroc}{0.706}
\@namedef{res@x/zs/mgpt-1.3b:obs_entropy/fpr}{3.7}
\@namedef{res@x/zs/mgpt-1.3b:obs_entropy/tpr}{1.6}
\@namedef{res@x/zs/mgpt-1.3b:obs_entropy/tpr-heldout}{3.2}
\@namedef{res@x/zs/mgpt-1.3b:obs_fdg/auroc}{0.808}
\@namedef{res@x/zs/mgpt-1.3b:obs_fdg/fpr}{1.0}
\@namedef{res@x/zs/mgpt-1.3b:obs_fdg/tpr}{10.0}
\@namedef{res@x/zs/mgpt-1.3b:obs_fdg/tpr-heldout}{26.7}
\@namedef{res@x/zs/mgpt-1.3b:obs_ll/auroc}{0.782}
\@namedef{res@x/zs/mgpt-1.3b:obs_ll/fpr}{3.3}
\@namedef{res@x/zs/mgpt-1.3b:obs_ll/tpr}{5.2}
\@namedef{res@x/zs/mgpt-1.3b:obs_ll/tpr-heldout}{11.1}
\@namedef{res@x/zs/mgpt-1.3b:obs_logrank/auroc}{0.784}
\@namedef{res@x/zs/mgpt-1.3b:obs_logrank/fpr}{2.9}
\@namedef{res@x/zs/mgpt-1.3b:obs_logrank/tpr}{5.4}
\@namedef{res@x/zs/mgpt-1.3b:obs_logrank/tpr-heldout}{10.0}
\@namedef{res@x/zs/mgpt-1.3b:obs_lrr/auroc}{0.701}
\@namedef{res@x/zs/mgpt-1.3b:obs_lrr/fpr}{1.7}
\@namedef{res@x/zs/mgpt-1.3b:obs_lrr/tpr}{3.4}
\@namedef{res@x/zs/mgpt-1.3b:obs_lrr/tpr-heldout}{4.5}
\@namedef{res@x/zs/mgpt-1.3b:perf_entropy/auroc}{0.696}
\@namedef{res@x/zs/mgpt-1.3b:perf_entropy/fpr}{2.7}
\@namedef{res@x/zs/mgpt-1.3b:perf_entropy/tpr}{0.5}
\@namedef{res@x/zs/mgpt-1.3b:perf_entropy/tpr-heldout}{1.1}
\@namedef{res@x/zs/mgpt-1.3b:perf_fdg/auroc}{0.849}
\@namedef{res@x/zs/mgpt-1.3b:perf_fdg/fpr}{0.6}
\@namedef{res@x/zs/mgpt-1.3b:perf_fdg/tpr}{9.8}
\@namedef{res@x/zs/mgpt-1.3b:perf_fdg/tpr-heldout}{18.1}
\@namedef{res@x/zs/mgpt-1.3b:perf_ll/auroc}{0.798}
\@namedef{res@x/zs/mgpt-1.3b:perf_ll/fpr}{2.8}
\@namedef{res@x/zs/mgpt-1.3b:perf_ll/tpr}{5.1}
\@namedef{res@x/zs/mgpt-1.3b:perf_ll/tpr-heldout}{7.0}
\@namedef{res@x/zs/mgpt-1.3b:perf_logrank/auroc}{0.799}
\@namedef{res@x/zs/mgpt-1.3b:perf_logrank/fpr}{2.9}
\@namedef{res@x/zs/mgpt-1.3b:perf_logrank/tpr}{6.4}
\@namedef{res@x/zs/mgpt-1.3b:perf_logrank/tpr-heldout}{8.4}
\@namedef{res@x/zs/mgpt-1.3b:perf_lrr/auroc}{0.711}
\@namedef{res@x/zs/mgpt-1.3b:perf_lrr/fpr}{1.1}
\@namedef{res@x/zs/mgpt-1.3b:perf_lrr/tpr}{3.2}
\@namedef{res@x/zs/mgpt-1.3b:perf_lrr/tpr-heldout}{3.6}
\@namedef{res@x/zs/min-fpr}{0.6}
\@namedef{res@x/zs/n-stats}{44}
\@namedef{res@x/zs/qwen3-4b:binoculars/auroc}{0.509}
\@namedef{res@x/zs/qwen3-4b:binoculars/fpr}{1.0}
\@namedef{res@x/zs/qwen3-4b:binoculars/tpr}{1.3}
\@namedef{res@x/zs/qwen3-4b:binoculars/tpr-heldout}{3.4}
\@namedef{res@x/zs/qwen3-4b:obs_entropy/auroc}{0.698}
\@namedef{res@x/zs/qwen3-4b:obs_entropy/fpr}{2.0}
\@namedef{res@x/zs/qwen3-4b:obs_entropy/tpr}{2.7}
\@namedef{res@x/zs/qwen3-4b:obs_entropy/tpr-heldout}{10.6}
\@namedef{res@x/zs/qwen3-4b:obs_fdg/auroc}{0.475}
\@namedef{res@x/zs/qwen3-4b:obs_fdg/fpr}{1.4}
\@namedef{res@x/zs/qwen3-4b:obs_fdg/tpr}{1.5}
\@namedef{res@x/zs/qwen3-4b:obs_fdg/tpr-heldout}{4.3}
\@namedef{res@x/zs/qwen3-4b:obs_ll/auroc}{0.681}
\@namedef{res@x/zs/qwen3-4b:obs_ll/fpr}{1.9}
\@namedef{res@x/zs/qwen3-4b:obs_ll/tpr}{1.8}
\@namedef{res@x/zs/qwen3-4b:obs_ll/tpr-heldout}{7.5}
\@namedef{res@x/zs/qwen3-4b:obs_logrank/auroc}{0.687}
\@namedef{res@x/zs/qwen3-4b:obs_logrank/fpr}{1.8}
\@namedef{res@x/zs/qwen3-4b:obs_logrank/tpr}{2.0}
\@namedef{res@x/zs/qwen3-4b:obs_logrank/tpr-heldout}{9.0}
\@namedef{res@x/zs/qwen3-4b:obs_lrr/auroc}{0.659}
\@namedef{res@x/zs/qwen3-4b:obs_lrr/fpr}{0.8}
\@namedef{res@x/zs/qwen3-4b:obs_lrr/tpr}{2.7}
\@namedef{res@x/zs/qwen3-4b:obs_lrr/tpr-heldout}{8.1}
\@namedef{res@x/zs/qwen3-4b:perf_entropy/auroc}{0.608}
\@namedef{res@x/zs/qwen3-4b:perf_entropy/fpr}{1.9}
\@namedef{res@x/zs/qwen3-4b:perf_entropy/tpr}{0.5}
\@namedef{res@x/zs/qwen3-4b:perf_entropy/tpr-heldout}{1.8}
\@namedef{res@x/zs/qwen3-4b:perf_fdg/auroc}{0.718}
\@namedef{res@x/zs/qwen3-4b:perf_fdg/fpr}{1.9}
\@namedef{res@x/zs/qwen3-4b:perf_fdg/tpr}{7.8}
\@namedef{res@x/zs/qwen3-4b:perf_fdg/tpr-heldout}{24.9}
\@namedef{res@x/zs/qwen3-4b:perf_ll/auroc}{0.689}
\@namedef{res@x/zs/qwen3-4b:perf_ll/fpr}{2.2}
\@namedef{res@x/zs/qwen3-4b:perf_ll/tpr}{3.1}
\@namedef{res@x/zs/qwen3-4b:perf_ll/tpr-heldout}{12.0}
\@namedef{res@x/zs/qwen3-4b:perf_logrank/auroc}{0.688}
\@namedef{res@x/zs/qwen3-4b:perf_logrank/fpr}{1.8}
\@namedef{res@x/zs/qwen3-4b:perf_logrank/tpr}{1.8}
\@namedef{res@x/zs/qwen3-4b:perf_logrank/tpr-heldout}{7.9}
\@namedef{res@x/zs/qwen3-4b:perf_lrr/auroc}{0.562}
\@namedef{res@x/zs/qwen3-4b:perf_lrr/fpr}{1.0}
\@namedef{res@x/zs/qwen3-4b:perf_lrr/tpr}{1.0}
\@namedef{res@x/zs/qwen3-4b:perf_lrr/tpr-heldout}{1.4}
\@namedef{res@x/zs/second-fpr}{2.1}
\@namedef{res@x/zs/second-name}{Gemma-4-E2B performer log-rank}
\@namedef{res@x/zs/second-tpr}{23.7}
\makeatother

